Double Machine Learning for Static Panel Models with Fixed Effects

Recent advances in causal inference have seen the development of methods which make use of the predictive power of machine learning algorithms. In this paper, we develop novel double machine learning (DML) procedures for panel data in which these algorithms are used to approximate high-dimensional and nonlinear nuisance functions of the covariates. Our new procedures are extensions of the well-known correlated random effects, within-group and first-difference estimators from linear to nonlinear panel models, specifically, Robinson (1988)'s partially linear regression model with fixed effects and unspecified nonlinear confounding. Our simulation study assesses the performance of these procedures using different machine learning algorithms. We use our procedures to re-estimate the impact of minimum wage on voting behaviour in the UK. From our results, we recommend the use of first-differencing because it imposes the fewest constraints on the distribution of the fixed effects, and an ensemble learning strategy to ensure optimum estimator accuracy.

==> 02_MODEL_OLD.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The Partially Linear Panel Regression Model}\label{sec:model}
\setcounter{equation}{0}
\setcounter{theorem}{0}
\setcounter{lemma}{0}
\setcounter{proposition}{0}

To introduce notation, suppose the panel study collected information on each of $N$ individuals at each of the $t$ time periods, or waves. %\footnote{The estimation problem and results hold with unbalanced panel with appropriate modifications in the notation.}  
Let $\{\yit,\dit,\xit : \ t=1,\ldots,T\}$ be independent and identically distributed (\emph{iid}) random variables for individuals $i=1,\ldots,N$, where $\yit$ is the outcome (or dependent) variable, $\dit$ a continuous or binary treatment  variable (or intervention), and $\xit$ a $p\times 1$ vector of control variables, usually including a constant term, able to capture time-varying confounding induced by non-random treatment selection. For continuous $\dit$, if $\dit\geq 0$ then a dose-response relationship is presumed to hold with $\dit=0$ indicating null treatment; otherwise, $\dit$ is taken to be centered around its mean $\mu_D$ such that $\dit \equiv \dit-\mu_D$. For binary $\dit\in\{0,1\}$, $\dit=0$ is taken to indicate the absence and $\dit=1$ the presence of treatment.

To extend the partially linear model of \citet{robinson1988} to panel data, we use the potential outcomes causal framework from, e.g., \citet{rubin1974}. As pointed out by \citet{lechner2015}, this allows us to interpret the resulting partially linear panel model as reduced-form without relying on specific parametric model for the data generating process. Hence, further define the set $\yit(.)=\{y_{it}(d):d\in \Omega_D\}$ containing all potential outcomes for individual $i$ at wave $t$, where $\yit(d)$ is the realization of the outcome for individual $i$ at wave $t$ were the treatment level set to $d$, with one potential outcome for every possible value the treatment could take. The realizations of the wave $t$ potential outcomes are taken to occur before treatment selection at wave $t$, and are linked to the observed outcome by the {\em consistency assumption} that $y_{it}(d_{it})=y_{it}$ with the others latent {\em counterfactuals}.\footnote{The stable unit treatment value (SUTVA) assumption, that $y_{it}(d)$ does not depend on the treatment assignments of any other individual, is implicitly taken to hold.} In the interval preceding wave $t$, it is also presumed that the realization of time-varying predictor $\xit$ precedes that of $(y_{it},d_{it})$. 

Finally, define the sets $\xi_i$ of time-invariant heterogeneity terms influencing $(\yit,\dit)$, and $L_{t-1}(w_i) = \{w_{i1},\dots,w_{it-1}\}$ the lags of variable(s) $w$ available at wave $t$ such that $L_0(w_i)\equiv\varnothing$. Using this notation, the assumptions which must be satisfied by the causal data generating process (DGP) can be stated as follows:
\begin{assumption}\label{item:asm_feedback} 
    \textsc{(No feedback to predictors)} $\xit \indep{}  {L_{t-1}(y_i,d_i)}   L_{t-1}({\bf x}_i),\xi_i.$ 
\end{assumption}
\begin{assumption}\label{item:asm_nolags} 
    \textsc{(Static panel)} $\yit,\dit  \indep{}  {L_{t-1}(y_i,{\bf x}_i,d_i)} \xit,\xi_i$. 
\end{assumption}
\begin{assumption}\label{item:asm_selection_fe} 
    \textsc{(Selection on observables and omitted time-invariant variables)}
    $\yit(.)\indep{}\dit \xit,\xi_i$.    
\end{assumption}
\begin{assumption} \label{item:asm_effect_fe}   
    \textsc{(Homogeneity of the treatment effect)}  \\
    $E[\yit(d)-\yit(0)|\xit]=d\theta_0$.
\end{assumption}
\begin{assumption}\label{item:asm_additive} 
    \textsc{(Additive Separability)} 
    $l_0(\xit,\xi_i)=l_1(\xit)+\alpha_i$ and $m_0(\xit,\xi_i) = m_1(\xit)+\gamma_i$, where $\alpha_i=\alpha(\xi_i)$ and $\gamma_i=\gamma(\xi_i)$.
\end{assumption}

%%%%%%%%%%%%%%%% 
To summarize, Assumptions~\ref{item:asm_feedback}-\ref{item:asm_nolags} together ensure that the panel is static and that all lag dependence is due to non-causal autocorrelation. These assumptions also avoid the {\em initial conditions problem} which would arise were the panel study to have started after the joint process began.  Assumption~\ref{item:asm_selection_fe} states that treatment selection at wave $t$ is (strongly) ignorable given $\xit$ and latent $\xi_i$; this can be relaxed to the weakly ignorable assumption that only $\yit(0)\indep{}\dit \xit,\xi_i$, in which case $\theta_0$ is the average treatment effect among the treated (ATT) $E[\yit(1)-\yit(0)\mid \dit=1]$, but we assume throughout that the strong version holds. Assumption~\ref{item:asm_effect_fe} requires the population average effect of treatment-level $d$ to be homogeneous, which holds if $y_{it}(d)-y_{it}(0)$ is constant or varies randomly between individuals; for non-binary treatments, this assumption additionally implies a linear dose-response relationship because the mean of $\yit(d)-\yit(0)$ is linear in $d$. If homogeneity is not a reasonable assumption then there are two options available to the analyst:\ the first is to interpret the estimand as an {\em honest} ATE; and the second is to allow for heterogeneity by directly estimating the conditional average treatment effect (CATE) (i.e., when $y_{it}(d)-y_{it}(0)$ depends on $\xit$). As such, we will focus on the homogenous case but discuss both options when introducing Proposition~\ref{prop:neyman} and Theorem \ref{thm:cre_dml}).\footnote{Heterogeneous causal effects can be estimated if the analyst is prepared to specify parametric model $E[\yit(d)-\yit(0) |\xit]=f_{\btheta_0}(d;\xit,t)$ for the CATE. If $E[\yit(d)-\yit(0)\mid\xit,\xi_i]$ depends on $\xi_i$ then $f_{\btheta_0}$ relates only to other populations with the same distribution of $\xi_i$ as the target population.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
Assumptions~\ref{item:asm_feedback}-\ref{item:asm_additive} lead to the partially linear panel regression (PLPR) model 
\begin{equation} 
    \yit = \dit\theta_0 + g_1(\xit) + \alpha_i + \uit, 
\end{equation} 
\noindent where $g_1(\xit)+\alpha_i=E[\yit(0)\mid\xit,\xi_i]$. Alternatively, the partialled-out partially linear panel regression (PO-PLPR) is 
\begin{align} 
    \yit & = \vit\theta_0  + l_1(\xit) + \alpha_i + \uit, \label{eqn:plr2_y} \\ 
    \vit & = \dit - m_1(\xit) - \gamma_i \label{eqn:plr2_v}, 
\end{align} 
\noindent where $l_1(\xit)+\gamma_i=E[\yit\mid\xit,\xi_i]$. Both models are extensions of \citet{robinson1988}'s PLR model to panel data with fixed effects, where $\alpha_i$ and $\gamma_i$ are generally correlated because both are functions of the omitted time-invariant influences~$\xi_i$. The derivation based on Assumptions~\ref{item:asm_feedback}-\ref{item:asm_additive} is detailed in the Online Supplement~\ref{sec:appx_model}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Fixed-effects Estimation}\label{sec:estimators}
\setcounter{equation}{0}
\setcounter{theorem}{0}
\setcounter{lemma}{0}
\setcounter{proposition}{0}

In this section, we propose two approaches for estimating $\theta_0$ based on PO-PLPR model \eqref{eqn:plr2_y}-\eqref{eqn:plr2_v}. The presence of the time-invariant fixed effects means that, naively, only $l_1(\xit)+E[\alpha_i|\xit]$ and $m_1(\xit)+E[\gamma_i|\xit]$ can be learnt from the observed data. These approaches are adaptations of existing techniques for {\em linear} panel data models based on correlated random effects (CRE) and two varieties of data transformation:\ the first-difference (FD) and within-group (WG).  

%%%%%%%%%%%%%
\subsection{Correlated Random Effects}\label{sec:three_approaches}
For the linear case $l_1(\xit)=\xit{\bf l}_1$, \citet{mundlak1978} proposes replacing $\alpha_i$ with the linear projection $\alpha_i=\bzi\bpi_0 + a_i$, where $\bzi=T^{-1}\sum_{t=1}^T\zit$ is the vector of individual-specific means of (mean-centred) ${\bf z}_{it}=(\xit,\dit)$. This results in a (reduced-form) linear panel model $\yit=\xit{\bf l}_0 + \dit\theta_0 + \bzi\bpi_0 + r_{it}$, where $r_{it}=a_i+u_{it}$ is orthogonal to the space spanned by $\zit$ such that $\theta_0$, ${\bf l}_1$ and $\bpi_0$ can be estimated using standard linear panel estimators \citep[Section\ 2.3]{wooldridge2010}.  However, linear projections cannot guarantee the orthogonality of non-linear $l_1(\xit)$ and $\alpha_i$, and $m_1(\xit)$ and $\gamma_i$ for the PO-PLPR model, so stronger modelling assumptions about $\alpha_i$ and $\gamma_i$ are required. 

\begin{proposition}[\textsc{CRE}]\label{prop:cre} 
Suppose that the data generating process $\mathcal{P}$ satisfies Assumption~\ref{item:asm_feedback} - Assumption~\ref{item:asm_additive} so that Model~\eqref{eqn:plr2_y}-\eqref{eqn:plr2_v} holds, and also that the fixed effects satisfy $\alpha_i= \omega_\alpha(\bxi)+a_i$  and  $\gamma_i = \omega_\gamma(\bxi) + c_i$,  where $(a_i,c_i)\ {\perp\!\!\!\perp}\ L_T({\bf x}_i)$ and $a_i\ {\perp\!\!\!\perp}\ c_i$. Then it is feasible to learn $\widetilde{l}_1$ and $\widetilde{m}_1$ in 
\begin{align} 
    \yit & =\vit\theta_0 + \widetilde{l}_1(\xit,\bxi)+a_i+\uit \label{eqn:cre_y}\\ 
    \vit & = \dit - \widetilde{m}_1(\xit,\bxi) - c_i, \label{eqn:cre_v} 
\end{align} 
\noindent where $E[\uit \mid\vit,\xit,\bxi,a_i\big]=E[\vit|\xit,\bxi,c_i]=0$, $\widetilde{l}_1(\xit,\bxi)=l_1(\xit) + \omega_{\alpha}(\bxi)$ and $\widetilde{m}_1(\xit,\bxi) = m_1(\xit)+\omega_\gamma(\bxi)$. 
\end{proposition} 
A proof is given in the printed appendix. 

The model in Proposition~\ref{prop:cre} is similar to that proposed by \citet{wooldridge2020}.  It effectively converts {\em fixed effects} Model~\eqref{eqn:plr2_y} and~\eqref{eqn:plr2_v}, with $\alpha_i$ and $\gamma_i$ mean-dependent on $\xit$ and $\dit$, into a random effects problem where $a_i$ and $c_i$ are mean-independent.\footnote{Under the \emph{random effects assumption}, where $E[\alpha_i|\xit]=E[\alpha_i]=0$ and $E[\gamma_i|\xit]=E[\gamma_i]=0$, $l_1$ and $m_1$ can be straightforwardly learnt from the observed data, but we assert that this is unlikely to hold in practice and hence valid causal inference would not be not guaranteed. However, were the analysis prepared to make the random effects assumption, we note that \citet{sela2012} developed an algorithm for using tree-based learners to estimate non-causal partially linear regression models.} 
This allows us to learn $\widetilde{l}_1$ and $\widetilde{m}_1$ from the observed data:\ it follows from proposition~\ref{prop:cre} that $l_0(\xit,\alpha_i)=E[\yit|\xit,\bar{{\bf x}}_i,a_i]$ such that $E[\yit|\xit,\bar{{\bf x}}_i]=\widetilde{l}_1(\xit,\bar{{\bf x}}_i)$ and, similarly, $E[\dit|\xit,\bar{{\bf x}}_i]=\widetilde{m}_1(\xit,\bar{{\bf x}}_i)$. A DML estimator for $\theta_0$ based on this model is derived in Section~\ref{sec:estimation}. 

%%%%%%%
\subsection{Data Transformations}\label{sec:exact}
The second approach we consider follows more conventional techniques for panel data by transforming the data to remove entirely the fixed effects from the analysis. 

Let $\wit$ be a generic random variable and $Q$ a panel data transformation operator such that $Q(\wit)=Q_t(w_{i1},\dots,w_{iT})$ is a function of the random variable at wave $t$ and the remaining realizations for \mbox{individual $i$}. We consider two such transformations:\ the WG (within-group), or time-demeaning, transformation $Q({w}_{it})=\wit-\overline{w}_{it}$, where  $\overline{w}_{i}= T\inv \sum_{t=1}^T \wit$; and the FD (first-difference) transformation $Q({w}_{it}) = \wit-w_{it-1}$ for $t=2,...,T$. The reduced-form model for $Q(\yit)$ and $Q(\vit)$ under Model~\eqref{eqn:plr2_y}-\eqref{eqn:plr2_v} is 
\begin{align}
    Q(\yit) & = Q(\vit)\theta_0 + Q\big({l}_1(\xit)\big) + Q(\uit) \label{eqn:Q_y} \\
    Q(\vit) & = Q(\vit)-Q\big({m}_1(\xit)\big), \label{eqn:Q_d}
\end{align}
\noindent which does not depend on fixed effects $\alpha_i$ and $\gamma_i$ because $Q(\alpha_i)=Q(\gamma_i)=0$.

The challenge of learning the transformed nuisance functions $Q\big({l}_1(\xit)\big)$ and $ Q\big({m}_1(\xit)\big)$ is complicated by the non-linearity of $l_1$ and $m_1$, as discussed in Section~\ref{sec:nuisance}.



==> 03a_ESTIMATION_OLD.tex <==
\section{DML for Panel Data}\label{sec:estimation}
\setcounter{equation}{0}

We now set out the two-stage DML procedure for the fixed-effects models presented in Section~\ref{sec:estimators}. Further details on the DML algorithm for panel data are provided in the Online Supplement~\ref{sec:dml_algorithm}. We wish to make inference on the target parameter $\theta_0$ given a suitable predictions of the collection of nuisance functions $\bmeta_0$ based on the observed data $W_i = \{W_{it}: t=1,\dots,T\}$, where $W_{it} = \{\yit,\dit,\xit, \bxi\}$ with $\bxi=T\inv\sum_{t=1}^T\xit$ for CRE, and $W_{it} = \{Q(\yit),Q(\dit),Q(\xit)\}$ for the transformation approach (noting that $W_{i1}\equiv\varnothing$ if $Q$ is the FD transformation) as appropriate for the approach chosen by the analyst to handle the fixed effects problem.  %Note that, in the descriptions below, we distinguish between the \emph{estimation} of causal parameter $\theta_0$ and \emph{learning} $\bmeta_0$ because, while statistical inference based on the method of moments is required for the former, ML is used only to obtain predictions for each person at each wave for the latter. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning the Nuisance Parameters}\label{sec:nuisance}
\setcounter{equation}{0}
\setcounter{theorem}{0}
\setcounter{lemma}{0}
\setcounter{proposition}{0}

The nuisance parameters vary between individuals as functions $\bmeta_{0i}=\bmeta_0(\x_{i1},\ldots,\x_{iT})$.  We take these   for each individual so stage one requires the analyst to model $\bmeta_0$.  As discussed previously, the presence of the fixed effects and possibly non-linear nuisance functional forms in the estimating equations~\eqref{eqn:plr2_y}-\eqref{eqn:plr2_v} pose some challenges in learning $l_1$ and $m_1$ directly from the data. Below we describe different procedures for learning the nuisance parameters with the CRE approach, the transformation approaches (\emph{approximation} or \emph{exact}) when the WG and FD transformations are chosen.  

%%% cre

\subsubsection{Correlated Random Effects}  

The estimation of $\theta_0$ based on model (\ref{eqn:cre_y})-(\ref{eqn:cre_v}) requires learning $\widetilde{l}_1(\xit,\bxi)$ from the data $\{\yit,\xit,\bxi:t=1,\dots,T\}_{i=1}^N$, and obtaining predicted residual $\hat{v}_{it}$ to plug into (\ref{eqn:cre_y}). Simply learning $\widetilde{m}_1(\xit,\bxi)$ from the data $\{\dit,\xit,\bxi:t=1,\dots,T\}_{i=1}^N$ and using $\hat{v}_{it}=\dit - {\widehat{m}_1}(\xit,\bxi)$ would ignore individual heterogeneity $c_i$ and so introduce bias. Hence, we propose the following: 
%% proposition 1: CRE 
\begin{proposition}[\textsc{CRE}]\label{prop:cre_dml} 
Suppose the conditions set out in Proposition \ref{prop:cre} all hold, and that $\bvi = T\inv \sum_{t=1}^T \vit$ can be ignored. We provide two results. 
(a) Multivariate normality. We can learn $\tmi_1(\xit,\bxi)+c_i$ by learning $m_1^*(\xit,\bxi,\bdi)$ from data $\{\dit,\xit,\bxi,\bdi:t=1,\dots,T\}_{i=1}^N$ (supervised by $\dit$) if $d_{i1},\dots,d_{iT}|\xit,\bxi$ is multivariate normal with $E[\dit|\xit,\bxi] = \tmi_1(\xit,\bxi)$ and a homoskedastic variance-covariance matrix with random effects structure. 
(b) Generally, the following algorithm can be used: 

\setcounter{bean}{0} 
\begin{center} 
\begin{list} 
{\textsc{Step} \arabic{bean}.}{\usecounter{bean}} 
\item Learn $\tmi_1(.)$ from $\big\{\dit,\xit,\bxi,:t=1,\dots,T \big\}_{i=1}^N$ with prediction $\widehat{m}_{1i}=\tmi_1\widehat{(\xit,\bxi)}$. 
    \item Calculate $\widehat{\bmi}_i=T\inv\sum_{t=1}^T\hmi_{1i}$. 
    \item Calculate $\widehat{m^*}{(\xit,\bxi,\bdi)}=\widehat{m}_{1i}+\bdi-\widehat{\bmi}_i$. 
\end{list} 
\end{center} 
\end{proposition} 
\noindent A proof is given in the printed appendix. 
It is essential to include the individual-specific treatment mean $\bdi$ to ensure $\vit$ is included in the prediction of $m_1^*$. If the data are multivariate normal then the necessary function can be learnt directly from the data, otherwise it has to be constructed via part~(b). 

%%% TRANSFORMATION
\subsubsection{Transformation approaches}  
Superficially, it appears that (\ref{eqn:Q_y})-(\ref{eqn:Q_d}) presents a straightforward learning problem.  For example, $E[\yit-y_{it-1} \mid {\bf x}_{it-1},\xit]=l_1(\xit)-l_1({\bf x}_{it-1})\equiv \Delta l_1({\bf x}_{it-1},\xit)$ and $E[\dit-d_{it-1} \mid {\bf x}_{it-1},\xit]=m_1(\xit)-m_1(\x_{it-1})\equiv \Delta m_1(\x_{it-1},\xit)$ under Assumptions \ref{item:asm_feedback}-\ref{item:asm_additive}, but it is not possible to learn $\Delta l_1(\x_{it-1},\xit)$ and $\Delta m_1(\x_{it-1},\xit)$ from the sample data in the same way as $\tilde{l}_1$ and $\tilde{m}_1$ are in Proposition \ref{prop:cre_dml}.
Other approaches are required. 

First, we consider learning based on the transformed data alone. Generally, $Q\big({l}_1(\xit)\big)\ne {l}_1\big(Q(\xit)\big)$ and $Q\big({m}_1(\xit)\big)\ne {m}_1\big(Q(\xit)\big)$ unless $l_1$ and $m_1$ are linear. This means a consistent estimator cannot be simply constructed from the transformed data. 
However, we propose the following approximate estimators. 

\begin{lemma}[\textsc{Approximation}]\label{lemma:approx} 
Model (\ref{eqn:Q_y})-(\ref{eqn:Q_d}) can be approximated by 
\begin{align} 
       Q(\yit) & \approx Q(\vit)\theta_0 + {l}_1\big(Q(\xit)\big) + Q(\uit) \label{eqn:aQ_y}\\ 
       Q(\dit) & \approx {m}_1\big(Q(\xit)\big) + Q(\vit), \label{eqn:aQ_v} 
\end{align} 
\noindent where $l_1$ and $m_1$ can be learnt from the transformed data $\{Q(\yit),Q(\xit): t=1,\dots,T\}_{i=1}^N$ and $\{Q(\dit),Q(\xit): t=1,\dots,T\}_{i=1}^N$ , respectively. 
\end{lemma} 
\noindent This approach can produce good approximations of the nuisance functions when these are expected to be linear in the covariates. A discussion of this approximation is given in the Appendix, but ultimately we do not consider it further.  Instead, we focus on the following {\em exact} estimators. 


\begin{proposition}\label{prop:exact}  
(a) \textsc{Exact.} Consider the FD transformation $Q(y_{it})=\yit-y_{it-1}$. Then under Assumptions \ref{item:asm_feedback}-\ref{item:asm_additive}, $E[\yit-y_{it-1} \mid \x_{it-1}, \xit]=\Delta l_1(\x_{it-1},\xit)$ and  $E[\dit-d_{it-1}\mid\x_{it-1},\xit]=\Delta m_1(\x_{it-1},\xit)$, so that $\Delta l_1(\x_{it-1},\xit)$ can be learnt using $\{\yit-y_{it-1},\x_{it-1}, \xit: t=2,\dots,T\}_{i=1}^N$ and $\Delta m_1(\x_{it-1},\xit)$ can be learnt using $\{\dit-d_{it-1}, \linebreak \x_{it-1}, \xit:t=2,\ldots,T\}_{i=1}^N$.  However, for the WG transformation where $E[\yit-\byi\mid L_T({\bf x}_i) ]=l_1(\xit) - T\inv\sum_{s=1}^T l_1(\x_{is}) $ and $E[\dit-\bdi| L_T({\bf x}_i))]=m_1(\xit) - T\inv\sum_{s=1}^T\linebreak m_1(\x_{is})$,  the dimension of the learning problem is $O(T^2)$ times greater than that of the first-difference transformation.\\ 
(b) \textsc{Hybrid.}  
Suppose the conditions of Proposition~\ref{prop:cre} hold and the data generating process satisfies $p(\alpha_i|\Xii)=p(\alpha_i|\bxi)$. Then $\tl_1(\xit,\bxi)=l_1 (\xit)+\omega_\alpha(\bxi)$ and $\tm_1(\xit,\bxi)=m_1(\xit)+\omega_\gamma(\bxi)$ learnt from the sample data satisfy $Q\big(\tl_1(\xit,\bxi)\big)=Q\big(l_1(\xit)\big)$ and $Q(\tm_1(\xit,\bxi)\big)=Q\big(m_1(\xit)\big)$. 
\end{proposition} 
\noindent A proof is given in the printed appendix. The exact WG estimator is unfeasible for nontrivial $T$ because it involves learning a function involving all $T\times p$ variables. Hence, we propose the hybrid WG estimator as an alternative but note its close relationship with the CRE estimator. In the following, we focus on the CRE, exact FD and hybrid WG procedures.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Neyman Orthogonal Score Function}\label{sec:no_score}
We wish to make inference on the target parameter $\theta_0$ given a suitable estimate of the nuisance parameter $\bmeta_0$ from the data $W = \{W_{it}: t=1,\dots,T\}_{i=1}^N$, where $W_{it} = w\{\yit,\dit,\xit\}$ and $w$ is a transformation of the data (possibly the identity) chosen by the analyst to implement one of the estimation approaches discussed in Section~\ref{sec:estimators}. Following the doubly/debiased approach in \citet{chernozhukov2018}, we construct a Neyman-orthogonal score function, whose property allows us to obtain valid inferences using DML algorithms (provided the ML algorithms converge at rate $N^{1/4}$). 

%The following proposition sets out the form of the Neyman-orthogonal score.  
\begin{proposition}[\textsc{Neyman orthogonal}]\label{prop:neyman}  
Let ${\bf r}_i$ be a column-vector containing the residuals of the reduced-form model (PO-)PLPR model (based on untransformed or transformed variables), $\Xii$ a matrix of conditioning variables, and $\Sigma(\Xii)=E[{\bf r}_i{\bf r}'_i\mid \Xii]$ the (potentially) heteroskedastic residual variance-covariance matrix (recall that ${\bf r}'$ is the matrix transpose of column vector ${\bf r}$). Suppose that $\bmeta$ is a finite-vector of square-integrable and Lipschitz-continuous functionals where true value $\bmeta_0\in {\cal T}$ a convex subset of a normed vector space.  Suppose also that $||E[\partial_{\theta}f_{\theta}| \Xii]||^4,||\partial_{\theta}f_{\theta}||^2$ and $||\Sigma(\Xii)||^{-2}$ all have finite expectations under data generating process ${\cal P}$; and there exists finite $C_h$ such that $\Pr(|| E[\psi^\perp | \di,\Xii] || < C_h) = 1$, where $h=\bmeta\neq \bmeta_0$ and norm $||.||$ is with respect to ${\cal P}$. Then the Neyman orthogonal score has the form 
\begin{equation}\label{eqn:sec_score} 
    \psi^\perp(W_i;\theta_0,\bmeta_0)=V_i^\perp\Sigma_0\inv(\Xii){\bf r}_i, 
\end{equation} 
\noindent where row vector $V^\perp_i$ contains the {\em orthogonalized regressors} chosen to ensure Neyman orthogonality. We consider two important special cases. 
%%%%%%%%%%%%%%%%%%%%%%%% 
(a) \textsc{The CRE approach.} Under model (\ref{eqn:cre_y})-(\ref{eqn:cre_v}), $r_{it}=a_i+u_{it}=\yit-\vit f_{\theta_0}(\xit,t) - \widetilde{l}_1(\xit,\bxi)$, $v_{it}=\dit - \widetilde{m}_1(\xit,\bxi)-c_i$ and $V_i^\perp=\big(v_{i1}\partial_{\theta}f_{\theta_0}(x_{i1},1),\ldots, v_{iT}\partial_{\theta}f_{\theta_0}(x_{iT},T)\big)$, where $\partial_{\theta}f_{\theta_0}(x_{it},t)$ is a column vector of partial derivatives of $f_{\theta}(x_{it},t)$ with respect to the elements of $\theta$ evaluated at $\theta_0$.  
%%%%%%%%%%%%%%%%%%%%%%% 
(b) \textsc{The transformation approach.} Under model (\ref{eqn:Q_y})-(\ref{eqn:Q_d}),  $r_{it}=Q(u_{it})=Q(\yit)-Q\big(\vit f_{\theta_0}(\xit,t)\big) - Q\big(l_1(\xit) \big)$ and $V_i^{\perp}=\big( Q(v_{i1}\partial_{\theta}f_{\theta_0}(x_{i1},1) ),\ldots, Q( v_{iT}\partial_{\theta}f_{\theta_0}(x_{iT},T) )\big)$.  
\end{proposition} 
\noindent A proof is given in the appendix. In both cases, the orthogonalized regressor simplifies under Assumption~\ref{item:asm_effect_fe} because $f_{\theta_0}(\xit,t)=\theta_0$ so that $V_i^\perp = (v_{i1},\ldots, v_{iT})$ for the CRE approach and $V_i^\perp = \big(Q(v_{i1}),\ldots, Q(v_{iT})\big)$ for the transformation approach. 
Were this assumption to fail, however, the estimand of ${\hat\theta}_{DML}$ would remain causal; e.g., the estimand of the CRE estimator becomes $E\big[\sum_t {\rm Var}(\dit|\xit)f_{\theta_0}(\xit,t)\big]/E\big[\sum_t {\rm Var}(\dit|\xit)\big]$.\footnote{Follows simply from extending the arguments used to derive Equation~(23) in \citet{vansteelandt2014}.} We call this an \emph{honest} ATE because groups with the greatest balance between treatment and controls, and hence greatest variance, contribute most to the average, and groups with zero variance, indicating no overlap, contribute nothing; under random treatment allocation, the honest ATE equals the ATE.

%\red{The orthogonal score reduces the regularization bias, while sample splitting with cross-fitting (for $K\ge2$) reduces the overfitting bias and restores efficiency. }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Inference About the Target Parameter}
We now present the main result concerning inference about $\theta_0$ using DML. 

\begin{theorem}\label{thm:cre_dml}
Suppose that the assumptions and conditions set out in Proposition \ref{prop:neyman}, the conditions in \citet[Assumptions 3.1-3.2]{chernozhukov2018} hold, and (\ref{eq:hetero}) satisfies $f_{\theta_0}(\xit,t)={\bf s}_{it}\theta_0$, where ${\bf s}_{it}={\bf s}(\xit,t)$ is a row-vector from design matrix $S_i=\{{\bf s}_{it}\}^T_{t=1}$ . Suppose also that we have suitable ML algorithms available to obtain ${\hat\bmeta}$ from learning $\bmeta_0$ in Section~\ref{sec:nuisance} at rate $N^{1/4}$, and a ${\sqrt N}$-consistent estimator for $\Sigma_0(\Xii)$.  Then the DML estimator $\thetano_{DML}$, based on a) Neyman-orthogonal score \eqref{eqn:sec_score} and b) block-$K$-fold cross-fitting, is $\sqrt{N}$-consistent for $\theta_0$ and converges to the normal limiting distribution given by \citet[Theorem~4.1]{chernozhukov2018} with variance-covariance estimated by $${\hat\sigma}^2 = J\inv\Big\{N\inv\sum_{i\in W}\psi^\perp({W}_i; \thetano_{DML}, {\hat\bmeta})\psi^\perp(W_i; \thetano_{DML}, {\hat\bmeta})'\Big\} J\inv,$$
where $J=N\inv\sum_{i\in W}V_i^\perp \big(V_i^\perp\big)'$ and $M'$ is the matrix transpose of arbitrary $M$.
\end{theorem}
%%%%%%%%%%
The proof is an extension of \citet[Theorem 4.1]{chernozhukov2018} from the PLR model to the PLPR and PO-PLPR models. The regularity conditions extend straightforwardly from those in \citet[Assumption 4.1]{chernozhukov2018}; for example, for the CRE approach where $\bmeta_0=(\widetilde{l}_1,\widetilde{m}_1)$, this involves setting $U \equiv {\bf r}_i$, $Y\equiv\yi$, $V \equiv V_i^\perp\Sigma_0^{-1}(\Xii,\bxi)$, $D\equiv {\rm diag}(\di)S_i$ and $X\equiv (\Xii,\bxi)$, where ${\rm diag}(\di)$ is a square diagonal matrix with $\di$ on the diagonal and zero elsewhere. The resulting score is linear with the form $\psi^\perp=\psi^a\theta_0 + \psi^b$ where $\psi^a=-S'_i{\rm diag}(\vi)\Sigma_0^{-1}(\Xii,\bxi){\rm diag}(\vi)S_i$ and the proof follows. %(noting that $M'$ is the transpose of matrix $M$)
Finally, note that block-$K$-fold cross-fitting involves sampling $W_i$ rather than $W_{it}$ to ensure the $i.i.d.$\ assumption required by DML is satisfied; this procedure is described in detail in Online Supplement~\ref{sec:dml_algorithm}.

%The estimator of $\Sigma_0(\Xii,\bxi)$, used to control the efficiency of the resulting estimator, is taken to be based on a parametric model and so to converge at rate $\sqrt{N}$ to a finite value matrix. If this model is mis-specified then ${\hat\theta}_{DML}$ remains consistent. 
The DML procedure we propose (see Online Supplement~\ref{sec:dml_algorithm}) is based on a locally efficient estimator equivalent to setting homoskedastic $\Sigma_0(\Xii,\bxi)=\Sigma_0$ (for the CRE estimator), but we handle the resulting clustering using cluster-robust standard errors. More generally, an estimator allowing for heteroskedastic residuals based on the above result would require the analyst to specify a parametric model for $\Sigma_0(\Xii,\bxi)$. The estimator based on this model need only converge to its plim at rate $\sqrt{N}$, even if this model is mis-specified:\ by standard generalized method of moments arguments, the  consistency of ${\hat\theta}_{DML}$ would be unaffected, only its efficiency, which would be locally efficient in the sense of being semi-parametrically efficient were the model for the variance-covariance matrix correctly specified.

==> 06_CONCLUSION_OLD.tex <==
\section{Conclusion}\label{sec:conclusion}
DML is a powerful tool for leveraging the power of ML for robust estimation of treatment, or policy-intervention, effects. Although the theory underpinning DML is very general, there have only been two applications of it to causal inference from panel data:\ for average causal effect estimation from static panels \citep{klosin2022} and conditional average causal effect estimation from dynamic panels \citep{semenova2023}. However, in contrast to these papers, and to much of the econometric literature on machine learning, we do not equate ML with LASSO but instead build estimation procedures more generally making only weak assumptions (specifically, Lipschitz continuity) about the form of the nuisance function. This means that analysts can choose any appropriate learner or adopt an {\em ensemble} learning strategy in which multiple learners are used and the final estimate based on the best-performing learner (as measured by a suitable loss function like RMSE).

Our paper describes novel DML estimation procedures for causal estimation from panel data with non-linear confounding effects with no (causal) lag dependence  and all unobserved confounding due to omitted time-invariant variables. We focus on the homogeneous case but show how our procedures extend straightforwardly to conditional average treatment effect estimation for user-specified treatment effect models. While \citet{klosin2022} and \citet{semenova2023} focus on using LASSO to learn the form of the treatment effect heterogeneity, the tailoring of DML to the class of problems we consider is important because it remains a staple of applied research, and the tailored solutions help to manage the computational challenges inherent in using any kind of ML. Analysts can use the estimation procedures we propose in place of existing ones or in a complementary way to test the robustness of their results to non-linearity.

In practice, even if the regularity conditions described in Proposition \ref{prop:cre_dml} are satisfied, the performance of the learner is an empirical challenge for applied researchers. In our simulations, the LASSO with an extended dictionary of non-linear terms performed best across all scenarios. However, despite Lipschitz continuity and weak sparsity conditions holding, we found tree-based learners to perform poorly in terms of bias (of the point and interval estimates) and in terms of standard deviation and normality, even after making extensive efforts to implement adaptive hyperparameter tuning.  We do not claim this is a general result (there are many successful applications of tree-based learners in the literature), but we do strongly recommend for practice that analysts use an ensemble strategy involving multiple learners, as is standard practice with the use of ML in the wider data sciences to ensure robustness.

Finally, our procedure does not extend to dynamic panel models. For example, while relaxing \ref{item:asm_nolags} to allow first-order conditional dependence of $(\dit,\yit)$ on $y_{it-1}$, and extending \ref{item:asm_selection_fe} so that $E[\yit(0)\mid \dit, y_{it-1},\xit,\xi_i]=E[\yit(0)\mid y_{it-1},\xit,\xi_i]$, would induce a PO-PLPR model with nuisance parameters $l_1(y_{it-1},\xit)$ and $m_1(y_{it-1},\xit)$ for which the FD transformation could be used to remove the fixed effects, the learning problem is unfeasible because Proposition \ref{prop:exact}.i fails if the conditioning set is extended to include $y_{it-1}$. 
Novel further work could involve following \citet{semenova2023} by directly modeling $l_0(y_{it-1},\xit,\alpha_i)$ under a strict sparsity assumption for $\alpha_i$. However, for panels with long between-wave intervals, the plausibility of $\xi_i$ inducing fixed or nonzero correlations irrespective of time interval between residual pairs, let alone as the dominant source of omitted confounding, seems questionable.

%We explicate the underlying assumptions which must be satisfied by data generating processes, without specifying a structural model, to derive the reduced-form PLPR model, and derive the form of the Neyman-orthogonal score function required for DML. This reduces to replacing the treatment regressor with a mean-centered the treatment (or treatment difference) and weighting by the covariance matrix of the residuals. While we focus on the homogeneous treatment effects in the simulation and empirical studies, our results generalize straightforwardly to user-specified parametric models for the treatment effect that can include wave fixed effects.

%DML is a powerful tool for %is already realizing the great potential it has for the social sciences, and particularly for 
%leveraging the power of ML for robust estimation of policy-intervention effects. Although the theory underpinning DML is very general, there have only been two applications of it to causal inference from panel data, \citet{klosin2022} and \citet{semenova2023}. %However, with the availability of longitudinal data sets, this may limit the applicability of the method.
%In this paper, we developed novel DML procedures for estimating intervention effects from panel studies. These procedures are based on a simple extension of the partially linear regression model to panel data.  We proposed three estimators -- CRE, WG, and FD -- that account for the presence of unobserved individual heterogeneity that is potentially correlated with the regressors. For the within-group and first-differences estimators, we proposed two alternative approaches called \emph{approximation} and \emph{hybrid}:\ the former was found to perform well when the nuisance functions were linear or non-linear and smooth without interactions, while the latter was more robust and performed best in terms of bias when the nuisance functions were non-linear and discontinuous. This is in line with other work showing that the final causal parameter estimate may be adversely affected by the functional forms of the nuisance parameters learned during the first stage of estimation \citep[Section S1.1 in the Supplementary Material]{rudolph2023}. 

%Our implementation of the DML method is general and widely applicable because it can be used with any ML algorithm (e.g., CART and RF) and not only with statistical learners like LASSO.  More negatively, we found that tree-based algorithms require considerable attention from the analyst particularly with regards to hyperparameter tuning to control the bias-variance trade-off. This is in line with recent work emphasizing the sensitivity of ML algorithms for causal analysis to hyperparameter choice \citep{machlanski2023}. 
%from incorrectly tuned learners may eventually affect the estimation and inference of the causal parameter in the second (\emph{domino effect}). 
%LASSO with an extended dictionary performed the best in terms of bias reduction and statistical inference. Although hyperparameter tuning is less challenging for LASSO because it has only one hyperparameter, the disadvantage of using LASSO is that the extended dictionary, specified by the analyst without knowledge of the true functional form of the nuisance parameters, must be rich enough to capture the truth and so can become computationally demanding in terms of storage memory. Trees, in contrast, do not require the analyst to guess the composition of the dictionary. % especially if hyperparameter tuning is not conducted properly  (e.g., short trees in a random forest may lead to underfitting). 
%However, LASSO with an extended dictionary including non-linear terms requires a larger data set including more transformed variables stored.  Trees have the advantage of not requiring this to capture higher-order polynomials and interactions, but we found difficulties in controlling both bias and precision using the two hyperparameter-tuning strategies we considered. 
%However, while the focus of our study was to investigate the performance of two widely used families of learner, our findings emphasize the importance of following the widely used practice in ML {\em not} to rely on one base learner but to use {\em ensembles} comprising multiple learners (e.g., boosting, stacked learners, and super learners) because these usually outperform single base learners \citep{valentini2002}. 

%Monte Carlo simulations showed that there are gains from the use of DML with flexible learners when the true functional form is highly non-linear with discontinuities and interactions. The sequence of estimated causal effects from tree-based learners may not be asymptotically normally distributed  when the hyperparameters are tuned incorrectly. No convergence of tree-based approach into a Gaussian distribution with consequences on the estimated standard errors being too small, hence, the importance of hyperparameter tuning.

%%%% DISCUSSION %%%%
%We have shown differences and similarities in the estimated effects between OLS and DML with different base learners. 
%We have also shown that DML for the partially linear panel model is a practicable alternative to conventional linear panel methods for static panel data. 
%The results of our empirical analysis showed that DML made no substantive difference to the conclusions drawn from OLS results, but this can be viewed as a robustness check for non-linearity.  However, our simulation study showed that the bias due to incorrectly assuming linearity can be substantial, and that DML can correct for it. Hence, DML has value as an estimation technique in its own right, {\em and} as a robustness check in analyses where it may be more convenient to report the results obtained using linear models, which are more familiar and easier to understand.  % This holds more generally also be used for robustness checks because it is easier for analysts to deal with a linear than a partially linear model. However, the advantage that our approach brings is a clear distinction between causal and nuisance parameters, and that the selection of the control variables is automatically conducted by the ML algorithms. 

%Finally, we note that it is relatively simple to extend our method to allow for treatment heterogeneity by estimating {\em conditional} average treatment effects rather than average treatment effects {\em if} the analyst is prepared to specify a parametric model for the heterogeneity in terms of the regressors and across time. However, if the analyst wishes to use ML to learn the heterogeneity function then another method is needed.  Further work will extend the {\em quasi-oracle} approach of \citet{nie2021} to static panel models, and further to dynamic models.  This would complement the LASSO-based dynamic approach with heterogeneous effects proposed by \citet{semenova2023} to a more general DML estimator which can be used as part of a conventional ML ensemble.

==> 888_additional_figs.tex <==
\section{Additional Figures}\label{sec:add_figs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% dotplots
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SHOW IN PRESENTATIONS!

% \begin{figure}[ht!]
%     \caption{Simulation results, CRE estimator}
%     \label{fig:dotplot_fd}
%     \centering
%     \subfloat{\includegraphics[scale=.8]{figs/dot_cre_dgp.pdf}}
%     \vspace{-1mm}
%     \begin{minipage}{.9\linewidth}
%     \vspace{-1mm}
%     \emph{Note: Averages over 100 Monte Carlo replications. DGP1 is linear in the nuisance functions; DGP2 smooth non-linear; DGP3 non-smooth non-linear; time is fixed to $t=10$ time periods.}
%     \end{minipage}
% \end{figure}


% \begin{figure}[ht!]
%     \caption{Simulation results, FD estimator (with lagged inputs)}
%     \label{fig:dotplot_fd}
%     \centering
%     \subfloat{\includegraphics[scale=.8]{figs/dot_fdLag_dgp.pdf}}
%     \vspace{-1mm}
%     \begin{minipage}{.9\linewidth}
%     \vspace{-1mm}
%     \emph{Note: Averages over 100 Monte Carlo replications. DGP1 is linear in the nuisance functions; DGP2 smooth non-linear; DGP3 non-smooth non-linear; time is fixed to $t=10$ time periods.}
%     \end{minipage}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% kdensities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
    \centering
    \subfloat{\includegraphics[scale=.75]{figs/kdensity_dgp_fdLag2.pdf}}
    \caption{Distribution of $\thetano$ across simulation designs, approximation FD estimator (with lagged inputs)}\label{fig:kdensity_dgp_fdLag}
    \vspace{1mm}
    \begin{minipage}{1\linewidth}
    \emph{Note: Comparison of estimated target parameter in 100 Monte Carlo replications. The true target parameter $\theta$ is 0.50. The sample size is fixed to 1000 cross-sectional units and 10 time periods. Hyperparameters of base learners are tuned via grid search.}
    \end{minipage}
\end{figure}

\begin{figure}[ht!]
    \centering
    \subfloat{\includegraphics[scale=.75]{figs/kdensity_dgp_wg_hybrid.pdf}}
    \caption{Distribution of $\thetano$ across simulation designs, WG estimator (hybrid)}\label{fig:kdensity_dgp_wg} 
    \vspace{1mm}
    \begin{minipage}{1\linewidth}
    \emph{Note: Comparison of estimated target parameter in 100 Monte Carlo replications. The true target parameter $\theta$ is 0.50. The sample size is fixed to 1000 cross-sectional units and 10 time periods. Hyperparameters of base learners are tuned via grid search.}
    \end{minipage}
\end{figure}



==> 888_additional_material.tex <==
\section{Supplementary Material}\label{sec:additional material}
\setcounter{table}{0}
\numberwithin{table}{section}
\setcounter{page}{0}

\input{tabs/sum_dgp.tex}

%\input{tabs/tab_summary_fazio5.tex}


==> 888_figures.tex <==
\begin{figure}[ht!]
    \centering
    \caption{Distribution of $\thetano$, CRE estimator}\label{fig:kdensity_dgp_cre}
    \subfloat{\includegraphics[scale=.85]{figs/kdensity_dgp_cre.pdf}}
    \vspace{-1mm}
    \begin{minipage}{.9\linewidth}
    \vspace{-1mm}
    \emph{Note: Comparison of estimated target parameter in 100 Monte Carlo replications. The true target parameter $\theta$ is 0.50. The sample size is fixed to 1000 cross-sectional units and 10 time periods. Hyperparameters of base learners are tuned via grid search, selecting values from intervals reported in Table~\ref{tab:hyperpara}.}
    \end{minipage}
\end{figure}

==> 888_tables.tex <==
\input{tabs/tab_design}
% %\input{tabs/scores}

\input{tabs/88_simul_results_cre.tex}
%\input{tabs/99_dml_tab5_fazio}
\input{tabs/04_tab5_ols_dmlsim}
% %\input{tabs/99_tabs_fazio}
% % \input{tabs/tab5_fazio_noFE.tex}
% % \input{tabs/tab5_fazio.tex}
% \input{tabs/tab_hp_tuned.tex}




==> 999_notes_hyperpara.tex <==


\begin{enumerate}
    \item ParamSet - Learner and Search Space: Decide which hyperparameters to tune and what range to tune them over.  Given infinite resources, we could tune all hyperparameters jointly, but in reality that is not possible (or maybe necessary), so usually only a subset of hyperparameters can be tuned. This subset of possible hyperparameter values to tune over is referred to as the search space (SS) or tuning space. \red{Set a search space (SS) for each param in Learner.} For numeric hyperparameters (we will explore others later) one must specify the bounds to tune over.
    \item Terminators - When to stop: We have decided which hyperparameters to tune, we specify when to stop the tuning process. The search stops after \texttt{n\_evals} iterations (evaluations).
    \item TuningInstance* - Search Scenario: The tuning instance collects the tuner-agnostic information required to optimize a model, i.e., all information about the tuning process, except for the tuning algorithm itself. This includes the task to tune over, the learner to tune, the resampling method and measure used to analytically compare hyperparameter optimization configurations, and the terminator to determine when the measure has been optimized ‘enough’. This implicitly defines a “black box” objective function, mapping hyperparameter configurations to (stochastic) performance values, to be optimized.  
    Evaluator and container for resampled performances of hyperparameter configurations (HPCs). Stores archive of all evaluated experiments and final result.
    \item Tuner - Search Strategy: we can now decide how to tune our model. Implements 
    different HPO (or more generally speaking black box optimization) algorithms
    Generates HPCs and passes to tuning instance for evaluation until termination. Grid search and random search (Bergstra and Bengio 2012) are the most basic algorithms and are often selected first in initial experiments. The idea of grid search is to exhaustively evaluate every possible combination of given hyperparameter values.  Categorical hyperparameters are usually evaluated over all possible values they can take. Numeric and integer hyperparameter values are then spaced equidistantly in their box constraints (upper and lower bounds) according to a given resolution, which is the number of distinct values to try per hyperparameter. Both methods are non-adaptive, which means each proposed configuration ignores the performance of previous configurations. Due to their simplicity, both grid search and random search can handle mixed search spaces (i.e., hyperparameters can be numeric, integer, or categorical) as well as hierarchical search spaces
    \item Triggering the tuning process: we can start the tuning process. To do this we simply pass the constructed TuningInstanceSingleCrit to the \$optimize() method of the initialized Tuner, which triggers the hyperparameter optimization loop. The optimizer returns the best hyperparameter configuration and the corresponding performance.

    \item Results: Each row of the archive is a different evaluated configuration on 5 resempling configurations
    \item Training an optimized model -- Once we found good hyperparameters for our learner through tuning, we can use them to train a final model on the whole data. set the learner hyperparameters to the optimal configuration. Now we can train the learner on the full dataset and we are ready to make predictions.


\end{enumerate}

As a rule of thumb, if the search space is small or does not have a complex structure, grid search may be able to exhaustively evaluate the entire search space in a reasonable time. However, grid search is generally not recommended due to the curse of dimensionality – the grid size ‘blows up’ very quickly as the number of parameters to tune increases – and insufficient coverage of numeric search spaces. By construction, grid search cannot evaluate a large number of unique values per hyperparameter, which is suboptimal when some hyperparameters have minimal impact on performance while others do. In such scenarios, random search is often a better choice as it considers more unique values per hyperparameter compared to grid search.

For higher-dimensional search spaces or search spaces with more complex structure, more guided optimization algorithms such as evolutionary strategies or Bayesian optimization tend to perform better and are more likely to result in peak performance.

The resolution is the number of distinct values to try per hyperparameter, which means in our example the tuner will construct a 5x5 grid of 25 configurations of equally spaced points between the specified upper and lower bounds. All configurations will be tried by the tuner (in random order) until either all configurations are evaluated or the terminator (Section 4.1.2) signals that the budget is exhausted. 

HPO requires additional resampling to reduce bias when estimating the performance of a model. If the same data is used for determining the optimal configuration and the evaluation of the resulting model itself, the actual performance estimate might be biased (Simon 2007). test-training like DML

\begin{itemize}
    \item \texttt{tune\_on\_folds=FALSE => data\_tune\_list = list(self\$data\$data\_model)}: passes all data in the function \texttt{dml\_tune()}
    \item \texttt{TuningInstanceSingleCrit\$new(...
    resampling = tune\_settings\$rsmp\_tune, ...)}
    \item \texttt{rsmp\_tune = mlr3::rsmp("cv", folds = 5)} in \$tune() divides the data into 5 folds (different from those used for the DML procedure) used for cv.
    \item The tuning process begins by deciding which hyperparameters to tune and what range to tune them over. The first place to start is therefore picking a learner and looking at the possible hyperparameters to tune with. This subset of possible hyperparameter values to tune over is referred to as the search space or tuning space.
    \item mlr3tuning includes many methods to specify when to terminate an algorithm, which are implemented in Terminator classes. 
    The most commonly used terminators are those that stop the tuning after a certain time (trm("run\_time")) or a given number of evaluations (trm("evals")).
    \item The tuning algorithm starts to optimize $x$ parameter(s) with TunerGridSearch and TerminatorEvals.  Runs $s$ evaluations for the benchmark (default 5). Once finished optimizing after the $s$ evaluation(s), you get the list of hyperparameters that min RMSE of the prediction model.Sampling units are divided in into 5 non-overlapping folds (different from those used for the DML procedure), each fold is used for tuning. The optimal hyperparameters are passed in the DML routine and used for learning.
    \item \href{https://mlr3book.mlr-org.com/chapters/chapter4/hyperparameter_optimization.html}{explanation}
    \item measure: Named list containing the measures used for parameter tuning. The default measures are \texttt{regr.mse} for continuous outcome variables and \texttt{classif.ce} for binary outcomes.
    \item resolution:  The key passed to the respective dictionary to specify  the tuning algorithm.
\end{itemize}


\begin{figure}[ht!]
    \caption{Hyperparameter Optimization}
    \label{fig:tuning}
    \centering
    \subfloat{\includegraphics[scale=.8]{figs/tuning_algorithm.png}}
    \vspace{-1mm}
    \begin{minipage}{.9\linewidth}
    \vspace{-1mm}
    \emph{Note: The diagram illustrates the hyperparameter optimization loop in \texttt{mlr3tuning.} Blue rectangles: Hyperparameter optimization loop. Purple rectangles: Objects of the tuning instance supplied by the user. Mint green rectangles: Internally created objects of the tuning instance. Green rectangle: Optimization Algorithm. Source: \href{https://mlr3book.mlr-org.com/chapters/chapter4/hyperparameter_optimization.html\#fig-optimization-loop-basic}{Applied Machine Learning Using mlr3 in R - 4  Hyperparameter Optimization}
    }
    \end{minipage}
\end{figure}


==> 999_wg_fd_ransformations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The WG and FD Transformations}\label{sec:exact}
Two alternative approaches are based on transforming the data. %This can be done by either removing the individual means from the original realisation (the WG transformation), or subtracting the realisation in $t-1$ from the value in $t$ (the FD transformation). 
%\begin{prop}\label{prop:transformation}
%    Suppose that the data generating process $\mathcal{P}$ satisfies \ref{item:asm_feedback}-\mbox{\ref{item:asm_additive}} so that model \eqref{eqn:plr2_y}-\eqref{eqn:plr2_v} holds. 
Let $\wit$ %$\{: t=1,\dots,T\}_{i=1}^N$% 
be a generic random variable and $Q$ a panel data transformation operator such that $Q(\wit)=Q_t(\wi)$ is a function of the random variable at wave $t$ and the remaining realisations for individual $i$. We consider two such transformations:\ the WG (within-group), or time-demeaning, transformation $Q({w}_{it})=\wit-\overline{w}_{it}$, where  $\overline{w}_{i}= T\inv \sum_{t=1}^T \wit$; %for all $T=1,\dots,T$; 
and the FD (first-difference) transformation $Q({w}_{it}) = \wit-w_{it-1}$ for $t=2,...,T$. Applying $Q$ to the model equations~\eqref{eqn:plr2_y}-\eqref{eqn:plr2_v} gives
\begin{align}
   & Q(\yit) = Q(\vit)\theta_0 + Q\big({l}_1(\xit)\big) + Q(\uit) \label{eqn:Q_y} \\
   & Q(\vit) = Q(\dit) - Q\big({m}_1(\xit)\big), \label{eqn:Q_d}
\end{align}
\noindent that do not depend on the fixed effects $\alpha_i$ or $\gamma_i$, respectively, because $Q(\alpha_i)=Q(\gamma_i)=0$.

Learning the transformed nuisance functions $Q\big({l}_1(\xit)\big)$ and $ Q\big({m}_1(\xit)\big)$ is challenging due to the nonlinearity of $l_1$ and $m_1$. We will discuss the procedures we propose for doing this in Section~\ref{sec:nuisance}.
%We propose DML procedures to estimate $\theta_0$ below. 

%functions of $\Xii$, that is, $\xit$ and also $({\bf x}_{i1},...,{\bf x}_{it-1},{\bf x}_{it+1},...,{\bf x}_{iT}$), but not of the transformed inputs, $Q(\xit)$.

% \begin{coro}[\bf FD transformation]
% Consider the FD transformation  $Q(\yit) = \yit-\yitminus$ and the transformed model in Proposition \ref{prop:transformation}. Learning $l_1$ under \ref{item:asm_feedback}-\ref{item:asm_additive}, 
% \begin{equation*}
%     \E(\yit-\yitminus|\xit,\xitminus,\alpha_i)=\E(\yit|\xit,\alpha_i)-\E(\yitminus,\alpha_i) = l_1(\xit)-l_1(\xitminus),
% \end{equation*}
% \noindent which implies
% \begin{equation*}
%     \E(\yit-\yitminus|\xit,\xitminus)= l_1(\xit)-l_1(\xitminus) \equiv \Delta l_1(\xitminus,\xit),
% \end{equation*}
% \end{coro}
% \noindent so that $\Delta l_1(\xitminus,\xit)$ can be learnt using $\{\yit=\yitminus,\xitminus,\xit:t=1,\dots,T\}_{i=1}^N$. Likewise,
% \begin{equation*}
%     \E(\dit-\ditminus|\xit,\xitminus,\alpha_i)=\E(\dit|\xit,\alpha_i)-\E(\ditminus,\alpha_i) = m_1(\xit)-m_1(\xitminus),
% \end{equation*}
% \noindent gives
% \begin{equation*}
%     \E(\dit-\ditminus|\xit,\xitminus)= m_1(\xit)-m_1(\xitminus) \equiv \Delta m_1(\xitminus,\xit),
% \end{equation*}
% \noindent so that $\Delta m_1(\xitminus,\xit)$ can be learnt using $\{\dit-\ditminus,\xitminus,\xit:t=1,\dots,T\}_{i=1}^N$.

%The role of the individual heterogeneity term in ensuring no feedback to the predictors and removing any Markov dependence of the joint treatment-outcome process is crucial, as is \mbox{\ref{item:asm_additive}.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent {\bf Transformation approaches.}  Superficially, it appears that (\ref{eqn:Q_y})-(\ref{eqn:Q_d}) presents a straightforward learning problem.  For example, $\E(\yit-y_{it-1}|x_{it-1},\xit)=l_1(\xit)-l_1({\bf x}_{it-1})\equiv \Delta l_1({\bf x}_{it-1},\xit)$ and $\E(\dit-d_{it-1}|x_{it-1},\xit)=m_1(\xit)-m_1({\bf x}_{it-1})\equiv \Delta m_1({\bf x}_{it-1},\xit)$ under \ref{item:asm_feedback}-\ref{item:asm_additive}, but it is not possible to learn $\Delta l_1({\bf x}_{it-1},\xit)$ and $\Delta m_1({\bf x}_{it-1},\xit)$ from the sample data in the same way as $\tilde{l}_1$ and $\tilde{m}_1$ are in Lemma \ref{lemma:cre_dml}. %The solution lies in a linear subspace of in which the difference functions lie, but this linear substpace is 
Other approaches are required.

First, we consider learning based on the transformed data alone. Generally, $Q\big({l}_1(\xit)\big)\ne {l}_1\big(Q(\xit)\big)$ and $Q\big({m}_1(\xit)\big)\ne {m}_1\big(Q(\xit)\big)$ unless $l_1$ and $m_1$ are linear. This means a consistent estimator cannot be simply constructed from the transformed data. %  $l_1(\xit)=\xit{\bf l}_0$ and $m_1(\xit)=\xit{\bf m}_0$, %$\lo=\xit\blo$, $\mo=\xit\bmo$ and where both ${\bf l}_0$ and ${\bf m}_0$ are conformable vectors of regression coefficients but, g. 
However, we propose the following approximate estimators.

\begin{lemma}[\bf{Approximation}]\label{lemma:approx}
%Suppose the conditions of Proposition~\ref{prop:transformation} hold. 
Model (\ref{eqn:Q_y})-(\ref{eqn:Q_d}) can be approximated by
    \begin{align}
       & Q(\yit) \approx Q(\vit)\theta_0 + {l}_1\big(Q(\xit)\big) + Q(\uit) \label{eqn:aQ_y}\\
       & Q(\vit) \approx Q(\dit) - {m}_1\big(Q(\xit)\big), \label{eqn:aQ_v}
    \end{align}
    \noindent where $l_1$ and $m_1$ can be learnt from the transformed data $\{Q(\yit),Q(\xit): t=1,\dots,T\}_{i=1}^N$ and $\{Q(\dit),Q(\xit): t=1,\dots,T\}_{i=1}^N$ , respectively.
\end{lemma}

\noindent A discussion of this approximation is given in Appendix~\ref{sec:proof_lemma_approx} but ultimately its performance is something to be assessed empirically. 

Second, we consider the following {\em exact} estimator based on the same Mundlak model as Proposition \ref{prop:cre}:

\begin{lemma}[\bf{Exact}]\label{lemma:exact} 
{\bf (i)} Consider the first-difference transformation $Q(y_{it})=\yit-y_{it-1}$. Then under \ref{item:asm_feedback}-\ref{item:asm_additive}
\[
\E(\yit-y_{it-1} | {\bf x}_{it-1}, \xit)=l_1 (\xit)-l_1({\bf x}_{it-1}),
\]
and
\[
\E(\dit-d_{it-1} |{\bf x}_{it-1},\xit)=m_1(\xit)-m_1({\bf x}_{t-1}),
\]
so that $\Delta 1_1({\bf x}_{it-1},\xit)\equiv l_1 (\xit)-l_1({\bf x}_{it-1})$ can be learnt using $\{\yit-y_{it-1},{\bf x}_{it-1},\xit: t=2,…,T\}_{i=1}^N$ and $\Delta m_1({\bf x}_{it-1},\xit)\equiv m_1 (\xit)-m_1({\bf x}_{it-1})$ can be learnt using $\{\dit-d_{it-1},{\bf x}_{it-1},\xit: t=2,…,T\}_{i=1}^N$.  However, for the within-group transformation,
\[
\E(\yit-\bar{y}_i|X_i )=l_1(\xit) - \frac{1}{T}\sum_{s=1}^T l_1({\bf x}_{is}),
\]
and similarly for $\dit-\bar{d}_i$. The dimension of the learning problem is $T^2/2$ times greater than that of the first-difference transformation.

{\bf (ii)} An alternative approach to the within-group transformation is based on Proposition \ref{prop:cre}. Suppose the data generating process satisfyies $\Pcal(\alpha_i|\Xii)=\Pcal(\alpha_i|\bxi)$ so that Mundlak model (\ref{eqn:mundlak_model}) holds.  Then $\tl_1(\xit,\bxi)=l_1 (\xit)+\omega_0(\bxi)$ and $\tm_1(\xit,\bxi)=m_1(\xit)+\tau_0(\bxi)$ learnt from the sample data satisfy $Q\big(\tl_1(\xit,\bxi)\big)=Q\big(l_1(\xit)\big)$ and $Q(\tm_1(\xit,\bxi)\big)=Q\big(m_1(\xit)\big)$.
\end{lemma}
 
\noindent A proof is given in Appendix~\ref{sec:proof_lemma_exact}.
% A practicable approach, inspired by the linear case, is based on the approximations 
% \begin{align}
% Q\big({l}_1(\xit)\big)& = l\big(Q(\xit)\big) + \epsilon^{it}_l \approx l_1\big(Q(\xit)\big) \label{eqn:approx_l} \\
% Q\big({m}_1(\xit)\big) &= m\big(Q(\xit)\big) + \epsilon^{it}_m \approx m_1\big(Q(\xit)\big), \label{eqn:approx_m}
% \end{align}
% \noindent because $l_1$ and $m_1$ are functions of the original variables $\xit$ and not their transformations.

% Learning the nuisance parameters $l_1\big(Q(\xit)\big)$ and $m_1\big(Q(\xit)\big)$ from the transformed sample data $\{Q(\yit),Q(\dit),Q(\xit)\}_{t=1}^T$ requires that the approximation errors $\epsilon^{it}_l=\epsilon_l(\xit)$ and $\epsilon^{it}_m=\epsilon_m(\xit)$ are small. This is the case if the true functions are linear or the approximation is accurate over regions of the predictors with the strongest support.\footnote{The existence of such a function is easily justified:\ a first-order Taylor series expansion of $l_0$ around some fixed value $\x$ gives $l_0(\xit)=(\xit-\x)\dot{l}_0(\x)+\mathcal{O}(\|\xit-\x\|^2)$, where $\|.\|$ is the $L_1$-norm and column-vector $\dot{l}_0(\x)$ is the partial derivative of $l_0$ with respect to $\xit$ evaluated at $\x$, so that $\widetilde{l}_0(\xit)=\widetilde{\bf{x}}_{it}\dot{l}_0(\x)+\mathcal{O}(\|\mathbf{b}_x\|^2)$, where $\mathbf{b}_x=\rm{sup}\|\xit-\x\|$. Hence, there is some $\txit\dot{l}_{0}(\x)+\mathcal{O}\big(\|\mathbf{b}\|^2\big)\approx \txit\dot{l}_{0}(\x)$ minimizing some loss function, where $\widebar{\mathbf{b}}=\inf_{\x}\mathbf{b}_{\x}$ and $\widebar{\x}=\arginf_{\x}\mathbf{b}_{\x}$ are respectively the smallest bound over the bounded support of all possible $\x$-centred confounders, and $\widebar{\x}$ any value obtaining this bound.} When $l_1$ and $m_1$ are nonlinear, however, standard learning becomes more difficult because both functions depend on $\Xii$. In this case, the \emph{exact} (or \emph{hybrid}) approach below should be preferred.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% {\bf Exact (hybrid) approach for WG and FD transformations.} The possibility of the approximations \eqref{eqn:approx_l}-\eqref{eqn:approx_m} performing poorly motivates an alternative \emph{exact} approach (or the \emph{hybrid} approach because it incorporates the CRE approach) to learn $l_1(\xit,\bxi)$ and $m_1(\xit,\bxi)$.

% % lemma 2: wg/fd
% \begin{coro}
% Suppose that Lemma \ref{lemma:cre_dml} holds. Let $Q$ be the operator for the time-demeaning or first-difference transformation, where the WG transformation of a generic random variable $\{w_{it}\}_{t=1}^T$ is  $Q({w}_{it})=w_{it}- T\inv \sum_{t=1}^T w_{it}$ for all $t=1,\dots,T$, and the FD transformation is $Q({w}_{it}) = w_{it}-w_{it-1}$ for $T\ge2$. Then, the transformed predictions of the nuisance parameters are calculated as $Q\Big(\widehat{l_1(\xit,\bxi)}\Big)$ and $Q\Big(\widehat{m_1(\xit,\bxi)}\Big)$.

% % Then, the quasi-oracle estimating equations from the transformed sample data are
% % \begin{align}
% %     Q(\yit) &=  Q(\dit)\theta_0  +   Q\Big(\widehat{l_1(\xit,\bxi)}\Big) +  Q(\uit)\\
% %     Q(\dit) &=  Q\Big(\widehat{m_1(\xit,\bxi)}\Big) +  Q(\vit),
% % \end{align}
% % \noindent from which inferences about $\theta_0$ can be made.
% \end{coro}

==> asm.tex <==
\subsection{Regularity conditions}
\begin{enumerate}
\item $\E[\yit(0)| \xit, \alpha] = l^*_0(\xit,\alpha)$ is an additively separable function s.t. $l^*_0(\xit, \alpha) = l_0(\xit) + \alpha$

\item $m^*_0(\xit,\alpha^*)$ is additively separable such that $m^*_0(\xit,\alpha^*) = m_0(\xit) + \alpha^*$ (where $\alpha$ and $\alpha^*$ are correlated). $m_0(\xit)\ne 0$ which makes the non-orthogonal estimator biased due to omitted variable bias.

\item The treatment effect is homogeneous such that $\E[\yit(1) - \yit(0) | \xit, \alpha] = \theta_0$

\item $(\xit, \alpha)$ controls for confounding and residual $E(\uit|\dit, \xit, \alpha) = 0$

\item $\{\dit, \xit\}$ is strictly exogenous
\end{enumerate}
You may note that the WG transformation imposes the constraint that $g_0$ (or $l_0$) and $m_0$ in the implied WG model sums to 0 across the T waves for each individual.  Have we imposed this for CART/REF (not needed for ols/Lasso)?  (The implied $g_0$ is $g_0(\xit) - \sum_{s=1}^T[ g_0(x_s)] / T$, etc.)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASM2
\begin{enumerate}[label=\sc{assumption}{ \arabic*}, leftmargin=1.65\parindent,  rightmargin=.5\parindent]
\item (\emph{Expectations}):\label{item:disturbances}
    \begin{enumerate}[label={\roman*})]
    \item (\emph{Strong exogeneity}): $\E\bigl(\tuit|\tdit, \txit\bigr)=0$, and $\E\bigl(\tvit|\txit\bigr)=0$ \label{item:exogeneity}
    \item {(\em Independence)}: $\E\bigl(\tuit, \tvit\bigr)=0$  \label{item:indep}
    \item  {(\em Auto-correlation)}: $\E(\tuit\tuis)\neq 0$, and $\E(\tvit\tvis)\neq 0$ for some or all pairs $t\neq s$ \label{item:autocorr}
    \end{enumerate}
\end{enumerate}
Strong exogeneity of the transformed variables guarantees that exogeneity is preserved after any transformation to remove the fixed effects \citep[p.707]{cameron2005}. In addition, it rules out feedback effects and implies contemporaneous exogeneity.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASM3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASM2
\begin{enumerate}[label=\sc{assumption}{ \arabic*}, leftmargin=1.65\parindent,  rightmargin=.5\parindent]
\setcounter{enumi}{1}
\item (\emph{Sparsity condition}): 
\begin{enumerate}[label={\roman*})]\label{item:sparsity}	    
    \item (\emph{Coefficients}): $\|\bbeta\|_0 = \sum_{j=1}^K\one\{\bj \ne0\} \le s<K$, \\
    such that $\bbeta{}^{(1)} = \Big(\bbeta_{1}^{(1)}, \dots, \bbeta_{k_0}^{(1)}\Big)'$ is a vector of non-zero parameters of order $k_0$, where $k_0\in[1,K)$ \label{item:coeffs}
\item (\emph{Set}):  $\Bn = \{j\in \{1,\dots, K\}, \bj \ne0\}$ is the set of non-zero coefficients\label{item:set}
    %therefore the non-zero components converge to (looka at page 1.a of notes)
    \end{enumerate}	
\end{enumerate}	
The assumption guarantees that there are at most $s$ non-zero coefficients, and the others are zero. The restricted eigenvector condition is not required because $k\ll N$.\footnote{The restricted eigenvector condition guarantees the invertibility of $\Cxn$ in high-dimensional settings by restricting all square sub-matrices of dimension no larger than $s$ to have a positive minimal eigenvalue.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASM4
\begin{enumerate}[label=\sc{assumption}{ \arabic*}, leftmargin=1.65\parindent,  rightmargin=.5\parindent]
\setcounter{enumi}{2}
\item (\emph{Rank conditions}): 
\begin{enumerate}[label={\roman*})]\label{item:rank}
       \item  $\Cxn \equiv N\inv \sum_{i=1}^N \Xii'\Xii \overset{p}{\to}\Cx<\infty$ is a finite positive-definite  symmetric block matrix with column rank $k$ such that
       \begin{equation*}
        \Cx = ((c_{ij})) = %
        \begin{pmatrix}
        \Cij{11}&\Cij{12}\\
        \Cij{21}&\Cij{22}\\       
        \end{pmatrix}   
        \end{equation*}
        where $\Cij{12} = \big\{ ((c_{ij})), i\in\{1,\dots,k_0\}, j\in\{(k_0+1),\dots,K\}\big\}$, and $\Cx\inv = ((c^{ij}))$
        \label{item:rank_x}
        \item  $\Cdn \equiv N\inv \sum_{i=1}^N \Dii'\Dii \overset{p}{\to}\Cd<\infty$ \label{item:rank_d}     
	\end{enumerate}	
\end{enumerate}	
These define the rank conditions for $\{\Xii, \Dii\}$, implying non-singularity of the matrices $\Cx$ and $\Cd$, hence, no perfect multicollinearity that guarantees the invertibility of the matrix \red{[ML context with few regressors but many that are zero]}. 

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASM5
 \begin{enumerate}[label=\sc{assumption}{ \arabic*}, leftmargin=1.65\parindent,  rightmargin=.5\parindent]
\setcounter{enumi}{3}
\item (\emph{Moment conditions}):  \label{item:mom} %%
 	\begin{enumerate}[label={\roman*})]		
        % \item  $\E\big\|\Xii\big\|^r<\infty$ for some $r>0$ $\Xii\in \mathbb{R}^{p\times p}$; $\underset{i+1,\dots,N}{\max\|\Xii\|_{\infty}\le M_x}$ almost surely \label{item:mom_x} 	
        % \item  $\E\big\|\Dii\big\|^r<\infty$ for some $r>0$ $\Dii\in \mathbb{R}^{T}$; $\underset{i+1,\dots,N}{\max\|\Dii\|_{\infty}\le M_d}$ almost surely  \label{item:mom_d} 	
        \item $\E\big\|\tui\big\|^r<\infty$ for some $r>0$, where $\E\big\|\tui\big\|=0$ and  $\E\big\|\tui\big\|^2=\sigma^2_u$ \label{item:mom_u} 	
        \item $\E\big\|\tvi\big\|^r<\infty$ for some $r>0$, where $\E\big\|\tvi\big\|=0$ and  $\E\big\|\tvi\big\|^2=\sigma^2_v$ \label{item:mom_v} 	
        % \item  $\mathrm{sup}_{i}\,\E\big\|\Xii' \tvi\big\|^{2+r}<\infty$ for some $r>0$, $\forall i$ and $\Xii' \tvi \in \mathbb{R}^p$
        % \item  $\mathrm{sup}_{i}\,\E\big\|\Dii' \tui\big\|^{2+r}<\infty$ for some $r>0$, $\forall i$ and $\Dii' \tui \in \mathbb{R}^p$ \label{item:mom_Adistr}	%uniform mom bound
	\end{enumerate}	
\end{enumerate}
This defines the finiteness and boundedness of moments in terms of the Euclidean norm. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ASM6
 \begin{enumerate}[label=\sc{assumption}{ \arabic*}, leftmargin=1.65\parindent,  rightmargin=.5\parindent]
\setcounter{enumi}{4}
\item (\emph{Regularization parameter for Lasso}): \label{item:lambda}
 	\begin{enumerate}[label={\roman*})]		
            \item (\emph{Rate of convergence in the prediction norm}):
            \begin{equation*}
            \lambda_n \approx s\phi\inv\sqrt{\log K/(NT)}
            \end{equation*}
            \noindent where $\phi\in(0,1]$ is a measure of correlation between covariates with non-zero coefficients and those with zero-coefficients \citep[as in][]{wainwright2009}. \label{item:approx}
            \item  (\emph{Convergence}): 
            \begin{equation*}
            \frac{\lambda_n}{N} \to \mathrm{a}\in(0,\infty)
            \end{equation*}
            \item (\emph{Growth Condition}): 
            \begin{equation*}
                \frac{s \log K}{\sqrt{N}}\to 0
            \end{equation*}
    \item (\emph{Concentration bound})
    \begin{equation*}
    \Bb \frac{1}{\sqrt{N}} \sum_i \Dii'\Xii\Bb_{\infty} \lesssim \sqrt{\log K}
    \end{equation*}
    \noindent where $a_n \lesssim b_n$ if $a_n \le C b_n$ for some constant $C$ that is independent of $N$.
    \end{enumerate}
\end{enumerate}
\ref{item:lambda} are required for \textsc{lasso}. The regularisation parameter is a function of the cross-sectional sample size $N$. LASSO theory requires that $\lambda_n$ exceeds a certain threshold, which depends on the standard deviations of the noise and the covariates. [See \textsc{thm 2.2} in \cite{chatterjee2011} for convergenge of $\bhat$ under different assumptions].

\red{Assume that $\eta_0$ can be estimated using a sub-set of the data $\mathcal{W}$. Following  \cite{chernozhukov2018} we need to clarify the assumptions we need to estimate $\eta_0$ -- i.e., approximate sparsity for lasso, well-approximability for trees and RF.}






==> cre.tex <==
%$\bdit = T\inv \sum_t\dit$;  $l_2(\bxi)= l_2\big(T\inv \sum_t\xit\big)$;  $m_2(\bxi)= m_2\big(T\inv \sum_t\xit\big)$;

Plugging \eqref{eqn:alpha_i} in \eqref{eqn:outcome} and \eqref{eqn:delta_i} in \eqref{eqn:treatment}, we get the partially linear model with correlated random effects as follows
\begin{align}
& \yit = \theta d_{it}  + \pi \overline{d_i}+ l(\xit, \bxi) + r_{it} \label{eqn:outcome_cre}\\
& \dit = m(\xit, \bxi)+  \zeta_{it} \label{eqn:treatment_cre}
\end{align}
\noindent where $\bdit = T\inv \sum_t\dit$; $l(\xit, \bxi)= l_1(\xit)+ l_2(\bxi)$; $m(\xit, \bxi) = m_1(\xit) +  m_2(\bxi)$; $r_{it}= a_i + e_{it}$ and  $\zeta_{it}= \xi_i + \nu_{it}$ are the error terms. $\theta$ is the parameter of interest with causal interpretation that is homogeneous across individuals $i=1,...,n$ and/or and time $t=1,...,T$ \red{(we will relax this assumption further on)}; $\pi$ is the difference of the between and within coefficients. The error terms in both equations are allowed to be {\em auto-correlated} such that $\E(\epsilon_{it}\epsilon_{is})\neq 0$ for some or all pairs $t\neq s$. \red{[Paul's notes on error terms]}


Identification is based \red{(for now)} on the conditional moment restriction
$\E(\epsilon_{it}| \dit, \xit)=0$, or $\E(\epsilon_{it}| \dit, \xit)=\E(\epsilon_{it} | \xit)$, for all $i,t$. Note that, if $\E(\epsilon_{it}| \dit, \xit)\ne 0$ but $\E(\epsilon_{it}| \dit, \xit, \alpha_i)=0$, where $\alpha_i$ is the individual effect in the decomposition $\epsilon_{it} = e_{it} + \alpha_i$, we could expand $\xit$ to include individual-mean predictors as per \emph{Mundlak}.

%Note also that (\ref{eqn:outcome}-\ref{eqn:treat}) does not define a model to be jointly estimated.  Any consistent estimating equation for $\theta_0$ must be based on (\ref{eqn:outcome}) and its identifying conditional moment restriction. In contrast, the inclusion of (\ref{eqn:treat}) is optional but desirable:\ it enables us to construct an estimating equation that is both locally efficient and Neyman orthogonal.

\section{Algorithm}
\noindent We proceed as follows:
\begin{enumerate}
    \item Estimate $l(\xit, \bxi)$ and $m(\xit, \bxi)$ on a set of time-varying covariates (set OLS/Lasso as default for $l_2(.)$ and $m_2(.)$);
    \item Save $\widehat{l}(\xit, \bxi)$ and $\widehat{m}(\xit, \bxi)$ for the ``Partialling-out'' score \red{(add the choice for a non-orthogonal score function in the package)}; 
    \item Plug the estimated functions in the panel version of the score function of $\dit$  below: 
    \begin{equation}
     \psi(.) =  \underbrace{- \dit \big(\dit-\widehat{m}(.)\big)}_{\equiv \psi_a}\theta + \underbrace{\big(\yit- \pi\overline{d_i}-\widehat{l}(.)\big) \big(\dit-\widehat{m}(.)\big)}_{\equiv\psi_b}\label{eqn:score_theta}
    \end{equation}
   \item Estimate $(\pi, \theta)$ simultaneously using the algorithm below (in the box).
\end{enumerate}
\vspace{5mm}

\fbox{\begin{minipage}{14.5cm}
\noindent \textbf{Algorithm for estimating} $(\bm\pi, \bm\theta)$:
\begin{enumerate}
    \item Start with iteration $p = 0$.
    \item For each $p$ iterate through the following steps until convergence of $\widehat{\pi}$ and $\widehat{\theta}$:
    \begin{enumerate}[label={\roman*}.]
        \item Initialise ${\pi}^{(p)}=0$ and ${\theta}^{(p)}=0$.
        \item Estimate $\widehat{\pi}^{(p)}$ from the (non-orthogonal) score function
            \begin{equation}\label{eqn:score_phi}
                \dot{\psi}^{(p)} = - \overline{d}_i^2 \pi^{(p)} + \overline{d}_i(\yit - \dit\theta^{(p)} - \widehat{l}(.))
            \end{equation}
        such that $\widehat{\pi}^{(p)}= -\E[\overline{d}_i(\yit - \dit\theta^{(p)} - \widehat{l}(.))]/\E[\overline{d}_i^2]$.
        \item Estimate initial $\theta^{(p)}$ using the score function for panel data, $\psi^{(p)}$, as defined in Equation~\eqref{eqn:score_theta} with $\widehat{m}(.)$, $\widehat{l}(.)$, and $\widehat{\pi}^{(p)}$.
        
        \item Stop when  $|\widehat{\pi}^{(p)}-\widehat{\pi}^{(p-1)}|\approx0$  \textbf{and} $|\widehat{\theta}^{(p)}-\widehat{\theta}^{(p-1)}|\approx0$ otherwise move to next iteration $p+1$ until convergence is achieved.
    \end{enumerate}
\end{enumerate}
\end{minipage}}


==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> model.tex <==
\section{Model and Assumptions}
\subsection{Model}
Let $\{\yit,\xit,\dit\}$ be a sequence of independent and identically distributed (\emph{iid}) random variables for all units $\, i = 1, \dots, N$ and time periods $t=1,\dots,T$, where $\yit$ is a scalar outcome, $\xit$ is a vector of high-dimensional predetermined variables of order $K$, and $\dit$ is the treatment or policy variable. Assume $K\ll N$ and $T$ is fixed.                                                                                                              

Consider a revisited version of \cite{chernozhukov2018}'s  partial linear regression model (PLRM) with repeated measures of form
%known as \cite{robinson1988}'s model.\footnote{\red{In Semenova et al. (2021) the model is extended a partially linear sequentially exogenous dynamic panel model.}}
\begin{align}
& \yit = \theta d_{it}  + h_0(\xit) + \alpha_i + \uit \label{eqn:outcome}\\
& \dit = %
%\begin{cases}
    %m_0(\xit)+ \delta_i + \vit & \text{ if continuous}  \\
\one\big[m_0(\xit)+ \delta_i + \vit>0\big]  \label{eqn:treat} %& \text{ if binary} \\ 
%\end{cases}
\end{align}
\noindent where $ h_0(\xit)$ and $m_0(\xit)$ are unknown \red{(possibly nonlinear)} nuisance functions, $\alpha_i$ and $\delta_i$ are unit-specific effects, and $\uit$ and $\vit$ are \emph{iid} disturbances. The parameter of interest, $\theta$, has causal interpretation and is homogeneous across individuals $i=1,...,N$ and time period $t=1,...,T$.\footnote{In future research, we will allow $\theta$ to be heterogeneous across individuals and/or time.} The model can easily accommodate continuous variables by adapting Equation~\eqref{eqn:treat}. For the sake of exposition, we present a binary case.

A common estimation practice with models with fixed effects consists in eliminating the
time-invariant components by applying a monotonic transformation to the original model  -- i.e., the \emph{within-group} (WG) transformation, or \emph{first-differences} (FD). Define a transformation operator $Q \equiv  1-T\inv \sum_t$ for WG transformation, and $Q \equiv \Delta_t$ for FD transformation. After applying the transformation to the original model, the model becomes
%%%%%%%%%%%%%%%
\begin{align}
& \tyit = \theta \tdit  + h_0(\txit) + \tuit \label{eqn:outcome_fe}\\
& \tdit = m_0(\txit)+  \tvit \label{eqn:treatment_fe}
\end{align}
%%%%%%%%%%%%%%%
\noindent where $\tyit = Q\yit$; $\tdit = Q\dit$; $\txit = Q\xit$; $\tuit = Q\uit$; and $\tvit = Q\vit$.\footnote{Abinary treatment $\dit$ becomes a discrete random variable $\tdit$ once transformed. The transformed variable ranges between $\pm1$ with zero included (if there is no change in the treatment status)  after the FD transformation, and between 0 and 1 included (indicating never/always treated) after the WG transformation.}  

Inference on the population parameter $\theta$ is usually conducted by estimating model~\eqref{eqn:outcome_fe} by OLS. This is the conventional WG or FD estimator, based on the choice of the transformation $Q$. Alternatively, the method of moments (MOM) estimator of $\theta$ is the debiased WG or FD estimator that solves the finite-sample analog of the moment conditions, as explained in Section~\ref{sec:estimation}. The nuisance parameters $\eta_0 = (h_0, m_0)$ can be estimated via OLS or ML tools (e.g., penalised regression, tree-based approaches, etc.).

%An appealing method for estimating sparse high-dimensional linear models is the Lasso. Lasso estimates regression coefficients by minimizing a least-squares objective plus an l-1 penalty term.



%For simplicity, let $ l_0(\txit)= \txit'\bbeta$, and $m_0(\txit)=\txit'\bdelta$.
% By stacking the variables over time, the model can be expressed in matrix form as
% \begin{align}
% & \Yii = \Dii\theta + \Xii\bbeta + \tui \label{eqn:out}\\
% & \Dii = \Xii\bdelta + \tvi \label{eqn:treat}
% \end{align}

%Identification is based on the conditional moment restriction $\E(\epsilon_{it}| \dit, \xit)=0$, or $\E(\epsilon_{it}| \dit, \xit)=\E(\epsilon_{it} | \xit)$, for all $i,t$. Note that, if $\E(\epsilon_{it}| \dit, \xit)\ne 0$ but $\E(\epsilon_{it}| \dit, \xit, \alpha_i)=0$, where $\alpha_i$ is the individual effect in the decomposition $\epsilon_{it} = e_{it} + \alpha_i$, we could expand $\xit$ to include individual-mean predictors as per \emph{Mundlak}.

%Note also that (\ref{eqn:outcome}-\ref{eqn:treat}) does not define a model to be jointly estimated.  Any consistent estimating equation for $\theta_0$ must be based on (\ref{eqn:outcome}) and its identifying conditional moment restriction. In contrast, the inclusion of (\ref{eqn:treat}) is optional but desirable:\ it enables us to construct an estimating equation that is both locally efficient and Neyman orthogonal.

==> preamble_pack.tex <==
%change margins in portion of text
%\usepackage{scrextend}

\usepackage[T1]{fontenc}
\usepackage [english]{babel}
\usepackage{natbib} %Serve per la bibliografia
%\usepackage[backend=biber]{biblatex}
\usepackage{authblk}%author w/affiliation

\usepackage{amsmath,amssymb}
\usepackage{mathabx}
\usepackage{tabularx}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{mathtools} %to be used to define =^H
\usepackage{bm}%bold greek letters
\usepackage{dsfont}%indicator operator
\usepackage{bbm}%indicator operator

\usepackage{amsmath,amsthm,amssymb}
\usepackage{amscd}
%\usepackage{enumitem}
\usepackage[inline]{enumitem}%easy to customize than \enumerate

\usepackage{multirow}
%\usepackage{graphicx}
\usepackage{graphicx,graphics,rotating}
\usepackage[graphicx]{realboxes} %rotate tables
\usepackage{epstopdf} % for eps files
\usepackage[font=scriptsize,labelfont=bf,labelsep=period,textfont=it]{caption}

\usepackage{mathrsfs}
\usepackage[a4paper,top=2.5cm,bottom=2.5cm,left=2cm,right=2cm,height rounded,bindingoffset=0.5cm]{geometry}
%\usepackage{floatpag}	%remove page number with \thisfloatpagestyle{empty} 

\usepackage{etoolbox}
\usepackage{xpatch}  
\usepackage[gen]{eurosym}
\usepackage{lscape}
%\usepackage[titletoc,toc,page]{appendix}
\usepackage[title,titletoc]{appendix}

\usepackage{sgame}
%\usepackage{pgfplots}
\setlength{\parindent}{10ex}
\linespread{2}
\usepackage{setspace}
\usepackage[font={small,sl}]{caption}
\usepackage{booktabs,caption} %to be used w/ \captionsetup
%\usepackage[margin=.5cm]{caption} %caption width
%\usepackage{longtable}
\usepackage[para,online,flushleft]{threeparttable}	%to align notes under table


\usepackage{blindtext}
\usepackage{fancyhdr}
\usepackage{setspace}
\usepackage[explicit]{titlesec}
\usepackage[normalem]{ulem}
\usepackage{lipsum}
\usepackage{mwe}  
\usepackage{verbatim}
\usepackage{booktabs,array}  
\usepackage{listings}
\usepackage{subfig}
%\usepackage{hyperref}
\usepackage[colorlinks=true,citecolor=blue,linkcolor = blue,urlcolor  = blue]{hyperref}
\usepackage{xcolor}
\usepackage{amssymb}


%\usepackage{apacite} %must be loaded after hyperref
%\usepackage[symbol]{footmisc}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\usepackage{booktabs}
\usepackage[hang,flushmargin]{footmisc}
\newtheorem{theorem}{Theorem}

\pdfminorversion=6  %raise pdf version to 1.6


==> preamble_pack_EctJ.tex <==
\usepackage [english]{babel}
\usepackage{natbib} %Serve per la bibliografia

\usepackage{amsmath,amssymb}
\usepackage{mathabx}
\usepackage{tabularx}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{mathtools} %to be used to define =^H
\usepackage{bm}%bold greek letters
\usepackage{dsfont}%indicator operator
\usepackage{bbm}%indicator operator

\usepackage{amsmath,amsthm,amssymb}
\usepackage{amscd}
%\usepackage{enumitem}
\usepackage[inline]{enumitem}%easy to customize than \enumerate

\usepackage{multirow}
\usepackage{graphicx,graphics,rotating}
\usepackage[graphicx]{realboxes} %rotate tables
\usepackage{epstopdf} % for eps files

\usepackage{mathrsfs}

\usepackage{etoolbox}
\usepackage{xpatch}  
\usepackage[gen]{eurosym}
\usepackage{lscape}
%\usepackage[title,titletoc]{appendix}

\usepackage{sgame}
\usepackage[para,online,flushleft]{threeparttable}	%to align notes under table


\usepackage{blindtext}
\usepackage{setspace}
%\usepackage[explicit]{titlesec}
\usepackage[normalem]{ulem}
\usepackage{lipsum}
\usepackage{mwe}  
\usepackage{verbatim}
\usepackage{booktabs,array}  
\usepackage{listings}
\usepackage{subfig}
\usepackage[colorlinks=true,citecolor=blue,linkcolor = blue,urlcolor  = blue]{hyperref}
\usepackage{xcolor}
\usepackage{amssymb}

\usepackage{booktabs}
\usepackage[hang,flushmargin]{footmisc}

\pdfminorversion=6  %raise pdf version to 1.6

\input{new_commands}
\def\citeapos#1{\citeauthor{#1}'s (\citeyear{#1})}%\citeapos

\makeatletter
\newcommand{\distas}[1]{\mathbin{\overset{#1}{\kern\z@\sim}}}%
\newsavebox{\mybox}\newsavebox{\mysim}
\newcommand{\distras}[1]{%
  \savebox{\mybox}{\hbox{\kern3pt$\scriptstyle#1$\kern3pt}}%
  \savebox{\mysim}{\hbox{$\sim$}}%
  \mathbin{\overset{#1}{\kern\z@\resizebox{\wd\mybox}{\ht\mysim}{$\sim$}}}%
}

%widebreve
\def\widebreve{\mathpalette\wide@breve}
\def\wide@breve#1#2{\sbox\z@{$#1#2$}%
     \mathop{\vbox{\m@th\ialign{##\crcr
\kern0.08em\brevefill#1{0.8\wd\z@}\crcr\noalign{\nointerlineskip}%
                    $\hss#1#2\hss$\crcr}}}\limits}
\def\brevefill#1#2{$\m@th\sbox\tw@{$#1($}%
  \hss\resizebox{#2}{\wd\tw@}{\rotatebox[origin=c]{90}{\upshape(}}\hss$}

==> preamble_pack_JBES.tex <==
%change margins in portion of text
%\usepackage{scrextend}

%\usepackage[T1]{fontenc}
\usepackage [english]{babel}
\usepackage{natbib} %Serve per la bibliografia
%\usepackage[backend=biber]{biblatex}
%\usepackage{authblk}%author w/affiliation

\usepackage{amsmath,amssymb}
\usepackage{mathabx}
\usepackage{tabularx}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{mathtools} %to be used to define =^H
\usepackage{bm}%bold greek letters
\usepackage{dsfont}%indicator operator
\usepackage{bbm}%indicator operator

\usepackage{amsmath,amsthm,amssymb}
\usepackage{amscd}
%\usepackage{enumitem}
\usepackage[inline]{enumitem}%easy to customize than \enumerate

\usepackage{multirow}
%\usepackage{graphicx}
\usepackage{graphicx,graphics,rotating}
\usepackage[graphicx]{realboxes} %rotate tables
\usepackage{epstopdf} % for eps files
%\usepackage[font=scriptsize,labelfont=bf,labelsep=period,textfont=it]{caption}

\usepackage{mathrsfs}
%\usepackage[a4paper,top=2.5cm,bottom=2.5cm,left=2cm,right=2cm,height rounded,bindingoffset=0.5cm]{geometry}
%\usepackage{floatpag}	%remove page number with \thisfloatpagestyle{empty} 

\usepackage{etoolbox}
\usepackage{xpatch}  
\usepackage[gen]{eurosym}
\usepackage{lscape}
%\usepackage[titletoc,toc,page]{appendix}
\usepackage[title,titletoc]{appendix}

\usepackage{sgame}
%\usepackage{pgfplots}
%\setlength{\parindent}{10ex}
%\linespread{2}
%\usepackage{setspace}
%\usepackage[font={small,sl}]{caption}
%\usepackage{booktabs,caption} %to be used w/ \captionsetup
%\usepackage[margin=.5cm]{caption} %caption width
%\usepackage{longtable}
\usepackage[para,online,flushleft]{threeparttable}	%to align notes under table


\usepackage{blindtext}
%\usepackage{fancyhdr}
\usepackage{setspace}
\usepackage[explicit]{titlesec}
\usepackage[normalem]{ulem}
\usepackage{lipsum}
\usepackage{mwe}  
\usepackage{verbatim}
\usepackage{booktabs,array}  
\usepackage{listings}
\usepackage{subfig}
%\usepackage{hyperref}
\usepackage[colorlinks=true,citecolor=blue,linkcolor = blue,urlcolor  = blue]{hyperref}
\usepackage{xcolor}
\usepackage{amssymb}


%\usepackage{apacite} %must be loaded after hyperref
%\usepackage[symbol]{footmisc}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\usepackage{booktabs}
\usepackage[hang,flushmargin]{footmisc}
\newtheorem{theorem}{Theorem}

\pdfminorversion=6  %raise pdf version to 1.6

%\usepackage{mathptmx}
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{coro}{Corollary}[prop]

\input{new_commands}
\def\citeapos#1{\citeauthor{#1}'s (\citeyear{#1})}%\citeapos


\makeatletter
\newcommand{\distas}[1]{\mathbin{\overset{#1}{\kern\z@\sim}}}%
\newsavebox{\mybox}\newsavebox{\mysim}
\newcommand{\distras}[1]{%
  \savebox{\mybox}{\hbox{\kern3pt$\scriptstyle#1$\kern3pt}}%
  \savebox{\mysim}{\hbox{$\sim$}}%
  \mathbin{\overset{#1}{\kern\z@\resizebox{\wd\mybox}{\ht\mysim}{$\sim$}}}%
}

%widebreve
\def\widebreve{\mathpalette\wide@breve}
\def\wide@breve#1#2{\sbox\z@{$#1#2$}%
     \mathop{\vbox{\m@th\ialign{##\crcr
\kern0.08em\brevefill#1{0.8\wd\z@}\crcr\noalign{\nointerlineskip}%
                    $\hss#1#2\hss$\crcr}}}\limits}
\def\brevefill#1#2{$\m@th\sbox\tw@{$#1($}%
  \hss\resizebox{#2}{\wd\tw@}{\rotatebox[origin=c]{90}{\upshape(}}\hss$}

==> reem.tex <==
\section{RE-EM algorithm}
\blue{Sela and Simonoff's (2012)} generalize the linear mixed effects model to tree-based models. A general effects model with additive errors is as follows:
\begin{equation}
y_{it} = Z_{it} \bi + f(\xit) +\epsilon_{it}
\end{equation}
\noindent where $\epsilon\distas{}{} N(0,R_i)$, and $\bi\distas{}{} N(0,\Dmat)$.

The attributes, $\x$, may be constant over time, constant across objects, or varying across time and objects. To account for the differences between objects across time periods, we include a known design matrix, $Z_{it}$, which may vary each period and depend on the attributes, and a vector of unknown time-constant, object-specific effects, $\bi$.\\ 

\noindent \textbf{Algorithm for the estimation of a RE-EM Tree:}

\begin{enumerate}
    \item Initialize the estimated random effects, $\bhat_i$, to zero.
    \item Iterate through the following steps until the estimated random effects, $\bhat_i$, converge (based
on change in the likelihood or restricted likelihood function being less than some tolerance value): 
    \begin{enumerate}[(a)]
        \item  Estimate a regression tree approximating $f(.)$, based on the target variable, \mbox{$y_{it} - Z_{it}\bhat_i$}, and attributes, $\x = (x_{it1},\dots,x_{itK})$, for $i = 1,\dots,I$ and $t = 1,\dots,T_i$. Use this regression tree to create a set of indicator variables, $\one(\x \in g_p)$, where $g_p$ ranges over all of the terminal nodes in the tree.
        \item  Fit the linear mixed effects model, $y_{it} = Z_{it}\bi +\one(\x \in g_p)\mu_p + \epsilon_{it}$. Extract $\bhat_i$ from the estimated model.
        \end{enumerate}
        \item Replace the predicted response at each terminal node of the tree with the estimated population level predicted response $\hat{\mu}_p$ from the linear mixed effects model fit in (2b).
\end{enumerate}

\noindent The fitting of the tree in Step (2a) can be achieved using any tree algorithm, based on any
tree growing and pruning rules that are desired. Tree building is based on the \textsc{R} function \texttt{rpart}, which is an implementation of the \textsc{CART} tree algorithm proposed in \blue{Breiman et al. (1984)}. However, using \textsc{CART} as the regression tree will lead to the algorithm being biased. \blue{Sela and Simonoff (2014)} propose to use the conditional inference trees of Hothorn et al. (2006) instead of \textsc{CART}  in Step (2a). Since the conditional inference tree is unbiased, this version of \textsc{RE-EM} Tree with \texttt{ctree} should also be unbiased, and they refer to them as ``unbiased RE-EM trees''.

The linear model with random effects in Step (2b) can be estimated using maximum likelihood or using restricted maximum likelihood (\textsc{REML}). In most of the results we present, we estimate the linear model with \textsc{REML}, because it yields unbiased estimates for the variance, $R_i$. Basing the algorithm on a linear model with random effects also allows us to account for autocorrelation of errors within objects using existing estimation methods for linear models (by allowing for non-diagonal $R_i$ in the model fitting), if necessary. Many statistical packages contain code to estimate linear mixed effects models; the \texttt{lme} function of the \texttt{Rnlme} package \blue{(Pinheiro et al., 2009)} is used here.

A useful property of tree algorithms is that they typically include automatic procedures to handle missing values in the attributes $\X$; for example, \texttt{rpart} uses surrogate split \blue{(Breiman et al. 1984)}. This results in the ability to produce estimated responses for objects with missing attribute values. This means that the \textsc{RE-EM} tree also can be fit when there are missing values in the attributes, since the tree fitting in Step 2a proceeds using (for example) surrogate split, while the estimating of $\bi$, $R_i$, and $\Dmat$ in Step (2b) does not use $\X$ \blue{(Laird and Ware 1982)}, and hence is unaffected by the missing attribute values.



==> score.tex <==
\section{Estimation and Inference}\label{sec:estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Let $\mathcal{W}=\{W_{it}|1\le i\le N, 1\le t\le T\}$ be the set of data with $W_{it} = (\yit, \dit, \xit)$, where $i$ denotes the cross-sectional dimension and $t$ the time dimension. Let $\eta = (m, h)$ be a vector of nuisance parameters with population value $\eta_0 = (m_0, h_0)$, and $\theta$ be the causal parameter. 
 
 Define a generic known score functions as
\begin{equation}
\psi(W; \theta, \eta) \equiv \tuit \tvit\label{eqn:score}
\end{equation}


Under some regularity conditions \red{[mention in asm],} $\theta$ satisfies the moment condition
\begin{equation}\label{eqn:mom_cond}
\E\big[\psi(W; \theta, \eta)\big]  = 0
\end{equation}
\noindent such that $\widehat{\theta}_0$ solves the finite-sample analog of the estimating equation \eqref{eqn:mom_cond}
\begin{equation}\label{eqn:fmom_cond}
\frac{1}{N}\sum_{i\in \Wk} \psi(W; \widehat{\theta}_0, \widehat{\eta}_0)  = 0
\end{equation}

\noindent \textbf{PO score:} $ a(\nabla_{it},\txit) = \Vii'\Vii$ where $\Vii = \Dii-m(\xit)$, and $h(\txit)=l(\xit)$. \\
\noindent  \textbf{IV score:} $ a(\nabla_{it},\txit) = \Dii'\Vii$, and $h(\txit)=g(\xit)$. 

%• The fit() method trains the model on the input data by adjusting the parameters of the decision trees to minimize the error between the predicted and actual values.


The estimation and inference of the causal parameter is conducted by following the algorithm \textsc{DML2}  from \cite{chernozhukov2018}. This is summarised in the algorithm below.

\noindent \textsc{Algorithm 2.1}:  Estimation of $\theta$
\begin{enumerate}[label={(\arabic*})]
    \item Divide the set $\mathcal{W}$ into $K$ random partitions (or folds) each of cross-sectional size $N_k = N/K$. Let $\Wk$ be the set of units in the $k$-th fold, and $\Wk^c$ the complementary set such that $\Wk \cup \Wk^c = \mathcal{W} $ and $\Wk \cap \Wk^c = \emptyset$. %Due to the nature of the data, 
    A unit with its full time series is either assigned to the $k$-th fold or to the complementary set, i.e., if $i\in\Wk \Rightarrow i\notin\Wk^c$. \label{item:step1}
    \item Fit the model using the data in the complementary set, $\Wk^c$, and use these estimates to predict the vector of nuisance parameters, $\widehat{\eta}_{0,k}$, from the data in the $k$-th partition, $\Wk$. Repeat this step for each fold $k\in \{1,\dots,K\}$. The inputs differ by panel data method. \label{item:step2}
    \begin{enumerate}[label={(\roman*})]
        \item \textbf{WG}: Learn $l(\txit)_k$  using $\{\tyit, \txit\}$; learn $m(\txit)_k$ using $\{\tdit,\txit\}$.
        \item \textbf{FD}: Learn $l(\Delta\xit)_k$ using $\{\Delta\yit, \Delta\xit\}$; learn $m(\Delta\xit)_k$ using $\{\Delta\dit,\Delta\xit\}$.
        \item \textbf{CRE}: Learn $l(\xit, \bxi)_k$ using $\{\yit, \xit, \bxi\}$; learn $m(\xit, \bxi,\bdi)_k$ using $\{\dit,\xit, \bxi,\bdi\}$.
    \end{enumerate}

    \item Plug the fold-specific predicted nuisances from step~\ref{item:step2} in the score functions~\eqref{eqn:score} and solve the finite-sample moment condition~\eqref{eqn:fmom_cond} with respect to $\theta$, using $i\in\Wk$. Average the scores over the $K$ folds to obtain an estimate of the causal effect and its variance.\label{item:step3}
\end{enumerate}

\noindent There are two types of Neywan-orthogonal (NO) scores that can be used at stage~\ref{item:step3} to retrieve the causal effect and the inference. These are partialling-out (PO) and IV-type score functions, that differ as follows  \\
    \input{tabs/scores}

\

\noindent The variance-covariance matrix is robust to heteroskedasticity, and clustered at the individual level. 
%\noindent The Newyman orthogonal estimator is consistent and unbiased \red{[ref or proof]}.



==> tabs/04_tab5_cre_pres.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Tab 5 - Mod (2) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
 \caption{The Effect of National Minimum Wage on Voting Behaviour in the UK}\label{tab:fazio5}
\scalebox{.65}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS&  DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)\\
\vspace{-3mm}\\
\hline
\vspace{-2mm}\\
\multicolumn{6}{c}{\emph{Dependent variable: ``Vote for conservative parties''}}\\
\vspace{-3mm}\\
\multicolumn{6}{l}{\emph{Panel A: Base control variables}}\\
\vspace{-3mm}\\
NMW &0.093*&0.086*&0.034&0.061*&0.245\\
&(0.047)&(0.046)&(0.034)&(0.035)&(0.298)\\
No. control variables&5&25&5&5&5\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel B: Additional control variables}}\\
\vspace{-3mm}\\
NMW &0.095*&0.083*&0.087*&0.135**&0.247\\
&(0.047)&(0.047)&(0.048)&(0.067)&(0.283)\\
No. control variables&36&738&36&36&36\\
\vspace{-3mm}\\
\hline
\vspace{-3mm}\\
Wave and region FE&Yes&Yes&Yes&Yes&Yes\\
No. observations&16,809&16,809&16,809&16,809&16,809\\
No. groups&4,342&4,342&4,342&4,342&4,342\\
\hline
\end{tabular} 	
\footnotesize
\textbf{Note:} The table reports our estimates based on Specification~(2) of Table~5 in \cite{fazio2023} using a different sample and covariates. Column~(1) reports the figures estimated via OLS while the remaining columns via DML with different learners. Panel A includes only base control variables like age, education, marital status, household size, income of other members. Panel B includes additional control variables such as other socio-demographic, economic, work-related and ideology variables in addition to base control variables. The number of control variables includes the raw variables (or the extended dictionary) and not their means. Additional Resampling information: CRE estimator, 5 folds, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01. \hyperlink{sec:appx_wg}{\beamergotobutton{Table WG}}
\end{threeparttable}
}
\end{table}


%rf:  0.0005241692 0.03828220  0.01369224 0.9890755    10
%cart: 0.05323519 0.03609347  1.4749260 0.14023243 10
%xgboost: 0.24686352 0.21029194 1.1739086 0.2404316

==> tabs/04_tab5_ols_dmlsim.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Tab 5 - Mod (2) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
 \caption{The Effect of National Minimum Wage on Voting Behavior in the UK}\label{tab:fazio5}
\scalebox{.9}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS&  DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)\\
\vspace{-3mm}\\
\hline
% \vspace{-2mm}\\
% \multicolumn{6}{c}{\emph{Dependent variable: ``Vote for conservative parties''}}\\
% \vspace{-3mm}\\
% \multicolumn{6}{l}{\emph{Panel A: Base control variables}}\\
% \vspace{-3mm}\\
% NMW &0.093*&0.086*&0.034&0.061*&0.245\\
% &(0.047)&(0.046)&(0.034)&(0.035)&(0.298)\\
% No. control variables&5&25&5&5&5\\

\multicolumn{6}{c}{\emph{Dependent variable: Voting for conservative parties}}\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel A: CRE approach}}\\
\vspace{-3mm}\\
NMW &0.095*&0.083*&0.087*&0.135**&0.247\\
&(0.047)&(0.047)&(0.048)&(0.067)&(0.283)\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel B: Exact approach with FD}}\\
\vspace{-3mm}\\
NMW &0.095*&0.083*&0.087*&0.135**&0.247\\
&(0.047)&(0.047)&(0.048)&(0.067)&(0.283)\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel C: Hybrid approach with WG}}\\
\vspace{-3mm}\\
NMW&0.097**&0.086***&0.091***&0.098***&\\
&(0.045)&(0.045)&(0.044)&(0.045)&\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel E: Approximation approach with WG}}\\
\vspace{-3mm}\\
NMW&0.097**&0.079**&0.091**&0.095***&\\
&(0.045)&(0.045)&(0.042)&(0.048)&\\

\vspace{-2mm}\\
\hline
\vspace{-3mm}\\
Wave and region FE&Yes&Yes&Yes&Yes&Yes\\
No. observations&16,809&16,809&16,809&16,809&16,809\\
No. groups&4,342&4,342&4,342&4,342&4,342\\
No. control variables&36&738&36&36&36\\
\hline
\end{tabular} 	
\footnotesize
\renewcommand{\baselineskip}{11pt}
\textbf{Note:} The table reports our estimates based on Specification~(2) of Table~5 in \cite{fazio2023} using a different sample and covariates. Column~(1) reports the figures estimated via OLS while the remaining columns via DML with different learners. Panel A includes only base control variables like age, education, marital status, household size, income of other members. Panel B includes additional control variables such as other socio-demographic, economic, work-related and ideology variables in addition to base control variables. The number of control variables includes the raw variables (or the extended dictionary) and not their means. Additional Resampling information: CRE estimator, 5 folds, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.
\end{threeparttable}}
\end{table}


%rf:  0.0005241692 0.03828220  0.01369224 0.9890755    10
%cart: 0.05323519 0.03609347  1.4749260 0.14023243 10
%xgboost: 0.24686352 0.21029194 1.1739086 0.2404316

==> tabs/05_simul_cre.tex <==
\begin{table}[th!]
\centering
 \caption{Simulation results, DGP1}\label{tab:collapse_dgp1}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: CRE   estimator}}\\
\vspace{-3mm}\\
OLS	&	0.000	&	0.039	&	0.852	&	0.003	&	0.012	&	0.917	&	0.001	&	0.005	&	1.123	\\
DML-Lasso	&	0.044	&	0.057	&	0.979	&	0.013	&	0.017	&	0.967	&	0.007	&	0.009	&	0.990	\\
DML-Lasso\texttt{+}	&	0.063	&	0.073	&	1.102	&	0.026	&	0.028	&	1.085	&	0.013	&	0.014	&	0.982	\\
DML-CART	&	0.010	&	0.054	&	1.064	&	0.015	&	0.030	&	0.627	&	0.021	&	0.032	&	0.333	\\
DML-RF	&	0.084	&	0.098	&	1.065	&	0.017	&	0.022	&	1.008	&	0.006	&	0.011	&	0.743	\\
DML-Boosting	&	0.022	&	0.047	&	1.303	&	-0.022	&	0.026	&	0.967	&	-0.014	&	0.016	&	0.811	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: WG hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.004	&	0.034	&	1.018	&	0.001	&	0.010	&	1.050	&	0.001	&	0.005	&	1.123\\
DML-Lasso	&	0.004	&	0.030	&	1.103	&	0.001	&	0.010	&	1.076	&	0.001	&	0.005	&	1.005\\
DML-Lasso\texttt{+}	&	0.003	&	0.030	&	1.112	&	0.001	&	0.010	&	1.091	&	0.001	&	0.005	&	0.999\\
DML-CART	&	-0.023	&	0.049	&	0.836	&	-0.014	&	0.028	&	0.412	&	0.000	&	0.027	&	0.190\\
DML-RF	&	0.017	&	0.040	&	0.936	&	-0.016	&	0.021	&	0.747	&	-0.026	&	0.030	&	0.327\\
DML-Boosting	&	-0.050	&	0.063	&	0.932	&	-0.043	&	0.045	&	0.846	&	-0.023	&	0.024	&	1.023\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: FD hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.002	&	0.042	&	0.987	&	0.004	&	0.013	&	1.024	&	0.001	&	0.006	&	1.028	\\
DML-Lasso	&	0.004	&	0.036	&	1.124	&	0.000	&	0.012	&	1.010	&	0.000	&	0.006	&	1.039	\\
DML-Lasso\texttt{+}	&	0.004	&	0.036	&	1.117	&	0.000	&	0.013	&	1.032	&	0.000	&	0.006	&	1.036	\\
DML-CART	&	-0.023	&	0.054	&	0.890	&	-0.014	&	0.030	&	0.467	&	-0.001	&	0.027	&	0.229	\\
DML-RF	&	0.013	&	0.045	&	0.968	&	-0.016	&	0.023	&	0.783	&	-0.027	&	0.031	&	0.397	\\
DML-Boosting	&	-0.049	&	0.067	&	0.925	&	-0.045	&	0.048	&	0.810	&	-0.023	&	0.024	&	1.008	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 100. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/06_mcsim.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CRE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
 \caption{Simulation results for $\thetano_N$, nonlinear and discontinuous DGP}\label{tab:mx_collapse}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	\\
\hline
% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel A: DGP1}}\\
% \vspace{-3mm}\\
% OLS	&	0.000	&	0.039	&	0.852	&	0.003	&	0.012	&	0.917	&	0.001	&	0.005	&	1.123	\\
% DML-Lasso	&	0.063	&	0.073	&	1.102	&	0.026	&	0.028	&	1.085	&	0.013	&	0.014	&	0.982	\\
% DML-CART	&	0.010	&	0.054	&	1.064	&	0.015	&	0.030	&	0.627	&	0.021	&	0.032	&	0.333	\\
% DML-RF	&	0.084	&	0.098	&	1.065	&	0.017	&	0.022	&	1.008	&	0.006	&	0.011	&	0.743	\\
% DML-Boosting	&	0.022	&	0.047	&	1.303	&	-0.022	&	0.026	&	0.967	&	-0.014	&	0.016	&	0.811	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel A: DGP2 - CRE approach}}\\
% \vspace{-3mm}\\
% OLS	&	-0.004	&	0.032	&	0.918	&	0.000	&	0.009	&	0.968	&	0.000	&	0.004	&	1.063	\\
% DML-Lasso	&	0.061	&	0.070	&	0.939	&	0.017	&	0.020	&	0.965	&	0.008	&	0.009	&	1.063	\\
% DML-CART	&	0.003	&	0.053	&	1.027	&	-0.025	&	0.028	&	1.045	&	-0.024	&	0.025	&	0.988	\\
% DML-RF	&	0.018	&	0.040	&	1.111	&	0.010	&	0.017	&	0.864	&	-0.017	&	0.028	&	0.268	\\
% DML-Boosting	&	-0.018	&	0.048	&	1.036	&	-0.039	&	0.042	&	0.990	&	-0.022	&	0.024	&	0.813	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: CRE approach}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.962	&	0.993	&	0.993	&	1.037	&	0.993	&	0.993	&	0.999	\\
DML-Lasso	&	0.103	&	0.130	&	1.062	&	0.021	&	0.049	&	0.778	&	0.009	&	0.014	&	1.235	\\
DML-CART	&	0.200	&	0.287	&	0.372	&	0.018	&	0.107	&	0.235	&	0.053	&	0.134	&	0.101	\\
DML-RF	&	0.705	&	0.760	&	0.234	&	0.268	&	0.485	&	0.108	&	0.151	&	0.440	&	0.056	\\
DML-Boosting	&	0.382	&	0.426	&	0.557	&	0.088	&	0.112	&	0.818	&	-0.007	&	0.039	&	0.792	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: Exact approach with FD transformation}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.889	&	0.993	&	0.993	&	0.961	&	0.993	&	0.993	&	0.951	\\
DML-Lasso	&	0.036	&	0.051	&	1.143	&	0.004	&	0.013	&	1.045	&0.005	&	0.008	&	1.050	\\
DML-CART	&	0.646	&	0.664	&	0.319	&	0.552	&	0.583	&	0.096	&0.537	&	0.566	&	0.051	\\
DML-RF	&	0.911	&	0.919	&	0.177	&	0.816	&	0.856	&	0.053	&0.702	&	0.802	&	0.023	\\
DML-Boosting	&	0.718	&	0.725	&	0.455	&	0.322	&	0.343	&	0.371	&0.031	&	0.078	&	0.380	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: Hybrid approach with WG transformation}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.999	&	0.993	&	0.993	&	1.001	&	0.993	&	0.993	&	0.999	\\
DML-Lasso	&	0.010	&	0.031	&	1.152	&	-0.004	&	0.011	&	1.042	&	-0.022	&	0.022	&	1.017	\\
DML-CART	&	0.200	&	0.278	&	0.400	&	-0.001	&	0.102	&	0.238	&	0.049	&	0.136	&	0.096	\\
DML-RF	&	0.683	&	0.739	&	0.233	&	0.255	&	0.490	&	0.103	&	0.175	&	0.515	&	0.053	\\
DML-Boosting	&	0.435	&	0.461	&	0.707	&	0.090	&	0.125	&	0.763	&	-0.034	&	0.055	&	0.823	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel D: Approximation approach for WG transformation}}\\
\vspace{-3mm}\\
OLS&	0.992	&	0.992	&	1.066	&	0.993	&	0.993	&	0.880	&	0.993	&	0.993	&	0.999	\\
DML-Lasso&	0.973	&	0.973	&	0.939	&	0.977	&	0.977	&	1.002	&	0.977	&	0.977	&	1.120	\\
DML-CART&	0.708	&	0.720	&	0.331	&	0.702	&	0.710	&	0.124	&	0.710	&	0.715	&	0.079	\\
DML-RF&	0.952	&	0.955	&	0.294	&	0.925	&	0.929	&	0.089	&	0.914	&	0.919	&	0.045	\\
DML-Boosting&	0.829	&	0.831	&	0.723	&	0.876	&	0.876	&	0.449	&	0.921	&	0.921	&	0.294	\\


\hline
\end{tabular} 	
% \begin{tablenotes}[para,flushleft]	
% \emph{Note: The figures in the table are the average values over the total number of replications. The number of Monte Carlo replications is 100; the true target parameter 
% is 0.50; $T=10$. We use the Neyman-orthogonal PO score and five-fold cross-fitting. Hyperparameters of base learners tuned.}
% \end{tablenotes}
\footnotesize
\renewcommand{\baselineskip}{11pt}
\textbf{Note:} The figures in the table are the average values over the total number of replications. The number of Monte Carlo replications is 100; the true target parameter is 0.50; $T=10$. We use the Neyman-orthogonal PO score and five-fold cross-fitting.
\end{threeparttable}
}
\end{table}


==> tabs/888_application_pres.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Tab 5 - Mod (2) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
 \caption{The Effect of NMW on Voting Behaviour in the UK}\label{tab:fazio5}
\scalebox{.6}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS&  DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)\\
\vspace{-3mm}\\
\hline

\multicolumn{6}{c}{\emph{Dependent variable: Voting for conservative parties}}\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel A: CRE approach}}\\
\vspace{-3mm}\\
NMW &0.051***&0.048**&0.069*&0.180&-0.319\\
&(0.019)&(0.019)&(0.036)&(0.151)&(0.278)\\
\vspace{-3mm}\\
RMSE of learner $l$&& 0.4574&0.4195&0.4130&0.4350\\
RMSE of learner $m$&&0.0645&0.0512&0.0155&0.0107\\
Model RMSE&&1.1143& 1.030&1.0085&1.0478\\
No. control variables&72&1,476&72&72&72\\

\hline

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel B: Exact approach with FD}}\\
\vspace{-3mm}\\
$\Delta$NMW&0.022*&0.021&0.026&0.018&0.024\\
&(0.013)&(0.026)&(0.026)&(0.026)&(0.026)\\
\vspace{-3mm}\\
RMSE of learner $l$&&0.2821&0.2823&0.2815&0.2859\\
RMSE of learner $m$&&0.0504&0.0499&0.0492&0.0533\\
Model RMSE&&0.6419&0.6427&0.6404&0.6261\\
No. control variables&72&1,476&72&72&72\\

\hline
\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel C: Approximation approach with WG}}\\
\vspace{-3mm}\\
$\widetilde{\rm{NMW}}$&0.050***&0.046**&0.048**&0.040**&0.048***\\
&(0.019)&(0.019)&(0.019)&(0.018)&(0.017)\\
\vspace{-3mm}\\
RMSE of learner $l$&&0.2121&0.2130&0.2124&0.2155\\
RMSE of learner $m$&&0.0642&0.0645&0.0651&0.0711\\
Model RMSE&&0.5276&0.5299&0.5278&0.5239\\
No. control variables&36&738&36&36&36\\

\hline
\end{tabular} 
\begin{tablenotes}[para,flushleft]	
\emph{Note: Our estimates based on Specification~(2) of Table~5 in \cite{fazio2023}. No. of observations ($NT$) is $59,745$ in Panels A, C and D, and is $49,823$ in Panel B;  no. of cross-sectional units ($N$) $9,922$. 
Cluster-robust standard errors at the respondent level in parenthesis. Significance levels: * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01. \,{\tiny \hyperlink{sec:hyperpara_appl}{\beamergotobutton{Tuning}}}}
\end{tablenotes}
\end{threeparttable}
}

\end{table}


==> tabs/88_simul_results.tex <==
\section{Additional Tables}\label{sec:add_tabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% FD LAG
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[th!]
\centering
 \caption{Simulation results for $\thetano_N$, FD estimator (with lagged inputs)}\label{tab:collapse_FDlag}
\scalebox{.9}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: DGP1}}\\
\vspace{-3mm}\\
OLS	&	0.003	&	0.041	&	1.002	&	0.000	&	0.012	&	1.016	& 0.001	&	0.006	&	1.029\\
DML-Lasso	&	0.018	&	0.041	&	1.077	&	0.001	&	0.013	&	1.007	&0.000	&	0.006	&	1.041\\
DML-CART	&	0.060	&	0.075	&	0.897	&	0.106	&	0.109	&	0.467	&0.119	&	0.122	&	0.221\\
DML-RF	&	0.067	&	0.077	&	0.997	&	0.039	&	0.043	&	0.704	&0.029	&	0.035	&	0.308	\\
DML-Boosting	&	-0.015	&	0.046	&	0.887	&	-0.040	&	0.043	&	0.837	&-0.021	&	0.022	&	0.798	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: DGP2}}\\
\vspace{-3mm}\\
OLS	&	-0.001	&	0.037	&	0.932	&	-0.002	&	0.011	&	1.022	&-0.001	&	0.005	&	1.021	\\
DML-Lasso	&	-0.002	&	0.035	&	0.969	&	-0.002	&	0.011	&	1.027	&-0.001	&	0.005	&	1.018	\\
DML-CART	&	-0.056	&	0.067	&	0.927	&	-0.027	&	0.029	&	1.003	&-0.027	&	0.028	&	0.993	\\
DML-RF	&	-0.027	&	0.043	&	1.020	&	0.001	&	0.014	&	0.839	&-0.009	&	0.015	&	0.553	\\
DML-Boosting	&	-0.055	&	0.068	&	0.881	&	-0.042	&	0.045	&	0.815	&-0.022	&	0.024	&	0.692	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: DGP3}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.889	&	0.993	&	0.993	&	0.961	&	0.993	&	0.993	&	0.951	\\
DML-Lasso	&	0.036	&	0.051	&	1.143	&	0.004	&	0.013	&	1.045	&0.005	&	0.008	&	1.050	\\
DML-CART	&	0.646	&	0.664	&	0.319	&	0.552	&	0.583	&	0.096	&0.537	&	0.566	&	0.051	\\
DML-RF	&	0.911	&	0.919	&	0.177	&	0.816	&	0.856	&	0.053	&0.702	&	0.802	&	0.023	\\
DML-Boosting	&	0.718	&	0.725	&	0.455	&	0.322	&	0.343	&	0.371	&0.031	&	0.078	&	0.380	\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: The figures in the table are the average values over the total number of replications. The number of replications is 100. The true target parameter $\theta$ is 0.50.  Hyperparameters of base learners tuned as described in Table~\ref{tab:hyperpara}.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% wg
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th!]
\centering
 \caption{Simulation results for $\thetano_N$,  WG estimator (hybrid)}\label{tab:collapse_WG}
\scalebox{.9}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: DGP1}}\\
\vspace{-3mm}\\
OLS	&	0.004	&	0.034	&	1.018	&	0.001	&	0.010	&	1.050	&	0.001	&	0.005	&	1.123\\
%DML-Lasso	&	0.004	&	0.030	&	1.103	&	0.001	&	0.010	&	1.076	&	0.001	&	0.005	&	1.005\\
DML-Lasso&	0.003	&	0.030	&	1.112	&	0.001	&	0.010	&	1.091	&	0.001	&	0.005	&	0.999\\
DML-CART	&	-0.023	&	0.049	&	0.836	&	-0.014	&	0.028	&	0.412	&	0.000	&	0.027	&	0.190\\
DML-RF	&	0.017	&	0.040	&	0.936	&	-0.016	&	0.021	&	0.747	&	-0.026	&	0.030	&	0.327\\
DML-Boosting	&	-0.050	&	0.063	&	0.932	&	-0.043	&	0.045	&	0.846	&	-0.023	&	0.024	&	1.023\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: DGP2}}\\
\vspace{-3mm}\\
OLS	&	0.000	&	0.034	&	0.915	&	0.003	&	0.010	&	0.996	&	0.001	&	0.004	&	1.156	\\
%DML-Lasso	&	0.000	&	0.029	&	0.968	&	-0.001	&	0.009	&	1.036	&	0.000	&	0.004	&	1.076	\\
DML-Lasso	&	0.001	&	0.031	&	0.942	&	-0.001	&	0.009	&	0.999	&	0.000	&	0.004	&	1.073	\\
DML-CART	&	-0.024	&	0.042	&	0.903	&	-0.047	&	0.048	&	0.847	&	-0.048	&	0.048	&	0.886	\\
DML-RF	&	-0.022	&	0.039	&	0.896	&	0.003	&	0.014	&	0.782	&	-0.007	&	0.017	&	0.318	\\
DML-Boosting	&	-0.061	&	0.070	&	0.949	&	-0.044	&	0.046	&	0.963	&	-0.024	&	0.025	&	1.134	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: DGP3}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.999	&	0.993	&	0.993	&	1.001	&	0.993	&	0.993	&	0.999	\\
%DML-Lasso	&	0.989	&	0.989	&	0.908	&	0.992	&	0.992	&	0.965	&	0.993	&	0.993	&	0.998	\\
DML-Lasso	&	0.010	&	0.031	&	1.152	&	-0.004	&	0.011	&	1.042	&	-0.022	&	0.022	&	1.017	\\
DML-CART	&	0.200	&	0.278	&	0.400	&	-0.001	&	0.102	&	0.238	&	0.049	&	0.136	&	0.096	\\
DML-RF	&	0.683	&	0.739	&	0.233	&	0.255	&	0.490	&	0.103	&	0.175	&	0.515	&	0.053	\\
DML-Boosting	&	0.435	&	0.461	&	0.707	&	0.090	&	0.125	&	0.763	&	-0.034	&	0.055	&	0.823	\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: The figures in the table are the average values over the total number of replications. The number of replications is 100. The true target parameter $\theta$ is 0.50.  Hyperparameters of base learners tuned as described in Table~\ref{tab:hyperpara}.}
\end{tablenotes}
\end{threeparttable}}
\end{table}


==> tabs/88_simul_results_cre.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CRE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
 \caption{Simulation results for $\thetano_N$, CRE estimator}\label{tab:collapse_CRE}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	%
&	Bias&	RMSE	&	SE/SD	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: DGP1}}\\
\vspace{-3mm}\\
OLS	&	0.000	&	0.039	&	0.852	&	0.003	&	0.012	&	0.917	&	0.001	&	0.005	&	1.123	\\
DML-Lasso	&	0.063	&	0.073	&	1.102	&	0.026	&	0.028	&	1.085	&	0.013	&	0.014	&	0.982	\\
DML-CART	&	0.010	&	0.054	&	1.064	&	0.015	&	0.030	&	0.627	&	0.021	&	0.032	&	0.333	\\
DML-RF	&	0.084	&	0.098	&	1.065	&	0.017	&	0.022	&	1.008	&	0.006	&	0.011	&	0.743	\\
DML-Boosting	&	0.022	&	0.047	&	1.303	&	-0.022	&	0.026	&	0.967	&	-0.014	&	0.016	&	0.811	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: DGP2}}\\
\vspace{-3mm}\\
OLS	&	-0.004	&	0.032	&	0.918	&	0.000	&	0.009	&	0.968	&	0.000	&	0.004	&	1.063	\\
DML-Lasso	&	0.061	&	0.070	&	0.939	&	0.017	&	0.020	&	0.965	&	0.008	&	0.009	&	1.063	\\
DML-CART	&	0.003	&	0.053	&	1.027	&	-0.025	&	0.028	&	1.045	&	-0.024	&	0.025	&	0.988	\\
DML-RF	&	0.018	&	0.040	&	1.111	&	0.010	&	0.017	&	0.864	&	-0.017	&	0.028	&	0.268	\\
DML-Boosting	&	-0.018	&	0.048	&	1.036	&	-0.039	&	0.042	&	0.990	&	-0.022	&	0.024	&	0.813	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: DGP3}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.962	&	0.993	&	0.993	&	1.037	&	0.993	&	0.993	&	0.999	\\
DML-Lasso	&	0.103	&	0.130	&	1.062	&	0.021	&	0.049	&	0.778	&	0.009	&	0.014	&	1.235	\\
DML-CART	&	0.200	&	0.287	&	0.372	&	0.018	&	0.107	&	0.235	&	0.053	&	0.134	&	0.101	\\
DML-RF	&	0.705	&	0.760	&	0.234	&	0.268	&	0.485	&	0.108	&	0.151	&	0.440	&	0.056	\\
DML-Boosting	&	0.382	&	0.426	&	0.557	&	0.088	&	0.112	&	0.818	&	-0.007	&	0.039	&	0.792	\\
\hline
\end{tabular} 	
% \begin{tablenotes}[para,flushleft]	
% \emph{Note: The figures in the table are the average values over the total number of replications. The number of Monte Carlo replications is 100; the true target parameter 
% is 0.50; $T=10$. We use the Neyman-orthogonal PO score and five-fold cross-fitting. Hyperparameters of base learners tuned.}
% \end{tablenotes}
\footnotesize
\renewcommand{\baselineskip}{11pt}
\textbf{Note:} The figures in the table are the average values over the total number of replications. The number of Monte Carlo replications is 100; the true target parameter is 0.50; $T=10$. We use the Neyman-orthogonal PO score and five-fold cross-fitting. Hyperparameters of base learners tuned.
\end{threeparttable}
}
\end{table}


==> tabs/99_dml_tab5_fazio.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Tab 5 - Mod (2) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th!]
\centering
 \caption{The Effect of National Minimum Wage on Voting Behaviour in the UK}\label{tab:fazio5}
\scalebox{.65}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lcccccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
&\multicolumn{5}{c}{\emph{Base control variables}}&\multicolumn{5}{c}{\emph{Additional control variables}}\\
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}
& OLS&  DML-Lasso& DML-CART& DML-RF& DML-Boosting&OLS& DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\vspace{-3mm}\\
\hline
\vspace{-2mm}\\

\multicolumn{11}{l}{\emph{Dependent variable: ``Vote conservative''}}\\
\vspace{-3mm}\\
NMW &0.091*&0.084**&0.053&0.001&0.247&0.097**&0.084**&0.053&0.105*&0.095\\
&(0.047)&(0.046)&(0.036)&(0.038)&(0.210)&(0.047)&(0.047)&(0.036)&(0.060)&(0.130)\\
\vspace{-3mm}\\
\hline
\vspace{-2mm}\\
% Base controls&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
% Additional controls&No&Yes&No&Yes&No&Yes&No&Yes\\
Wave and region FE&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
% \vspace{-3mm}\\
% \hline
% \vspace{-2mm}\\

No. observations&16,809&16,809&16,809&16,809&16,809&16,809&16,809&16,809&16,809&16,809\\
No. groups&4,342&4,342&4,342&4,342&4,342&4,342&4,342&4,342&4,342&4,342\\
No. control variables&12&50&10&10&10&82&1,476&144&144&144\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: The table reports our replicated results of Specification~(2) of Table~5 in \cite{fazio2023} using a different sample and covariates. Columns~(1) and~(5) report the figures estimated via least squares while remaining columns via DML with different learners. Regressions with base control variables include: age, age squared (not for CART and RF), education, marital status, household size, income of other members. Regressions with additional control variables include other socio-demgraphic, economic, work-related and ideology variables in addition to base control variables. Additional Resampling information: CRE estimator, 5 folds, cross-fitting, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}


%rf:  0.0005241692 0.03828220  0.01369224 0.9890755    10
%cart: 0.05323519 0.03609347  1.4749260 0.14023243 10
%xgboost: 0.24686352 0.21029194 1.1739086 0.2404316

==> tabs/99_fazio_pres.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Tab 5 - Mod (2) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
 \caption{The Effect of NMW on Voting Behaviour in the UK}\label{tab:fazio5}
\scalebox{.6}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS&  DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)\\
\vspace{-3mm}\\
\hline

\multicolumn{6}{c}{\emph{Dependent variable: Voting for conservative parties}}\\

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel A: CRE approach}}\\
\vspace{-3mm}\\
NMW &0.051***&0.048**&0.069*&0.180&-0.319\\
&(0.019)&(0.019)&(0.036)&(0.151)&(0.278)\\
\vspace{-3mm}\\
RMSE of learner $l$&& 0.4574&0.4195&0.4130&0.4350\\
RMSE of learner $m$&&0.0645&0.0512&0.0155&0.0107\\
Model RMSE&&1.1143& 1.030&1.0085&1.0478\\
No. control variables&72&1,476&72&72&72\\
% No. observations&59,745&&&&\\
% No. groups& 9,922&&&&\\
\hline

\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel B: Exact approach with FD}}\\
\vspace{-3mm}\\
$\Delta$NMW&0.022*&0.021&0.026&0.018&0.024\\
&(0.013)&(0.026)&(0.026)&(0.026)&(0.026)\\
\vspace{-3mm}\\
RMSE of learner $l$&&0.2821&0.2823&0.2815&0.2859\\
RMSE of learner $m$&&0.0504&0.0499&0.0492&0.0533\\
Model RMSE&&0.6419&0.6427&0.6404&0.6261\\
No. control variables&72&1,476&72&72&72\\

\hline
\vspace{-2mm}\\
\multicolumn{6}{l}{\emph{Panel C: Approximation approach with WG}}\\
\vspace{-3mm}\\
$\widetilde{\rm{NMW}}$&0.051***&0.046**&0.048**&0.040**&0.048***\\
&(0.019)&(0.019)&(0.019)&(0.018)&(0.017)\\
\vspace{-3mm}\\
RMSE of learner $l$&&0.2121&0.2130&0.2124&0.2155\\
RMSE of learner $m$&&0.0642&0.0645&0.0651&0.0711\\
Model RMSE&&0.5276&0.5299&0.5278&0.5239\\
No. control variables&36&738&36&36&36\\
\hline
\end{tabular} 
\begin{tablenotes}[para,flushleft]	
\emph{Note: Our estimates based on Specification~(2) of Table~5 in \cite{fazio2023}. No. of observations ($NT$) is $59,745$ in Panels A, C and D, and is $49,823$ in Panel B;  no. of cross-sectional units ($N$) $9,922$. 
Cluster-robust standard errors at the respondent level in parenthesis. Significance levels: * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01. \hyperlink{sec:hyperpara_appl}{\beamergotobutton{Tuning}}}
\end{tablenotes}
\end{threeparttable}
}

\end{table}


==> tabs/99_tabs_fazio.tex <==
\begin{table}[th!]
\centering
 \caption{Replication Results without fixed effects, WG estimator}\label{tab:fazio5_noFE}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
&&\multicolumn{3}{c}{\emph{Approximation approach}}&\multicolumn{3}{c}{\emph{Hybrid approach}}\\
 \cmidrule(l{.35cm}r{.25cm}){3-5}\cmidrule(l{.35cm}r{.25cm}){6-8}
& OLS& DML-Lasso\texttt{+}& DML-CART& DML-RF& DML-Lasso\texttt{+}& DML-CART& DML-RF\\
&(1)&(2)&(3)&(4)&(5)&(6)&(7)\\
\vspace{-3mm}\\	
\hline
\vspace{-2mm}\\
\multicolumn{8}{c}{\emph{Dependent variable: ``Vote conservative''}}\\
\vspace{-3mm}\\
NMW &0.101**&0.103***&0.091***&0.099***&0.100***&0.091***&0.101***\\
&(0.044)&(0.044)&(0.044)&(0.044)&(0.045)&(0.044)&(0.045)\\

\vspace{-3mm}\\
No. Observations&19,961&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927&4,927&4,927\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: This table replicates Specification~(2) in Table~5 in \cite{fazio2023} without wave and region fixed effects. Column~(1) reports the least squares estimates; remaining columns use DML with different base learners. Base control variables include: age, age squared (not for CART and RF), education, marital status, household size, income of other members, and their individual means. DML-Lasso uses an extended dictionary of non-linear terms of the control variables (i.e., polynomials of order three and interactions of the control variables and their individual means). The hybrid approach includes the individual means of the control variables and fixed effects. Standard errors (in parenthesis) are clustered at the individual level. Resampling information: 5 folds, cross-fitting, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% with fixed effects
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th!]
\centering
 \caption{Replication  of Specification~(2) in Table~5 in \cite{fazio2023}}\label{tab:fazio5}
\scalebox{.75}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lcccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	

&&&\multicolumn{3}{c}{\emph{Approximation approach}}&\multicolumn{3}{c}{\emph{Hybrid approach}}\\
 \cmidrule(l{.35cm}r{.25cm}){4-6}\cmidrule(l{.35cm}r{.25cm}){7-9}
& OLS& OLS& DML-Lasso\texttt{+}& DML-CART& DML-RF& DML-Lasso\texttt{+}& DML-CART& DML-RF\\
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)\\
\vspace{-3mm}\\
\hline
\vspace{-2mm}\\

\multicolumn{9}{c}{\emph{Dependent variable: ``Vote conservative''}}\\
\vspace{-3mm}\\
NMW &0.097**&0.088**&0.086***&0.091***&0.098***&0.079**&0.091**&0.095***\\
&(0.045)&(0.045)&(0.045)&(0.044)&(0.045)&(0.045)&(0.042)&(0.048)\\
\vspace{-3mm}\\
\hline
\vspace{-2mm}\\
Wave FE&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
Wave x Region FE&No&Yes&Yes&No&No&Yes&No&No\\
% \vspace{-3mm}\\
\vspace{-3mm}\\
\hline
\vspace{-2mm}\\
No. Observations&19,961&19,961&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927&4,927&4,927&4,927\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: Column~(1) reports the original figures of Specification~(2) in Table~5 in \cite{fazio2023} estimated using least squares;  Column~(2) adds the interaction between wave and region fixed effects to Column~(1); remaining columns use DML with different learners. Base control variables include: age, age squared (not for CART and RF), education, marital status, household size, income of other members. DML-Lasso uses an extended dictionary of non-linear terms of the control variables and fixed effects (i.e., polynomials of order three and interactions of the control variables). The hybrid approach includes the individual means of the control variables and fixed effects. Standard errors (in parenthesis) are clustered at the individual level.  Standard errors (in parenthesis) are clustered at the individual level. Resampling information: 5 folds, cross-fitting, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/FDlag_wrong.tex <==
\begin{table}[th!]
\centering
 \caption{Simulation results, FD estimator (with lagged inputs) \red{[wrong!]}}\label{tab:collapse_FDlag}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: DGP1}}\\
\vspace{-3mm}\\
OLS	&	0.137	&	0.149	&	0.933	&	0.138	&	0.140	&	1.020	&	0.139	&	0.139	&	1.065	\\
DML-Lasso	&	0.148	&	0.159	&	0.987	&	0.141	&	0.142	&	1.048	&	0.139	&	0.140	&	1.129	\\
DML-CART	&	0.143	&	0.154	&	0.929	&	0.178	&	0.179	&	0.957	&	0.184	&	0.185	&	0.520	\\
DML-RF	&	0.149	&	0.161	&	0.901	&	0.145	&	0.146	&	1.161	&	0.141	&	0.141	&	0.857	\\
DML-Boosting	&	0.076	&	0.099	&	0.798	&	0.085	&	0.087	&	0.880	&	0.112	&	0.113	&	0.748	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: DGP2}}\\
\vspace{-3mm}\\
OLS	&	0.117	&	0.130	&	0.927	&	0.116	&	0.118	&	1.001	&	0.115	&	0.116	&	1.029	\\
DML-Lasso	&	0.120	&	0.132	&	0.986	&	0.117	&	0.118	&	1.047	&	0.116	&	0.116	&	1.167	\\
DML-CART	&	0.091	&	0.107	&	0.997	&	0.132	&	0.132	&	1.175	&	0.132	&	0.132	&	0.943	\\
DML-RF	&	0.106	&	0.119	&	1.008	&	0.137	&	0.138	&	1.227	&	0.135	&	0.135	&	0.947	\\
DML-Boosting	&	0.053	&	0.083	&	0.849	&	0.084	&	0.086	&	0.897	&	0.112	&	0.112	&	0.773	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: DGP3}}\\
\vspace{-3mm}\\
OLS	&	1.012	&	1.012	&	0.993	&	1.013	&	1.013	&	0.963	&	1.013	&	1.013	&	1.043	\\
DML-Lasso	&	0.162	&	0.179	&	1.087	&	0.143	&	0.144	&	1.069	&	0.140	&	0.140	&	1.175	\\
DML-CART	&	0.412	&	0.459	&	0.404	&	0.323	&	0.373	&	0.162	&	0.271	&	0.316	&	0.097	\\
DML-RF	&	0.829	&	0.865	&	0.201	&	0.609	&	0.727	&	0.113	&	0.317	&	0.519	&	0.066	\\
DML-Boosting	&	0.593	&	0.622	&	0.511	&	0.262	&	0.278	&	0.621	&	0.151	&	0.157	&	0.663	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 100. The true target parameter $\theta$ is 0.50.  Hyperparameters of base learners tuned as described in Table~\ref{tab:hyperpara}.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tabs/scores.tex <==
\begin{table}[th!]
\centering
\caption{Summary of the algorithm of NO scores}
\scalebox{.95}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{ll}  
\vspace{-3mm}\\   
\hline
\vspace{-3mm}\\
Partialling-out score & IV-type score\\	
\hline
\vspace{-3mm}\\
a. Learn $l(\txit)_k$ from $\tyit$ and $\txit$ &a. Learn $l(\txit)_k$ from $\tyit$ and $\txit$  \\
b. Learn $m(\txit)_k$ from $\tdit$ and $\txit$ & b. Learn $m(\txit)_k$ from $\tdit$ and $\txit$ \\
c.  Calculate $\widehat{\theta}^{PO}_k$ using $\widehat{l}(\txit)_k$ and $\widehat{m}(\txit)_k$ & c. Calculate $\widehat{\theta}^{PO}_k$ using $\widehat{l}(\txit)_k$ and $\widehat{m}(\txit)_k$\\
\vspace{-2mm}\\
& d. Learn $g(\txit)_k$ from $(\tyit-\widehat{\theta}^{PO}_k\tdit$) and $\txit$ \\
& e. Calculate $\widehat{\theta}^{IV}_k$ using $\widehat{g}(\txit)_k$ and $\widehat{m}(\txit)_k$\\
\vspace{-3mm}\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: This table summarises the main steps used to learn the nuisance parameters when the partialling-out (PO) or IV-type score functions are chosen. In the paper, we focus on the former for the explained reasons.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/sum_dgp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% DGP1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th!]
\centering
 \caption{Simulation results, DGP1}\label{tab:collapse_dgp1}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: CRE   estimator}}\\
\vspace{-3mm}\\
OLS	&	0.000	&	0.039	&	0.852	&	0.003	&	0.012	&	0.917	&	0.001	&	0.005	&	1.123	\\
DML-Lasso	&	0.044	&	0.057	&	0.979	&	0.013	&	0.017	&	0.967	&	0.007	&	0.009	&	0.990	\\
DML-Lasso\texttt{+}	&	0.063	&	0.073	&	1.102	&	0.026	&	0.028	&	1.085	&	0.013	&	0.014	&	0.982	\\
DML-CART	&	0.010	&	0.054	&	1.064	&	0.015	&	0.030	&	0.627	&	0.021	&	0.032	&	0.333	\\
DML-RF	&	0.084	&	0.098	&	1.065	&	0.017	&	0.022	&	1.008	&	0.006	&	0.011	&	0.743	\\
DML-Boosting	&	0.022	&	0.047	&	1.303	&	-0.022	&	0.026	&	0.967	&	-0.014	&	0.016	&	0.811	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: WG hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.004	&	0.034	&	1.018	&	0.001	&	0.010	&	1.050	&	0.001	&	0.005	&	1.123\\
DML-Lasso	&	0.004	&	0.030	&	1.103	&	0.001	&	0.010	&	1.076	&	0.001	&	0.005	&	1.005\\
DML-Lasso\texttt{+}	&	0.003	&	0.030	&	1.112	&	0.001	&	0.010	&	1.091	&	0.001	&	0.005	&	0.999\\
DML-CART	&	-0.023	&	0.049	&	0.836	&	-0.014	&	0.028	&	0.412	&	0.000	&	0.027	&	0.190\\
DML-RF	&	0.017	&	0.040	&	0.936	&	-0.016	&	0.021	&	0.747	&	-0.026	&	0.030	&	0.327\\
DML-Boosting	&	-0.050	&	0.063	&	0.932	&	-0.043	&	0.045	&	0.846	&	-0.023	&	0.024	&	1.023\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: FD hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.002	&	0.042	&	0.987	&	0.004	&	0.013	&	1.024	&	0.001	&	0.006	&	1.028	\\
DML-Lasso	&	0.004	&	0.036	&	1.124	&	0.000	&	0.012	&	1.010	&	0.000	&	0.006	&	1.039	\\
DML-Lasso\texttt{+}	&	0.004	&	0.036	&	1.117	&	0.000	&	0.013	&	1.032	&	0.000	&	0.006	&	1.036	\\
DML-CART	&	-0.023	&	0.054	&	0.890	&	-0.014	&	0.030	&	0.467	&	-0.001	&	0.027	&	0.229	\\
DML-RF	&	0.013	&	0.045	&	0.968	&	-0.016	&	0.023	&	0.783	&	-0.027	&	0.031	&	0.397	\\
DML-Boosting	&	-0.049	&	0.067	&	0.925	&	-0.045	&	0.048	&	0.810	&	-0.023	&	0.024	&	1.008	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 100. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% DGP2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tp!]
\centering
 \caption{Simulation results, DGP2}\label{tab:collapse_dgp2}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: CRE   estimator}}\\
\vspace{-3mm}\\
OLS	&	-0.004	&	0.032	&	0.918	&	0.000	&	0.009	&	0.968	&	0.000	&	0.004	&	1.063	\\
DML-Lasso	&	0.035	&	0.047	&	0.952	&	0.009	&	0.013	&	1.017	&	0.004	&	0.006	&	1.071	\\
DML-Lasso\texttt{+}	&	0.061	&	0.070	&	0.939	&	0.017	&	0.020	&	0.965	&	0.008	&	0.009	&	1.063	\\
DML-CART	&	0.003	&	0.053	&	1.027	&	-0.025	&	0.028	&	1.045	&	-0.024	&	0.025	&	0.988	\\
DML-RF	&	0.018	&	0.040	&	1.111	&	0.010	&	0.017	&	0.864	&	-0.017	&	0.028	&	0.268	\\
DML-Boosting	&	-0.018	&	0.048	&	1.036	&	-0.039	&	0.042	&	0.990	&	-0.022	&	0.024	&	0.813	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: WG hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.000	&	0.034	&	0.915	&	0.003	&	0.010	&	0.996	&	0.001	&	0.004	&	1.156	\\
DML-Lasso	&	0.000	&	0.029	&	0.968	&	-0.001	&	0.009	&	1.036	&	0.000	&	0.004	&	1.076	\\
DML-Lasso\texttt{+}	&	0.001	&	0.031	&	0.942	&	-0.001	&	0.009	&	0.999	&	0.000	&	0.004	&	1.073	\\
DML-CART	&	-0.024	&	0.042	&	0.903	&	-0.047	&	0.048	&	0.847	&	-0.048	&	0.048	&	0.886	\\
DML-RF	&	-0.022	&	0.039	&	0.896	&	0.003	&	0.014	&	0.782	&	-0.007	&	0.017	&	0.318	\\
DML-Boosting	&	-0.061	&	0.070	&	0.949	&	-0.044	&	0.046	&	0.963	&	-0.024	&	0.025	&	1.134	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: FD hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.001	&	0.037	&	0.914	&	-0.002	&	0.010	&	1.084	&	-0.001	&	0.005	&	1.021	\\
DML-Lasso	&	-0.001	&	0.033	&	1.007	&	-0.002	&	0.011	&	1.023	&	-0.002	&	0.006	&	1.003	\\
DML-Lasso\texttt{+}	&	0.000	&	0.035	&	0.967	&	-0.002	&	0.011	&	1.016	&	-0.001	&	0.005	&	1.013	\\
DML-CART	&	-0.027	&	0.051	&	0.859	&	-0.047	&	0.048	&	0.869	&	-0.049	&	0.050	&	0.961	\\
DML-RF	&	-0.025	&	0.046	&	0.883	&	0.003	&	0.015	&	0.823	&	-0.008	&	0.018	&	0.386	\\
DML-Boosting	&	-0.063	&	0.075	&	0.934	&	-0.045	&	0.047	&	0.921	&	-0.025	&	0.026	&	1.166	\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 100. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% DGP3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tp!]
\centering
 \caption{Simulation results, DGP3}\label{tab:collapse_dgp3}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=4,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: CRE   estimator}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.962	&	0.993	&	0.993	&	1.037	&	0.993	&	0.993	&	0.999	\\
DML-Lasso	&	1.013	&	1.013	&	0.993	&	1.000	&	1.000	&	1.185	&	0.997	&	0.997	&	0.955	\\
DML-Lasso\texttt{+}	&	0.103	&	0.130	&	1.062	&	0.021	&	0.049	&	0.778	&	0.009	&	0.014	&	1.235	\\
DML-CART	&	0.200	&	0.287	&	0.372	&	0.018	&	0.107	&	0.235	&	0.053	&	0.134	&	0.101	\\
DML-RF	&	0.705	&	0.760	&	0.234	&	0.268	&	0.485	&	0.108	&	0.151	&	0.440	&	0.056	\\
DML-Boosting	&	0.382	&	0.426	&	0.557	&	0.088	&	0.112	&	0.818	&	-0.007	&	0.039	&	0.792	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: WG hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.993	&	0.993	&	0.999	&	0.993	&	0.993	&	1.001	&	0.993	&	0.993	&	0.999	\\
DML-Lasso	&	0.989	&	0.989	&	0.908	&	0.992	&	0.992	&	0.965	&	0.993	&	0.993	&	0.998	\\
DML-Lasso\texttt{+}	&	0.010	&	0.031	&	1.152	&	-0.004	&	0.011	&	1.042	&	-0.022	&	0.022	&	1.017	\\
DML-CART	&	0.200	&	0.278	&	0.400	&	-0.001	&	0.102	&	0.238	&	0.049	&	0.136	&	0.096	\\
DML-RF	&	0.683	&	0.739	&	0.233	&	0.255	&	0.490	&	0.103	&	0.175	&	0.515	&	0.053	\\
DML-Boosting	&	0.435	&	0.461	&	0.707	&	0.090	&	0.125	&	0.763	&	-0.034	&	0.055	&	0.823	\\


\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: FD hybrid estimator}}\\
\vspace{-3mm}\\
OLS	&	0.992	&	0.992	&	0.964	&	0.993	&	0.993	&	0.974	&	0.993	&	0.993	&	0.950	\\
DML-Lasso	&	0.989	&	0.989	&	0.972	&	0.992	&	0.992	&	0.874	&	0.993	&	0.993	&	0.992	\\
DML-Lasso\texttt{+}	&	0.011	&	0.037	&	1.146	&	-0.005	&	0.014	&	1.005	&	-0.023	&	0.024	&	1.013	\\
DML-CART	&	0.200	&	0.281	&	0.410	&	0.000	&	0.102	&	0.250	&	0.050	&	0.137	&	0.101	\\
DML-RF	&	0.684	&	0.739	&	0.244	&	0.255	&	0.489	&	0.105	&	0.174	&	0.514	&	0.055	\\
DML-Boosting	&	0.436	&	0.464	&	0.697	&	0.089	&	0.126	&	0.767	&	-0.034	&	0.055	&	0.833	\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 100. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}


==> tabs/tab4_fazio2023.tex <==
\begin{table}[th!]
\centering
 \caption{Replication of Table 4 Specification (2)}\label{tab:fazio_t4}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-2mm}\\
	
& OLS & DML-OLS & DML-Lasso& DML-CART& DML-RF\\
\hline
\vspace{-2mm}\\
\multicolumn{5}{l}{\emph{Dependent variable: ``Tolerance for high incomes''}}\\
\vspace{-3mm}\\
NMW &0.084***&0.081***&0.083***&0.108***&0.088***\\
&(0.029)&(0.029)&(0.029)&(0.029)&(0.029)\\

% NMW &0.084***&0.081***&0.083***&0.109***&0.091***\\
% &(0.029)&(0.029)&(0.029)&(0.029)&(0.029)\\
\vspace{-3mm}\\
Basic controls&Yes&Yes&Yes&Yes&Yes\\
Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes\\
Income other members HH&Yes&Yes&Yes&Yes&Yes\\

\vspace{-3mm}\\
\multicolumn{6}{c}{\emph{Resampling Information}}  \\
No. folds&--&5&5&5&5\\
Folds per cluster&--&5&5&5&5\\
No. repeated sample splits&--&1&1&1&1\\
Cross-fitting&--&Yes&Yes&Yes&Yes\\
Score&--&PO&PO&PO&PO\\
%Score&--&IV&IV&IV&IV\\
DML algorithm&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: This table replicates Specification (2) in Table 4 in Fazio and Reggiani (2023). Column~(1) reports the results from the paper, the remaining use DML and different learners. Lasso uses $\lambda$ equivalent to minimum mean cross-validated error. Random forest (RF) is tuned doing a random grid search for $num.trees\in(5,100)$, $min.node.size\in(5,N/2)$, $max.depth\in(1,10)$. The number of observations is 31,115, and the number of individuals is 8,222. Standard errors (in parenthesis) are clustered at the individual level. * p < 0.10, ** p < 0.05, *** p < 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab4_fazio_new.tex <==
\begin{table}[th!]
\centering
 \caption{Replication of Table 4 Specification (2) \hyperlink{sec:nmv}{\beamergotobutton{Back}}}\label{tab:fazio4}
\scalebox{.55}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-2mm}\\
	
& OLS & DML-Lasso & DML-Lasso& DML-CART& DML-RF\\
\hline
\vspace{-2mm}\\
\multicolumn{5}{l}{\emph{Dependent variable: ``Tolerance for high incomes''}}\\
\vspace{-3mm}\\
NMW &0.084***&0.081***&0.083***&0.108***&0.088***\\
&(0.029)&(0.029)&(0.029)&(0.029)&(0.029)\\

\vspace{-3mm}\\
No. Observations&31,115&31,115&31,115&31,115&31,115\\
No. Groups&8,222&8,222&8,222&8,222&8,222\\
\vspace{-3mm}\\
Basic controls&Yes&Yes&Yes&Yes&Yes\\
Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes\\
Income other members HH&Yes&Yes&Yes&Yes&Yes\\
Augmented controls&No&No&Yes&No&No\\

\vspace{-3mm}\\
\multicolumn{6}{c}{\emph{Resampling Information}}  \\
Estimator&WG&WG-hybrid&WG-hybrid&WG-hybrid&WG-hybrid\\
No. folds&--&5&5&5&5\\
Folds per cluster&--&5&5&5&5\\
No. repeated sample splits&--&1&1&1&1\\
Cross-fitting&--&Yes&Yes&Yes&Yes\\
%Score&--&IV&IV&IV&IV\\
Score&--&PO&PO&PO&PO\\
DML algorithm&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: This table replicates Specification (2) in Table 4 in \cite{fazio2023} Column~(1) reports the results of the paper estimated using DID; the remaining use DML and different learners. Lasso uses $\lambda$ equivalent to minimum mean cross-validated error. Random forest (RF) and Regression Trees (CART) are tuned with a random grid search for  $min.node.size\in(5,N/2)$, $max.depth\in(1,10)$, and the $num.trees\in(5,100)$ for RF. The number of observations is 31,115, and the number of individuals is 8,222. Standard errors (in parenthesis) are clustered at the individual level. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab4_fazio_pres.tex <==
\begin{table}[th!]
\centering
 \caption{Replication of Table 4 Specification (2) \hyperlink{sec:nmv}{\beamergotobutton{Back}}}\label{tab:fazio4}
\scalebox{.55}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-2mm}\\
	
& OLS & DML-OLS & DML-Lasso& DML-CART& DML-RF\\
\hline
\vspace{-2mm}\\
\multicolumn{5}{l}{\emph{Dependent variable: ``Tolerance for high incomes''}}\\
\vspace{-3mm}\\
NMW &0.084***&0.081***&0.083***&0.108***&0.088***\\
&(0.029)&(0.029)&(0.029)&(0.029)&(0.029)\\

% NMW &0.084***&0.081***&0.083***&0.109***&0.091***\\
% &(0.029)&(0.029)&(0.029)&(0.029)&(0.029)\\
\vspace{-3mm}\\
Basic controls&Yes&Yes&Yes&Yes&Yes\\
Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes\\
Income other members HH&Yes&Yes&Yes&Yes&Yes\\

\vspace{-3mm}\\
\multicolumn{6}{c}{\emph{Resampling Information}}  \\
No. folds&--&5&5&5&5\\
Folds per cluster&--&5&5&5&5\\
No. repeated sample splits&--&1&1&1&1\\
Cross-fitting&--&Yes&Yes&Yes&Yes\\
Score&--&PO&PO&PO&PO\\
%Score&--&IV&IV&IV&IV\\
DML algorithm&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: This table replicates Specification (2) in Table 4 in \cite{fazio2023} Column~(1) reports the results of the paper estimated using DID; the remaining use DML and different learners. Lasso uses $\lambda$ equivalent to minimum mean cross-validated error. Random forest (RF) and Regression Trees (CART) are tuned with a random grid search for  $min.node.size\in(5,N/2)$, $max.depth\in(1,10)$, and the $num.trees\in(5,100)$ for RF. The number of observations is 31,115, and the number of individuals is 8,222. Standard errors (in parenthesis) are clustered at the individual level. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab5_fazio.tex <==
\begin{table}[th!]
\centering
 \caption{Replication  of Specification~(2) in Table~5 in \cite{fazio2023}}\label{tab:fazio5}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
  \begin{tabular}{lccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS& OLS& DML-Lasso & DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)&(6)&(7)\\
\hline
\vspace{-2mm}\\
\multicolumn{8}{l}{\emph{Dependent variable: ``Vote conservative''}}\\
&&&\multicolumn{5}{c}{\emph{Approximation approach}}\\
 \cmidrule(l{.35cm}r{.25cm}){4-8}
\vspace{-3mm}\\
NMW &0.097**&0.088**&0.095**&0.086***&0.091***&0.098***&\\
&(0.045)&(0.045)&(0.045)&(0.045)&(0.044)&(0.045)&\\
\vspace{-2mm}\\


&&&\multicolumn{5}{c}{\emph{Hybrid approach}}\\
 \cmidrule(l{.35cm}r{.25cm}){4-8}
\vspace{-3mm}\\
&&&0.093***&0.079**&0.091**&0.095***&0.217\\
&&&(0.045)&(0.045)&(0.042)&(0.048)&(0.133)\\

\vspace{-2mm}\\
\hline
\vspace{-2mm}\\

%Controls vars&Yes&Yes&Yes&Yes&Yes&Yes\\
%Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes&Yes&Yes\\
%Wave x Region FE&No&Yes&No&Yes&No&No&No\\
Extended dictionary&No&No&No&Yes&No&No&No\\

%Income other members HH&Yes&Yes&Yes&Yes&Yes\\
%No. control vars&37&37&1,408&37&37\\
\vspace{-3mm}\\
No. Observations&19,961&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927&4,927&4,927\\

% \vspace{-2mm}\\
% \hline 
% \vspace{-2mm}\\
% \multicolumn{7}{c}{\emph{Resampling Information}}  \\
% \vspace{-3mm}\\

% Estimator&WG&WG&WG&WG&WG&WG\\
% No. folds&--&--&5&5&5&5\\
% %Folds per cluster&--&--&5&5&5&5\\
% %No. repeated sample splits&--&--&1&1&1&1\\
% Cross-fitting&--&--&Yes&Yes&Yes&Yes\\
% %Score&--&IV&IV&IV&IV\\
% Score&--&--&PO&PO&PO&PO\\
% DML algorithm&--&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: Column~(1) reports the original figures of Specification~(2) in Table~5 in \cite{fazio2023} estimated using least squares;  Column~(2) adds the interaction between wave and region fixed effects to Column~(1); remaining columns use DML with different learners. Base control variables include: age, age squared (not for CART and RF), education, marital status, household size, income of other members. Column~(4) uses an extended dictionary of non-linear terms of the control variables and fixed effects (i.e., polynomials of order three and interactions of the control variables). The hybrid approach includes the individual means of the control variables and fixed effects. Standard errors (in parenthesis) are clustered at the individual level.  Standard errors (in parenthesis) are clustered at the individual level. Resampling information: 5 folds, cross-fitting, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab5_fazio_hybrid.tex <==
\begin{table}[th!]
\centering
 \caption{Replication Results with WG-hybrid estimator}\label{tab:fazio5_hybrid}
\scalebox{.85}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lcccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS& OLS & DML-Lasso & DML-Lasso& DML-CART& DML-RF\\
&(1)&(2)&(3)&(4)&(5)&(6)\\
\hline
\vspace{-2mm}\\
\multicolumn{7}{l}{\emph{Dependent variable: ``Vote conservative''}}\\
\vspace{-3mm}\\
NMW &0.097**&0.088**&0.093***&0.079**&0.089**&0.131**\\
&(0.045)&(0.045)&(0.045)&(0.045)&(0.05)&(0.074)\\

% NMW &0.097**&0.088**&0.093***&0.079**&0.077&0.131**\\
% &(0.045)&(0.045)&(0.045)&(0.045)&(0.053)&(0.074)\\
% cp minsplit maxdepth learner_param_vals  x_domain   regr.mse
% 0.02     2464        8          <list[4]> <list[3]> 0.09201294
\vspace{-3mm}\\

No. Observations&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927&4,927\\


\vspace{-3mm}\\
% Controls vars&Yes&Yes&Yes&Yes&Yes&Yes\\
% %Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes&Yes\\
Wave x Region FE&No&Yes&No&Yes&No&No\\
Extended dictionary&No&No&No&Yes&No&No\\
%Income other members HH&Yes&Yes&Yes&Yes&Yes\\
%No. control vars&37&37&1,408&37&37\\
\vspace{-3mm}\\
\hline 
\multicolumn{7}{c}{\emph{Resampling Information}}  \\
\vspace{-3mm}\\

Estimator&WG&WG&WG&WG&WG&WG\\
No. folds&--&--&5&5&5&5\\
Folds per cluster&--&--&5&5&5&5\\
No. repeated sample splits&--&--&1&1&1&1\\
Cross-fitting&--&--&Yes&Yes&Yes&Yes\\
%Score&--&IV&IV&IV&IV\\
Score&--&--&PO&PO&PO&PO\\
DML algorithm&--&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: Column~(1) reports the original figures of Specification~(2) in Table~5 in \cite{fazio2023} estimated using least squares;  Column~(2) adds the interaction between wave and region fixed effects to Column~(1); remaining columns use DML with different learners. Base control variables include: age, age squared (not for CART and RF), education, marital status, household size, income of other members, and their individual means. Column~(4) uses an extended dictionary of non-linear terms of the control variables and fixed effects (i.e., polynomials of order three and interactions of the control variables and their individual means). Standard errors (in parenthesis) are clustered at the individual level. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab5_fazio_hybrid_pres.tex <==
\begin{table}[th!]
\centering
% \caption{Replication Results with WG-hybrid estimator}
\label{tab:fazio5_hybrid}
\scalebox{.6}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lcccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS& OLS & DML-Lasso & DML-Lasso& DML-CART& DML-RF\\
&(1)&(2)&(3)&(4)&(5)&(6)\\
\hline
\vspace{-2mm}\\
\multicolumn{7}{l}{\emph{Dependent variable: ``Vote conservative''}}\\
\vspace{-3mm}\\
NMW &0.097**&0.088**&0.093***&0.079**&0.089**&0.149\\
&(0.045)&(0.045)&(0.045)&(0.045)&(0.05)&(0.127)\\

\vspace{-3mm}\\

No. Observations&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927&4,927\\


\vspace{-3mm}\\
Controls vars&Yes&Yes&Yes&Yes&Yes&Yes\\
%Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes&Yes\\
Wave x Region FE&No&Yes&No&Yes&No&No\\

%Income other members HH&Yes&Yes&Yes&Yes&Yes\\
%No. control vars&37&37&1,408&37&37\\
\vspace{-3mm}\\
\hline 
\multicolumn{7}{c}{\emph{Resampling Information}}  \\
\vspace{-3mm}\\

Estimator&WG&WG&WG-hybrid&WGG-hybrid&WGG-hybrid&WGG-hybrid\\
No. folds&--&--&5&5&5&5\\
Folds per cluster&--&--&5&5&5&5\\
No. repeated sample splits&--&--&1&1&1&1\\
Cross-fitting&--&--&Yes&Yes&Yes&Yes\\
%Score&--&IV&IV&IV&IV\\
Score&--&--&PO&PO&PO&PO\\
DML algorithm&--&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: Column~(1) reports the figures of Specification~(2) in Table~5 in \cite{fazio2023} estimated using least squares;  Column~(2) is LS regression with controls from Column~(1) and interaction terms between wave and region fixed effects; remaining columns use DML with different (tuned) learners. Control variables include: age,  education, marital status, household size, income of other members, and their individual means. Age squared and is included in Columns~(1)-(3). Standard errors (in parenthesis) are clustered at the individual level. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.} \hyperlink{sec:simres}{\beamergotobutton{Back}}
\end{tablenotes}
\end{threeparttable}}
\end{table}

%%cart w/t age2

==> tabs/tab5_fazio_noFE.tex <==
\begin{table}[th!]
\centering
 \caption{Replication Results without fixed effects, WG estimator}\label{tab:fazio5_noFE}
\scalebox{.9}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lcccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\	
& OLS& DML-Lasso & DML-Lasso& DML-CART& DML-RF& DML-Boosting\\
&(1)&(2)&(3)&(4)&(5)&(6)\\
\hline
\vspace{-2mm}\\
\multicolumn{7}{l}{\emph{Dependent variable: ``Vote conservative''}}\\
&&\multicolumn{5}{c}{\emph{Approximation approach}}\\
 \cmidrule(l{.35cm}r{.25cm}){3-7}
\vspace{-3mm}\\
NMW &0.101**&0.099***&0.103***&0.091***&0.099***&\red{0.099}***\\
&(0.044)&(0.045)&(0.044)&(0.044)&(0.044)&(0.039)\\

\vspace{-2mm}\\
&&\multicolumn{5}{c}{\emph{Hybrid approach}}\\
 \cmidrule(l{.35cm}r{.25cm}){3-7}
\vspace{-3mm}\\
 &&0.100***&0.100***&0.091***&0.101***&0.099***\\
&&(0.044)&(0.045)&(0.044)&(0.045)&(0.039)\\

\vspace{-2mm}\\
\hline
\vspace{-2mm}\\
Extended dictionary&No&No&Yes&No&No&No\\
Region and wave FE&No&No&No&No&No&No\\

\vspace{-3mm}\\
No. Observations&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927&4,927\\
% \vspace{-3mm}\\
% \hline 
% \vspace{-2mm}\\
% \multicolumn{6}{c}{\emph{Resampling Information}}  \\
% \vspace{-2mm}\\

% Estimator&WG&WG&WG&WG&WG&WG\\
% No. folds&--&5&5&5&5&5\\
% %Folds per cluster&--&5&5&5&5\\
% %No. repeated sample splits&--&1&1&1&1\\
% Cross-fitting&--&Yes&Yes&Yes&Yes&Yes\\
% %Score&--&IV&IV&IV&IV\\
% Score&--&PO&PO&PO&PO\\
% DML algorithm&--&2&2&2&2\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: Column~(1) reports the least squares estimates based on Specification~(2) in Table~5 in \cite{fazio2023} without wave and region fixed effects; remaining columns use DML with different learners. Base control variables include: age, age squared (not for CART and RF), education, marital status, household size, income of other members, and their individual means. Column~(3) uses an extended dictionary of non-linear terms of the control variables (i.e., polynomials of order three and interactions of the control variables and their individual means). The hybrid approach includes the individual means of the control variables and fixed effects. Standard errors (in parenthesis) are clustered at the individual level. Resampling information: 5 folds, cross-fitting, PO score, DML algorithm 2. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab5_fazio_pres.tex <==
\begin{table}[th!]
\centering
 \caption{Replication with WG `approximate' estimator}\label{tab:fazio5}
\scalebox{.6}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lccccc}   
\vspace{-5mm}\\   
\hline\hline
\vspace{-3mm}\\
	
& OLS &DML-Lasso & DML-Lasso+& DML-CART& DML-RF\\
\hline
\vspace{-2mm}\\
\multicolumn{5}{l}{\emph{Dependent variable: ``Vote conservative''}}\\
\vspace{-3mm}\\
% NMW &0.097**&0.094**&0.095**&0.094**&0.097**\\
% &(0.045)&(0.045)&(0.045)&(0.044)&(0.045)\\

NMW &0.097**&0.095**&0.086***&0.094**&0.096**\\
&(0.045)&(0.045)&(0.045)&(0.044)&(0.045)\\

\vspace{-2mm}\\

No. Observations&19,961&19,961&19,961&19,961&19,961&19,961\\
No. Groups&4,927&4,927&4,927&4,927&4,927\\

\vspace{-3mm}\\
Basic controls&Yes&Yes&Yes&Yes&Yes\\
Individual FE&Yes&Yes&Yes&Yes&Yes\\
Wave FE&Yes&Yes&Yes&Yes&Yes\\
Region FE&Yes&Yes&Yes&Yes&Yes\\
Income other members HH&Yes&Yes&Yes&Yes&Yes\\
No. control vars&37&37&1,408&37&37\\
\vspace{-3mm}\\
\hline 
\multicolumn{6}{c}{\emph{Resampling Information}}  \\
\vspace{-3mm}\\

Estimator&WG&WG&WG&WG&WG\\
No. folds&--&5&5&5&5\\
Folds per cluster&--&5&5&5&5\\
No. repeated sample splits&--&1&1&1&1\\
Cross-fitting&--&Yes&Yes&Yes&Yes\\
%Score&--&IV&IV&IV&IV\\
Score&--&PO&PO&PO&PO\\
DML algorithm&--&2&2&2&2\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{Note: Column~(1) reports the figures of Specification~(2) in Table~5 in \cite{fazio2023} estimated using least squares; the remaining use DML with different (tuned) learners.  Standard errors (in parenthesis) are clustered at the individual level. * p $<$ 0.10, ** p $<$ 0.05, *** p $<$ 0.01.}
\end{tablenotes}
\end{threeparttable}}
\end{table}



==> tabs/tab_bin_iv.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with binary treatment, nonlinear functions and IV scores}
\scalebox{.7}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lccccccccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}&\multicolumn{5}{c}{Under FE (DGP3)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}\cmidrule(l{.35cm}r{.25cm}){12-16}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias \\
\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.506	&	0.090	&	0.092	&	0.008	&	-0.006	&	0.508	&	0.093	&	0.091	&	0.009	&	-0.008	&	0.504	&	0.085	&	0.083	&	0.007	&	-0.004	\\
LASSO&0.515	&	0.088	&	0.086	&	0.008	&	-0.015	&	0.517	&	0.091	&	0.086	&	0.009	&	-0.017	&	0.504	&	0.083	&	0.080	&	0.007	&	-0.004	\\
CART&0.521	&	0.093	&	0.091	&	0.009	&	-0.021	&	0.523	&	0.093	&	0.090	&	0.009	&	-0.023	&	0.507	&	0.083	&	0.080	&	0.007	&	-0.007	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.506	&	0.029	&	0.028	&	0.001	&	-0.006	&	0.507	&	0.028	&	0.028	&	0.001	&	-0.007	&	0.498	&	0.025	&	0.025	&	0.001	&	0.002	\\
LASSO&0.507	&	0.029	&	0.028	&	0.001	&	-0.007	&	0.508	&	0.028	&	0.028	&	0.001	&	-0.008	&	0.498	&	0.025	&	0.025	&	0.001	&	0.002	\\
CART&0.527	&	0.029	&	0.028	&	0.002	&	-0.027	&	0.525	&	0.029	&	0.028	&	0.001	&	-0.025	&	0.503	&	0.026	&	0.025	&	0.001	&	-0.003	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.507	&	0.008	&	0.009	&	0.000	&	-0.007	&	0.506	&	0.008	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
LASSO&0.507	&	0.008	&	0.009	&	0.000	&	-0.007	&	0.506	&	0.008	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
CART&0.531	&	0.009	&	0.009	&	0.001	&	-0.031	&	0.530	&	0.010	&	0.009	&	0.001	&	-0.030	&	0.504	&	0.008	&	0.008	&	0.000	&	-0.004	\\

\vspace{-2mm}\\

\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.503	&	0.115	&	0.112	&	0.013	&	-0.003	&	0.503	&	0.110	&	0.112	&	0.012	&	-0.003	&	0.502	&	0.107	&	0.101	&	0.011	&	-0.002	\\
LASSO&0.511	&	0.110	&	0.105	&	0.012	&	-0.011	&	0.510	&	0.107	&	0.104	&	0.012	&	-0.010	&	0.501	&	0.102	&	0.096	&	0.010	&	-0.001	\\
CART&0.523	&	0.114	&	0.108	&	0.014	&	-0.023	&	0.526	&	0.114	&	0.107	&	0.014	&	-0.026	&	0.498	&	0.098	&	0.097	&	0.010	&	0.002	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.504	&	0.035	&	0.034	&	0.001	&	-0.004	&	0.504	&	0.034	&	0.034	&	0.001	&	-0.004	&	0.495	&	0.030	&	0.031	&	0.001	&	0.005	\\
LASSO&0.505	&	0.035	&	0.034	&	0.001	&	-0.005	&	0.505	&	0.034	&	0.033	&	0.001	&	-0.005	&	0.495	&	0.030	&	0.030	&	0.001	&	0.005	\\
CART&0.528	&	0.035	&	0.034	&	0.002	&	-0.028	&	0.528	&	0.036	&	0.034	&	0.002	&	-0.028	&	0.496	&	0.031	&	0.031	&	0.001	&	0.004	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.505	&	0.010	&	0.011	&	0.000	&	-0.005	&	0.503	&	0.010	&	0.011	&	0.000	&	-0.003	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
LASSO&0.505	&	0.010	&	0.011	&	0.000	&	-0.005	&	0.503	&	0.010	&	0.011	&	0.000	&	-0.003	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
CART&0.535	&	0.011	&	0.011	&	0.001	&	-0.035	&	0.533	&	0.011	&	0.011	&	0.001	&	-0.033	&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are non-linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_bin_lin_iv.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with binary treatment, linear functions and IV scores}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lcccccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias	&		$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias\\
\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.505	&	0.093	&	0.092	&	0.009	&	-0.005	&	0.499	&	0.091	&	0.092	&	0.008	&	0.001	\\
LASSO	&0.516	&	0.089	&	0.086	&	0.008	&	-0.016	&	0.510	&	0.089	&	0.086	&	0.008	&	-0.010	\\
CART&0.555	&	0.098	&	0.097	&	0.013	&	-0.055	&	0.551	&	0.100	&	0.097	&	0.013	&	-0.051	\\
RF1	&0.691	&	0.147	&	0.121	&	0.058	&	-0.191	&	0.692	&	0.142	&	0.121 &		0.057	&	-0.192		\\
RF5	&0.703	&	0.100	&	0.093	&	0.051	&	-0.203	&	0.697	&	0.099	&	0.093	&	0.048	&	-0.197	\\
RF10	&0.705	&	0.095	&	0.090	&	0.051	&	-0.205	&	0.699	&	0.094	&	0.090	&	0.049	&	-0.199	\\

\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.504	&	0.028	&	0.028	&	0.001	&	-0.004	&	0.498	&	0.028	&	0.028	&	0.001	&	0.002	\\
LASSO	&0.505	&	0.028	&	0.028	&	0.001	&	-0.005	&	0.499	&	0.028	&	0.028	&	0.001	&	0.001	\\
CART&0.633	&	0.032	&	0.029	&	0.019	&	-0.133	&	0.630	&	0.032	&	0.029	&	0.018	&	-0.130	\\
RF1	&0.676	&	0.072	&	0.032	&	0.036	&	-0.176	&	0.673	&	0.075	&	0.032&		0.035	&	-0.173	\\
RF5	&0.677	&	0.038	&	0.028	&	0.033	&	-0.177	&	0.673	&	0.039	&	0.028	&	0.031	&	-0.173	\\
RF10	&0.676	&	0.033	&	0.028	&	0.032	&	-0.176	&	0.672	&	0.033	&	0.028	&	0.031	&	-0.172	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.503	&	0.008	&	0.009	&	0.000	&	-0.003	&	0.499	&	0.008	&	0.009	&	0.000	&	0.001	\\
LASSO	&0.503	&	0.008	&	0.009	&	0.000	&	-0.003	&	0.499	&	0.008	&	0.009	&	0.000	&	0.001	\\
CART&0.649	&	0.014	&	0.009	&	0.022	&	-0.149	&	0.647	&	0.014	&	0.009	&	0.022	&	-0.147	\\
RF1	&0.691	&	0.066	&	0.010	&	0.041	&	-0.191	&	0.688 &0.068	&	0.010	&	0.040	&	-0.188	\\
RF5	&0.695	&	0.027	&	0.009	&	0.039	&	-0.195	&	0.691	&	0.027	&	0.009	&	0.037	&	-0.191	\\
RF10	&0.696	&	0.020	&	0.009	&	0.039	&	-0.196	&	0.692	&	0.020	&	0.009	&	0.037	&	-0.192	\\


\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.508	&	0.116	&	0.113	&	0.014	&	-0.008	&	0.498	&	0.113	&	0.112	&	0.013	&	0.002	\\
LASSO	&0.515	&	0.111	&	0.105	&	0.013	&	-0.015	&	0.507	&	0.109	&	0.105	&	0.012	&	-0.007	\\
CART&0.560	&	0.119	&	0.116	&	0.018	&	-0.060	&	0.551	&	0.116	&	0.115	&	0.016	&	-0.051	\\
RF1	&0.706	&	0.159	&	0.139	&	0.068	&	-0.206	&	0.703	&	0.158	&	0.139	&	0.066	&	-0.203	\\
RF5	&0.715	&	0.117	&	0.111	&	0.060	&	-0.215	&	0.713	&	0.118	&	0.111	&	0.059	&	-0.213	\\
RF10	&0.720	&	0.113	&	0.107	&	0.061	&	-0.220	&	0.715	&	0.113	&	0.107	&	0.059	&	-0.215	\\

\vspace{-3mm}\\

\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.505	&	0.034	&	0.034	&	0.001	&	-0.005	&	0.497	&	0.034	&	0.034	&	0.001	&	0.003	\\
LASSO &0.505	&	0.034	&	0.034	&	0.001	&	-0.005	&	0.498	&	0.034	&	0.033	&	0.001	&	0.002	\\
CART&0.641	&	0.038	&	0.034	&	0.021	&	-0.141	&	0.635	&	0.037	&	0.034	&	0.020	&	-0.135	\\
RF1	&0.681	&	0.075	&	0.037	&	0.039	&	-0.181	&	0.671	&	0.074	&	0.037	&	0.035		&-0.171	\\
RF5	&0.684	&	0.043	&	0.034	&	0.036	&	-0.184	&	0.678	&	0.042	&	0.034	&	0.034	&	-0.178	\\
RF10	&0.684	&	0.038	&	0.033	&	0.035	&	-0.184	&	0.678	&	0.038	&	0.033	&	0.033	&	-0.178	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.503	&	0.010	&	0.011	&	0.000	&	-0.003	&	0.498	&	0.010	&	0.011	&	0.000	&	0.002	\\
LASSO	&0.503	&	0.010	&	0.011	&	0.000	&	-0.003	&	0.498	&	0.010	&	0.011	&	0.000	&	0.002	\\
CART&0.665	&	0.016	&	0.011	&	0.028	&	-0.165	&	0.661	&	0.017	&	0.011	&	0.026	&	-0.161	\\
RF1	&0.700	&	0.066	&	0.011	&	0.044	&	-0.200	&	0.695	&	0.067	&	0.011	&	0.043	&	-0.195	\\
RF5	&0.701	&	0.028	&	0.011	&	0.041	&	-0.201	&	0.697	&	0.028	&	0.011	&	0.040	&	-0.197	\\
RF10	&0.702	&	0.020	&	0.011	&	0.041	&	-0.202	&	0.698	&	0.021	&	0.011	&	0.040	&	-0.198	\\



\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_bin_lin_po.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with binary treatment, linear functions and PO scores}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lcccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias\\
\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.503	&	0.091	&	0.088	&	0.008	&	-0.003	&	0.500	&	0.093	&	0.088	&	0.009	&	0.000	\\
LASSO	&0.510	&	0.088	&	0.088	&	0.008	&	-0.010	&	0.508	&	0.090	&	0.088	&	0.008	&	-0.008	\\
CART&0.507	&	0.090	&	0.088	&	0.008	&	-0.007	&	0.508	&	0.092	&	0.088	&	0.009	&	-0.008	\\
RF1	&0.513	&	0.111	&	0.096	&	0.013	&	-0.013	&	0.513	&	0.117	&	0.096	&	0.014	&	-0.013	\\
RF5	&0.655	&	0.094	&	0.093	&	0.033	&	-0.155	&	0.651	&	0.095	&	0.093	&	0.032	&	-0.151	\\
RF10	&0.678	&	0.089	&	0.092	&	0.040	&	-0.178	&	0.676	&	0.093	&	0.092	&	0.040	&	-0.176	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.504	&	0.028	&	0.028	&	0.001	&	-0.004	&	0.500	&	0.028	&	0.028	&	0.001	&	0.000	\\
LASSO	&0.505	&	0.028	&	0.028	&	0.001	&	-0.005	&	0.500	&	0.028	&	0.028	&	0.001	&	0.000	\\
CART&0.619	&	0.032	&	0.029	&	0.015	&	-0.119	&	0.616	&	0.032	&	0.029	&	0.014	&	-0.116	\\
RF1	&0.611	&	0.071	&	0.031	&	0.017	&	-0.111	&	0.606	&	0.068	&	0.031	&	0.016	&	-0.106	\\
RF5	&0.664	&	0.038	&	0.029	&	0.028	&	-0.164	&	0.661	&	0.040	&	0.029	&	0.027	&	-0.161	\\
RF10	&0.673	&	0.033	&	0.029	&	0.031	&	-0.173	&	0.670	&	0.034	&	0.029	&	0.030	&	-0.170	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.502	&	0.009	&	0.009	&	0.000	&	-0.002	&	0.500	&	0.008	&	0.009	&	0.000	&	0.000	\\
LASSO	&0.502	&	0.009	&	0.009	&	0.000	&	-0.002	&	0.500	&	0.008	&	0.009	&	0.000	&	0.000	\\
CART&0.629	&	0.016	&	0.009	&	0.017	&	-0.129	&	0.627	&	0.015	&	0.009	&	0.016	&	-0.127	\\
RF1	&0.657	&	0.070	&	0.010	&	0.030	&	-0.157	&	0.651	&	0.067	&	0.010	&	0.027	&	-0.151	\\
RF5	&0.688	&	0.028	&	0.009	&	0.036	&	-0.188	&	0.685	&	0.029	&	0.009	&	0.035	&	-0.185	\\
RF10&0.692	&	0.021	&	0.009	&	0.037	&	-0.192	&	0.689	&	0.021	&	0.009	&	0.036	&	-0.189	\\

\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.498	&	0.117	&	0.106	&	0.014	&	0.002	&	0.500	&	0.114	&	0.106	&	0.013	&	0.000	\\
LASSO	&0.504	&	0.111	&	0.106	&	0.012	&	-0.004	&	0.505	&	0.110	&	0.106	&	0.012	&	-0.005	\\
CART&0.491	&	0.106	&	0.103	&	0.011	&	0.009	&	0.492	&	0.106	&	0.102	&	0.011	&	0.008	\\
RF1&0.509	&	0.126	&	0.110	&	0.016	&	-0.009	&	0.513	&	0.125	&	0.110	&	0.016	&	-0.013	\\
RF5&0.661	&	0.114	&	0.110	&	0.039	&	-0.161	&	0.661	&	0.111	&	0.110	&	0.038	&	-0.161	\\
RF10	&0.684	&	0.111	&	0.110	&	0.046	&	-0.184	&	0.686	&	0.109	&	0.110	&	0.047	&	-0.186	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.506	&	0.033	&	0.034	&	0.001	&	-0.006	&	0.498	&	0.034	&	0.034	&	0.001	&	0.002	\\
LASSO	&0.506	&	0.033	&	0.034	&	0.001	&	-0.006	&	0.498	&	0.034	&	0.034	&	0.001	&	0.002	\\
CART&0.623	&	0.038	&	0.034	&	0.017	&	-0.123	&	0.618	&	0.037	&	0.034	&	0.015	&	-0.118	\\
RF1	&0.618	&	0.070	&	0.036	&	0.019	&	-0.118	&	0.609	&	0.070	&	0.036	&	0.017	&	-0.109	\\
RF5	&0.675	&	0.044	&	0.035	&	0.032	&	-0.175	&	0.668	&	0.043	&	0.035	&	0.030	&	-0.168	\\
RF10	&0.681	&	0.038	&	0.035	&	0.034	&	-0.181	&	0.675	&	0.038	&	0.035	&	0.032	&	-0.175	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.502	&	0.010	&	0.011	&	0.000	&	-0.002	&	0.498	&	0.010	&	0.011	&	0.000	&	0.002	\\
LASSO	&0.502	&	0.010	&	0.011	&	0.000	&	-0.002	&	0.498	&	0.010	&	0.011	&	0.000	&	0.002	\\
CART&0.635	&	0.017	&	0.011	&	0.019	&	-0.135	&	0.632	&	0.016	&	0.011	&	0.018	&	-0.132	\\
RF1&	0.659	&	0.066	&	0.012	&	0.030	&	-0.159	&	0.657	&	0.069	&	0.012	&	0.029	&	-0.157	\\
RF5	&0.697	&	0.030	&	0.011	&	0.040	&	-0.197	&	0.692	&	0.029	&	0.011	&	0.038	&	-0.192	\\
RF10	&0.702	&	0.022	&	0.011	&	0.041	&	-0.202	&	0.697	&	0.022	&	0.011	&	0.039	&	-0.197	\\


\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.  $\widehat{l}(.)$ and $\widehat{m}(.)$ are linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_bin_po.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with binary treatment, nonlinear functions and PO scores}
\scalebox{.7}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lccccccccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}&\multicolumn{5}{c}{Under FE (DGP3)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}\cmidrule(l{.35cm}r{.25cm}){12-16}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias \\
\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.504	&	0.092	&	0.088	&	0.009	&	-0.004	&	0.505	&	0.091	&	0.087	&	0.008	&	-0.005	&	0.498	&	0.083	&	0.079	&	0.007	&	0.002	\\
LASSO&0.512	&	0.089	&	0.088	&	0.008	&	-0.012	&	0.512	&	0.088	&	0.088	&	0.008	&	-0.012	&	0.497	&	0.080	&	0.080	&	0.006	&	0.003	\\
CART&0.511	&	0.088	&	0.089	&	0.008	&	-0.011	&	0.507	&	0.092	&	0.088	&	0.008	&	-0.007	&	0.494	&	0.080	&	0.080	&	0.006	&	0.006	\\

% RF1	&0.406	&	0.090	&	0.085	&	0.017	&	0.094	&	0.406	&	0.090	&	0.085	&	0.017	&	0.094	\\
% RF5	&0.510	&	0.087	&	0.087	&	0.008	&	-0.010	&	0.509	&	0.088	&	0.086	&	0.008	&	-0.009	\\
% RF10	&0.526	&	0.087	&	0.087	&	0.008	&	-0.026	&	0.526	&	0.087	&	0.086	&	0.008	&	-0.026	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.507	&	0.029	&	0.028	&	0.001	&	-0.007	&	0.507	&	0.028	&	0.028	&	0.001	&	-0.007	&	0.499	&	0.025	&	0.025	&	0.001	&	0.001	\\
LASSO&0.508	&	0.029	&	0.028	&	0.001	&	-0.008	&	0.508	&	0.028	&	0.028	&	0.001	&	-0.008	&	0.500	&	0.025	&	0.025	&	0.001	&	0.000	\\
CART&0.519	&	0.028	&	0.028	&	0.001	&	-0.019	&	0.518	&	0.028	&	0.028	&	0.001	&	-0.018	&	0.498	&	0.024	&	0.025	&	0.001	&	0.002	\\
% RF1	&	0.486	&	0.034	&	0.027	&	0.001	&	0.014	&	0.485	&	0.033	&	0.027	&	0.001	&	0.015	\\
% RF5	&	0.527	&	0.029	&	0.028	&	0.002	&	-0.027	&	0.526	&	0.029	&	0.027	&	0.001	&	-0.026	\\
% RF10	&0.532	&	0.029	&	0.028	&	0.002	&	-0.032	&	0.531	&	0.028	&	0.028	&	0.002	&	-0.031	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.507	&	0.008	&	0.009	&	0.000	&	-0.007	&	0.506	&	0.009	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
LASSO&0.508	&	0.008	&	0.009	&	0.000	&	-0.008	&	0.506	&	0.009	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
CART&0.529	&	0.010	&	0.009	&	0.001	&	-0.029	&	0.528	&	0.010	&	0.009	&	0.001	&	-0.028	&	0.497	&	0.008	&	0.008	&	0.000	&	0.003	\\

% RF1	&	0.508	&	0.021	&	0.009	&	0.001	&	-0.008	&	0.507	&	0.020	&	0.009	&	0.000	&	-0.007	\\
% RF5	&0.535	&	0.010	&	0.009	&	0.001	&	-0.035	&	0.534	&	0.011	&	0.009	&	0.001	&	-0.034	\\
% RF10	&0.538	&	0.009	&	0.009	&	0.002	&	-0.038	&	0.537	&	0.010	&	0.009	&	0.001	&	-0.037	\\

\vspace{-2mm}\\

\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.113	&	0.105	&	0.013	&	-0.001	&	0.502	&	0.108	&	0.105	&	0.012	&	-0.002	&	0.497	&	0.105	&	0.095	&	0.011	&	0.003	\\
LASSO&0.507	&	0.108	&	0.106	&	0.012	&	-0.007	&	0.506	&	0.103	&	0.105	&	0.011	&	-0.006	&	0.496	&	0.099	&	0.095	&	0.010	&	0.004	\\
CART&0.501	&	0.105	&	0.105	&	0.011	&	-0.001	&	0.501	&	0.103	&	0.104	&	0.011	&	-0.001	&	0.487	&	0.096	&	0.095	&	0.009	&	0.013	\\

% RF1& 0.399	&	0.096	&	0.097	&	0.019	&	0.101	&	0.401	&	0.096	&	0.097	&	0.019	&	0.099	\\
% RF5&0.510	&	0.103	&	0.102	&	0.011	&	-0.010	&	0.510	&	0.098	&	0.102	&	0.010	&	-0.010	\\
% RF10	&0.528	&	0.104	&	0.103	&	0.012	&	-0.028	&	0.528	&	0.097	&	0.103	&	0.010	&	-0.028	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.507	&	0.035	&	0.034	&	0.001	&	-0.007	&	0.505	&	0.034	&	0.034	&	0.001	&	-0.005	&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\
LASSO&0.506	&	0.035	&	0.034	&	0.001	&	-0.006	&	0.505	&	0.034	&	0.034	&	0.001	&	-0.005	&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\
CART&0.521	&	0.034	&	0.034	&	0.002	&	-0.021	&	0.518	&	0.034	&	0.033	&	0.001	&	-0.018	&	0.498	&	0.030	&	0.031	&	0.001	&	0.002	\\
% RF1	&0.488	&	0.037	&	0.032	&	0.002	&	0.012	&	0.486	&	0.037	&	0.032	&	0.002	&	0.014	\\
% RF5	&0.530	&	0.035	&	0.033	&	0.002	&	-0.030	&	0.528	&	0.033	&	0.033	&	0.002	&	-0.028	\\
% RF10	&0.535	&	0.034	&	0.033	&	0.002	&	-0.035	&	0.534	&	0.033	&	0.033	&	0.002	&	-0.034	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.505	&	0.010	&	0.011	&	0.000	&	-0.005	&	0.504	&	0.010	&	0.011	&	0.000	&	-0.004	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
LASSO&0.506	&	0.010	&	0.011	&	0.000	&	-0.006	&	0.504	&	0.010	&	0.011	&	0.000	&	-0.004	&	0.498	&	0.009	&	0.010	&	0.000	&	0.002	\\
CART&0.532	&	0.011	&	0.011	&	0.001	&	-0.032	&	0.529	&	0.011	&	0.011	&	0.001	&	-0.029	&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\

 % RF1	&0.510	&	0.021	&	0.010	&	0.001	&	-0.010	&	0.508	&	0.020	&	0.010	&	0.000	&	-0.008	\\
 % RF5	&0.537	&	0.012	&	0.010	&	0.002	&	-0.037	&	0.535	&	0.012	&	0.010	&	0.001	&	-0.035	\\
 % RF10	&0.541	&	0.011	&	0.010	&	0.002	&	-0.041	&	0.539	&	0.011	&	0.010	&	0.002	&	-0.039	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are non-linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_bin_po_underFE.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with binary treatment, PO scores}
\scalebox{.8}{
\begin{threeparttable}
   \label{tab:}
   \begin{tabular}{lcccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{DGP1}&\multicolumn{5}{c}{DGP2}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}	
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  \\
\hline
\vspace{-2mm}\\
\multicolumn{11}{c}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&	0.500	&	0.093	&	0.088	&	0.009	&	0.000	&	0.498	&	0.083	&	0.079	&	0.007	&	0.002	\\
LASSO&	0.508	&	0.090	&	0.088	&	0.008	&	-0.008	&	0.497	&	0.080	&	0.080	&	0.006	&	0.003	\\
CART&	0.508	&	0.092	&	0.088	&	0.009	&	-0.008	&	0.494	&	0.080	&	0.080	&	0.006	&	0.006	\\
RF&		&		&		&		&		&	0.495	&	0.079	&	0.079	&	0.006	&	0.005	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&	0.500	&	0.028	&	0.028	&	0.001	&	0.000	&	0.499	&	0.025	&	0.025	&	0.001	&	0.001	\\
LASSO&	0.500	&	0.028	&	0.028	&	0.001	&	0.000	&	0.500	&	0.025	&	0.025	&	0.001	&	0.000	\\
CART&	0.616	&	0.032	&	0.029	&	0.014	&	-0.116	&	0.498	&	0.024	&	0.025	&	0.001	&	0.002	\\
RF&		&		&		&		&		&	0.496	&	0.024	&	0.025	&	0.001	&	0.004	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&	0.500	&	0.008	&	0.009	&	0.000	&	0.000	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
LASSO&	0.500	&	0.008	&	0.009	&	0.000	&	0.000	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
CART&	0.627	&	0.015	&	0.009	&	0.016	&	-0.127	&	0.497	&	0.008	&	0.008	&	0.000	&	0.003	\\
RF&		&		&		&		&		&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\


\vspace{-2mm}\\

\hline
\vspace{-2mm}\\
\multicolumn{11}{c}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&0.500	&	0.114	&	0.106	&	0.013	&	0.000	&	0.497	&	0.105	&	0.095	&	0.011	&	0.003	\\
LASSO&0.505	&	0.110	&	0.106	&	0.012	&	-0.005	&	0.496	&	0.099	&	0.095	&	0.010	&	0.004	\\
CART&0.492	&	0.106	&	0.102	&	0.011	&	0.008	&	0.487	&	0.096	&	0.095	&	0.009	&	0.013	\\
RF&		&		&		&		&		&	0.491	&	0.095	&	0.095	&	0.009	&	0.009	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&0.498	&	0.034	&	0.034	&	0.001	&	0.002	&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\
LASSO&0.498	&	0.034	&	0.034	&	0.001	&	0.002	&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\
CART&0.618	&	0.037	&	0.034	&	0.015	&	-0.118	&	0.498	&	0.030	&	0.031	&	0.001	&	0.002	\\
RF&		&		&		&		&		&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
LASSO&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.498	&	0.009	&	0.010	&	0.000	&	0.002	\\
CART&0.632	&	0.016	&	0.011	&	0.018	&	-0.132	&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\
RF&		&		&		&		&		&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\


\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are non-linear functions of $\xit$ and $\dit$. DGP1 is additive and linear in the nuisance functions; DGP2 is additive and nonlinear.  \red{CART is not tuned for DGP1.}}
\end{tablenotes}
\end{threeparttable}}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tp!]
\centering
 \caption{Simulation results with binary treatment, IV scores}
\scalebox{.8}{
\begin{threeparttable}
   \label{tab:}
   \begin{tabular}{lcccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{DGP1}&\multicolumn{5}{c}{DGP2}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}	
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  \\
\hline
\vspace{-2mm}\\
\multicolumn{11}{c}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&	0.499	&	0.091	&	0.092	&	0.008	&	0.001	&	0.504	&	0.085	&	0.083	&	0.007	&	-0.004	\\
LASSO&	0.510	&	0.089	&	0.086	&	0.008	&	-0.010	&	0.504	&	0.083	&	0.080	&	0.007	&	-0.004	\\
CART&	0.551	&	0.100	&	0.097	&	0.013	&	-0.051	&	0.507	&	0.083	&	0.080	&	0.007	&	-0.007	\\
RF&		&		&		&		&		&	0.507	&	0.082	&	0.080	&	0.007	&	-0.007	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&	0.498	&	0.028	&	0.028	&	0.001	&	0.002	&	0.498	&	0.025	&	0.025	&	0.001	&	0.002	\\
LASSO&	0.499	&	0.028	&	0.028	&	0.001	&	0.001	&	0.498	&	0.025	&	0.025	&	0.001	&	0.002	\\
CART&	0.630	&	0.032	&	0.029	&	0.018	&	-0.130	&	0.503	&	0.026	&	0.025	&	0.001	&	-0.003	\\
RF&		&		&		&		&		&	0.500	&	0.025	&	0.025	&	0.001	&	0.000	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&	0.499	&	0.008	&	0.009	&	0.000	&	0.001	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
LASSO&	0.499	&	0.008	&	0.009	&	0.000	&	0.001	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
CART&0.647	&	0.014	&	0.009	&	0.022	&	-0.147	&	0.504	&	0.008	&	0.008	&	0.000	&	-0.004	\\
RF&		&		&		&		&		&	0.500	&	0.008	&	0.008	&	0.000	&	0.000	\\



\vspace{-2mm}\\

\hline
\vspace{-2mm}\\
\multicolumn{11}{c}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&0.498	&	0.113	&	0.112	&	0.013	&	0.002	&	0.502	&	0.107	&	0.101	&	0.011	&	-0.002	\\
LASSO&0.507	&	0.109	&	0.105	&	0.012	&	-0.007	&	0.501	&	0.102	&	0.096	&	0.010	&	-0.001	\\
CART&	0.551	&	0.116	&	0.115	&	0.016	&	-0.051	&	0.498	&	0.098	&	0.097	&	0.010	&	0.002	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&0.497	&	0.034	&	0.034	&	0.001	&	0.003	&	0.495	&	0.030	&	0.031	&	0.001	&	0.005	\\
LASSO&0.498	&	0.034	&	0.033	&	0.001	&	0.002	&	0.495	&	0.030	&	0.030	&	0.001	&	0.005	\\
CART&	0.635	&	0.037	&	0.034	&	0.020	&	-0.135	&	0.496	&	0.031	&	0.031	&	0.001	&	0.004	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
LASSO&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
CART&	0.661	&	0.017	&	0.011	&	0.026	&	-0.161	&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\


\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are non-linear functions of $\xit$ and $\dit$. DGP1 is additive and linear in the nuisance functions; DGP2 is additive and nonlinear.  \red{CART is not tuned for DGP1.}}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_cnt_iv.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with continuous treatment, nonlinear functions and IV scores}
\scalebox{.7}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lccccccccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}&\multicolumn{5}{c}{Under FE (DGP3)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}\cmidrule(l{.35cm}r{.25cm}){12-16}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias \\
\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.034	&	0.035	&	0.001	&	-0.001	&	0.501	&	0.034	&	0.035	&	0.001	&	-0.001	&	0.501	&	0.032	&	0.032	&	0.001	&	-0.001	\\
LASSO&0.505	&	0.033	&	0.032	&	0.001	&	-0.005	&	0.505	&	0.033	&	0.032	&	0.001	&	-0.005	&	0.501	&	0.031	&	0.031	&	0.001	&	-0.001	\\
CART&0.512	&	0.034	&	0.034	&	0.001	&	-0.012	&	0.512	&	0.034	&	0.034	&	0.001	&	-0.012	&	0.504	&	0.033	&	0.033	&	0.001	&	-0.004	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.010	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.010	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.010	&	0.010	&	0.000	&	-0.001	\\
LASSO&0.501	&	0.010	&	0.010	&	0.000	&	-0.001	&	0.501	&	0.010	&	0.010	&	0.000	&	-0.001	&	0.501	&	0.009	&	0.010	&	0.000	&	-0.001	\\
CART&0.512	&	0.011	&	0.010	&	0.000	&	-0.012	&	0.512	&	0.011	&	0.010	&	0.000	&	-0.012	&	0.501	&	0.011	&	0.010	&	0.000	&	-0.001	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
LASSO&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
CART&0.516	&	0.005	&	0.003	&	0.000	&	-0.016	&	0.516	&	0.005	&	0.003	&	0.000	&	-0.016	&	0.500	&	0.004	&	0.003	&	0.000	&	0.000	\\
\vspace{-2mm}\\

\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.500	&	0.042	&	0.042	&	0.002	&	0.000	&	0.500	&	0.042	&	0.042	&	0.002	&	0.000	&	0.498	&	0.037	&	0.035	&	0.001	&	0.002	\\
LASSO&0.503	&	0.041	&	0.039	&	0.002	&	-0.003	&	0.503	&	0.041	&	0.039	&	0.002	&	-0.003	&	0.498	&	0.035	&	0.034	&	0.001	&	0.002	\\
CART&0.511	&	0.042	&	0.040	&	0.002	&	-0.011	&	0.510	&	0.042	&	0.040	&	0.002	&	-0.010	&	0.499	&	0.035	&	0.034	&	0.001	&	0.001	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.498	&	0.011	&	0.011	&	0.000	&	0.002	\\
LASSO&0.501	&	0.012	&	0.013	&	0.000	&	-0.001	&	0.501	&	0.012	&	0.013	&	0.000	&	-0.001	&	0.498	&	0.011	&	0.011	&	0.000	&	0.002	\\
CART&0.512	&	0.013	&	0.012	&	0.000	&	-0.012	&	0.512	&	0.013	&	0.012	&	0.000	&	-0.012	&	0.499	&	0.011	&	0.011	&	0.000	&	0.001	\\


\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.498	&	0.003	&	0.003	&	0.000	&	0.002	\\
LASSO&0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.498	&	0.003	&	0.003	&	0.000	&	0.002	\\
CART&0.516	&	0.005	&	0.004	&	0.000	&	-0.016	&	0.516	&	0.005	&	0.004	&	0.000	&	-0.016	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are non-linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_cnt_lin_iv.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with continuous treatment, linear functions and IV scores}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lcccccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias	&		$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias\\
\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.035	&	0.035	&	0.001	&	0.000	&	0.501	&	0.034	&	0.035	&	0.001	&	-0.001	\\
LASSO	&0.504	&	0.034	&	0.032	&	0.001	&	-0.004	&	0.505	&	0.033	&	0.032	&	0.001	&	-0.005	\\
CART&0.536	&	0.036	&	0.035	&	0.003	&	-0.036	&	0.537	&	0.036	&	0.035	&	0.003	&	-0.037	\\
RF1	&0.691	&	0.147	&	0.121	&	0.058	&	-0.191	&	0.692	&	0.142	&	0.121	&	0.057	&	-0.192	\\
RF5	&0.705	&	0.095	&	0.090	&	0.051	&	-0.205	&	0.699	&	0.094	&	0.090	&	0.049	&	-0.199	\\
RF10	&0.703	&	0.100	&	0.093	&	0.051	&	-0.203	&	0.697	&	0.099	&	0.093	&	0.048	&	-0.197	\\

\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.011	&	0.011	&	0.000	&	0.000	&	0.501	&	0.010	&	0.011	&	0.000	&	-0.001	\\
LASSO	&0.500	&	0.011	&	0.010	&	0.000	&	0.000	&	0.501	&	0.010	&	0.010	&	0.000	&	-0.001	\\
CART&0.576	&	0.013	&	0.011	&	0.006	&	-0.076	&	0.578	&	0.013	&	0.011	&	0.006	&	-0.078	\\
RF1	&0.676	&	0.072	&	0.032	&	0.036	&	-0.176	&	0.673	&	0.075	&	0.032	&	0.035	&	-0.173	\\
RF5	&0.677	&	0.038	&	0.028	&	0.033	&	-0.177	&	0.673	&	0.039	&	0.028	&	0.031	&	-0.173	\\
RF10	&0.676	&	0.033	&	0.028	&	0.032	&	-0.176	&	0.672	&	0.033	&	0.028	&	0.031	&	-0.172	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.003	&	0.003	&	0.000	&	0.000	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
LASSO	&0.500	&	0.003	&	0.003	&	0.000	&	0.000	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
CART&0.593	&	0.008	&	0.003	&	0.009	&	-0.093	&	0.593	&	0.008	&	0.003	&	0.009	&	-0.093	\\
RF1	&0.691	&	0.066	&	0.010	&	0.041	&	-0.191	&	0.688	&	0.068	&	0.010	&	0.040	&	-0.188	\\
RF5	&0.695	&	0.027	&	0.009	&	0.039	&	-0.195	&	0.691	&	0.027	&	0.009	&	0.037	&	-0.191	\\
RF10	&0.696	&	0.020	&	0.009	&	0.039	&	-0.196	&	0.692	&	0.020	&	0.009	&	0.037	&	-0.192	\\

\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.502	&	0.042	&	0.042	&	0.002	&	-0.002	&	0.641	&	0.056	&	0.057	&	0.023	&	-0.141	\\
LASSO	&0.505	&	0.040	&	0.039	&	0.002	&	-0.005	&	0.646	&	0.056	&	0.054	&	0.024	&	-0.146	\\
CART&0.534	&	0.042	&	0.042	&	0.003	&	-0.034	&	0.657	&	0.058	&	0.057	&	0.028	&	-0.157	\\
RF1	&0.691	&	0.066	&	0.010	&	0.041	&	-0.191	&	0.688 &0.068	&	0.010	&	0.040	&	-0.188	\\
RF5	&0.695	&	0.027	&	0.009	&	0.039	&	-0.195	&	0.691	&	0.027	&	0.009	&	0.037	&	-0.191	\\
RF10	&0.696	&	0.020	&	0.009	&	0.039	&	-0.196	&	0.692	&	0.020	&	0.009	&	0.037	&	-0.192	\\
\vspace{-3mm}\\

\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.639	&	0.017	&	0.018	&	0.020	&	-0.139	\\
LASSO	&0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.639	&	0.017	&	0.018	&	0.020	&	-0.139	\\
CART&	0.577	&	0.015	&	0.013	&	0.006	&	-0.077	&	0.687	&	0.018	&	0.017	&	0.035	&	-0.187	\\
RF1	&0.596	&	0.034	&	0.013	&	0.010	&	-0.096	&	0.685	&	0.026	&	0.017	&	0.035	&	-0.185	\\
RF5	&0.609	&	0.018	&	0.011	&	0.012	&	-0.109	&	0.691	&	0.018	&	0.016	&	0.037	&	-0.191	\\
RF10	&0.612	&	0.015	&	0.011	&	0.013	&	-0.112	&	0.691	&	0.017	&	0.016	&	0.037	&	-0.191	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.639	&	0.005	&	0.006	&	0.019	&	-0.139	\\
LASSO	&0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.639	&	0.005	&	0.006	&	0.019	&	-0.139	\\
CART&0.593	&	0.008	&	0.004	&	0.009	&	-0.093	&	0.703	&	0.006	&	0.005	&	0.041	&	-0.203	\\
RF1	&0.611	&	0.031	&	0.004	&	0.013	&	-0.111	&	0.695	&	0.019	&	0.005	&	0.038	&	-0.195	\\
RF5	&0.622	&	0.014	&	0.004	&	0.015	&	-0.122	&	0.698	&	0.009	&	0.005	&	0.039	&	-0.198	\\
RF10	&0.623	&	0.010	&	0.004	&	0.015	&	-0.123	&	0.698	&	0.007	&	0.005	&	0.039	&	-0.198	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_cnt_lin_po.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with continuous treatment, linear functions and PO scores}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lcccccccccc}   
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias	&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias\\
\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.502	&	0.036	&	0.033	&	0.001	&	-0.002	&	0.499	&	0.034	&	0.033	&	0.001	&	0.001	\\
LASSO	&0.504	&	0.034	&	0.033	&	0.001	&	-0.004	&	0.501	&	0.034	&	0.033	&	0.001	&	-0.001	\\
CART&	0.511	&	0.038	&	0.034	&	0.002	&	-0.011	&	0.508	&	0.037	&	0.034	&	0.001	&	-0.008	\\
RF1	&0.421	&	0.053	&	0.039	&	0.009	&	0.079	&	0.420	&	0.055	&	0.039	&	0.009	&	0.080	\\
RF5	&0.569	&	0.039	&	0.035	&	0.006	&	-0.069	&	0.567	&	0.039	&	0.035	&	0.006	&	-0.067	\\
RF10	&0.596	&	0.036	&	0.034	&	0.011	&	-0.096	&	0.593	&	0.035	&	0.035	&	0.010	&	-0.093	\\


\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.011	&	0.011	&	0.000	&	0.000	&	0.501	&	0.011	&	0.011	&	0.000	&	-0.001	\\
LASSO	&0.500	&	0.011	&	0.011	&	0.000	&	0.000	&	0.502	&	0.011	&	0.011	&	0.000	&	-0.002	\\
CART&0.554	&	0.014	&	0.011	&	0.003	&	-0.054	&	0.555	&	0.014	&	0.011	&	0.003	&	-0.055	\\
RF1	&0.506	&	0.043	&	0.012	&	0.002	&	-0.006	&	0.509	&	0.044	&	0.012	&	0.002	&	-0.009	\\
RF5	&0.591	&	0.020	&	0.011	&	0.009	&	-0.091	&	0.593	&	0.021	&	0.011	&	0.009	&	-0.093	\\
RF10	&0.605	&	0.017	&	0.011	&	0.011	&	-0.105	&	0.605	&	0.017	&	0.011	&	0.011	&	-0.105	\\


\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.003	&	0.003	&	0.000	&	0.000	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
LASSO	&0.500	&	0.003	&	0.003	&	0.000	&	0.000	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
CART&0.561	&	0.008	&	0.003	&	0.004	&	-0.061	&	0.561	&	0.009	&	0.003	&	0.004	&	-0.061	\\
RF1	&0.544	&	0.047	&	0.004	&	0.004	&	-0.044	&	0.541	&	0.046	&	0.004	&	0.004	&	-0.041	\\
RF5	&0.608	&	0.018	&	0.003	&	0.012	&	-0.108	&	0.608	&	0.018	&	0.004	&	0.012	&	-0.108	\\
RF10	&0.618	&	0.014	&	0.003	&	0.014	&	-0.118	&	0.618	&	0.013	&	0.003	&	0.014	&	-0.118	\\


\hline
\vspace{-2mm}\\
\multicolumn{11}{l}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{11}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.502	&	0.044	&	0.040	&	0.002	&	-0.002	&	0.640	&	0.057	&	0.054	&	0.023	&	-0.140	\\
LASSO&	0.502	&	0.042	&	0.040	&	0.002	&	-0.002	&	0.641	&	0.056	&	0.056	&	0.023	&	-0.141	\\
CART&0.504	&	0.043	&	0.040	&	0.002	&	-0.004	&	0.600	&	0.057	&	0.053	&	0.013	&	-0.100	\\
RF1	&0.418	&	0.056	&	0.044	&	0.010	&	0.082	&	0.500	&	0.056	&	0.051	&	0.003	&	0.000	\\
RF5	&0.569	&	0.045	&	0.041	&	0.007	&	-0.069	&	0.649	&	0.052	&	0.052	&	0.025	&	-0.149	\\
RF10	&0.596	&	0.042	&	0.041	&	0.011	&	-0.096	&	0.675	&	0.052	&	0.053	&	0.033	&	-0.175	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.640	&	0.018	&	0.018	&	0.020	&	-0.140	\\
LASSO	&0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.640	&	0.018	&	0.018	&	0.020	&	-0.140	\\
CART&0.554	&	0.016	&	0.013	&	0.003	&	-0.054	&	0.668	&	0.020	&	0.017	&	0.028	&	-0.168	\\
RF1	&0.508	&	0.044	&	0.014	&	0.002	&	-0.008	&	0.612	&	0.030	&	0.017	&	0.013	&	-0.112	\\
RF5	&0.592	&	0.022	&	0.013	&	0.009	&	-0.092	&	0.676	&	0.019	&	0.017	&	0.031	&	-0.176	\\
RF10	&0.604	&	0.017	&	0.013	&	0.011	&	-0.104	&	0.686	&	0.017	&	0.017	&	0.035	&	-0.186	\\

\vspace{-3mm}\\
\multicolumn{11}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-11}
OLS	&0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.639	&	0.005	&	0.006	&	0.019	&	-0.139	\\
LASSO &0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.639	&	0.005	&	0.006	&	0.019	&	-0.139	\\
CART&	0.557	&	0.007	&	0.004	&	0.003	&	-0.057	&	0.680	&	0.009	&	0.005	&	0.033	&	-0.180	\\
RF1	&0.538	&	0.044	&	0.004	&	0.003	&	-0.038	&	0.643	&	0.027	&	0.005	&	0.021	&	-0.143	\\
RF5	&0.607	&	0.018	&	0.004	&	0.012	&	-0.107	&	0.688	&	0.012	&	0.005	&	0.035	&	-0.188	\\
RF10	&0.616	&	0.013	&	0.004	&	0.014	&	-0.116	&	0.694	&	0.009	&	0.005	&	0.038	&	-0.194	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_cnt_po.tex <==
\begin{table}[tp!]
\centering
 \caption{Simulation results with continuous treatment, nonlinear functions and PO scores}
\scalebox{.7}{
\begin{threeparttable}	%use it for notes
   \label{tab:}
   \begin{tabular}{lccccccccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{5}{c}{Under RE (DGP1)}&\multicolumn{5}{c}{Under FE (DGP2)}&\multicolumn{5}{c}{Under FE (DGP3)}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-6}\cmidrule(l{.35cm}r{.25cm}){7-11}\cmidrule(l{.35cm}r{.25cm}){12-16}		
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias  %
&	$\widehat{\theta}$	&	SD	&	SE	&	RMSE	&	Bias \\
\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel A: Within-Group (WG) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.499	&	0.034	&	0.033	&	0.001	&	0.001	&	0.499	&	0.034	&	0.033	&	0.001	&	0.001	&	0.500	&	0.032	&	0.031	&	0.001	&	0.000	\\
LASSO&0.501	&	0.034	&	0.033	&	0.001	&	-0.001	&	0.501	&	0.034	&	0.033	&	0.001	&	-0.001	&	0.499	&	0.031	&	0.031	&	0.001	&	0.001	\\
CART&0.490	&	0.034	&	0.034	&	0.001	&	0.010	&	0.490	&	0.034	&	0.034	&	0.001	&	0.010	&	0.486	&	0.033	&	0.032	&	0.001	&	0.014	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.502	&	0.010	&	0.010	&	0.000	&	-0.002	\\
LASSO&0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.502	&	0.010	&	0.010	&	0.000	&	-0.002	\\
CART&0.503	&	0.012	&	0.011	&	0.000	&	-0.003	&	0.503	&	0.012	&	0.011	&	0.000	&	-0.003	&	0.490	&	0.010	&	0.010	&	0.000	&	0.010	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
LASSO&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
CART&0.513	&	0.006	&	0.003	&	0.000	&	-0.013	&	0.513	&	0.006	&	0.003	&	0.000	&	-0.013	&	0.489	&	0.003	&	0.003	&	0.000	&	0.011	\\
\vspace{-2mm}\\

\hline
\vspace{-2mm}\\
\multicolumn{16}{c}{\emph{Panel B: First-differences (FD) transformation}}\\
\vspace{-3mm}\\
\multicolumn{16}{c}{$N=100$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.498	&	0.042	&	0.040	&	0.002	&	0.002	&	0.498	&	0.042	&	0.040	&	0.002	&	0.002	&	0.498	&	0.035	&	0.033	&	0.001	&	0.002	\\
LASSO&0.499	&	0.040	&	0.040	&	0.002	&	0.001	&	0.499	&	0.040	&	0.040	&	0.002	&	0.001	&	0.496	&	0.034	&	0.034	&	0.001	&	0.004	\\
CART&0.484	&	0.041	&	0.039	&	0.002	&	0.016	&	0.484	&	0.041	&	0.039	&	0.002	&	0.016	&	0.489	&	0.034	&	0.034	&	0.001	&	0.011	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=1,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.013	&	0.013	&	0.000	&	-0.001	&	0.501	&	0.013	&	0.013	&	0.000	&	-0.001	&	0.499	&	0.011	&	0.011	&	0.000	&	0.001	\\
LASSO&0.501	&	0.013	&	0.013	&	0.000	&	-0.001	&	0.501	&	0.013	&	0.013	&	0.000	&	-0.001	&	0.499	&	0.011	&	0.011	&	0.000	&	0.001	\\
CART&0.502	&	0.014	&	0.013	&	0.000	&	-0.002	&	0.502	&	0.014	&	0.013	&	0.000	&	-0.002	&	0.499	&	0.010	&	0.011	&	0.000	&	0.001	\\

\vspace{-3mm}\\
\multicolumn{16}{c}{$N=10,000$}\\
\cmidrule(l{.35cm}r{.25cm}){2-16}
OLS	&0.501	&	0.004	&	0.004	&	0.000	&	-0.001	&	0.501	&	0.004	&	0.004	&	0.000	&	-0.001	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\
LASSO&0.501	&	0.004	&	0.004	&	0.000	&	-0.001	&	0.501	&	0.004	&	0.004	&	0.000	&	-0.001	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\
CART&0.515	&	0.006	&	0.004	&	0.000	&	-0.015	&	0.514	&	0.006	&	0.004	&	0.000	&	-0.014	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50. $\widehat{l}(.)$ and $\widehat{m}(.)$ are non-linear functions of $\xit$ and $\dit$.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

==> tabs/tab_cnt_po_under_FE.tex <==
%%CNT, Fe,PO
OLS&0.499	&	0.034	&	0.033	&	0.001	&	0.001	&	0.499	&	0.034	&	0.033	&	0.001	&	0.001	&	0.500	&	0.032	&	0.031	&	0.001	&	0.000	\\
LASSO&0.501	&	0.034	&	0.033	&	0.001	&	-0.001	&	0.501	&	0.034	&	0.033	&	0.001	&	-0.001	&	0.499	&	0.031	&	0.031	&	0.001	&	0.001	\\
CART&0.508	&	0.037	&	0.034	&	0.001	&	-0.008	&	0.490	&	0.034	&	0.034	&	0.001	&	0.010	&	0.486	&	0.033	&	0.032	&	0.001	&	0.014	\\

OLS&0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.502	&	0.010	&	0.010	&	0.000	&	-0.002	\\
LASSO&0.502	&	0.011	&	0.011	&	0.000	&	-0.002	&	0.501	&	0.011	&	0.011	&	0.000	&	-0.001	&	0.502	&	0.010	&	0.010	&	0.000	&	-0.002	\\
CART&0.555	&	0.014	&	0.011	&	0.003	&	-0.055	&	0.503	&	0.012	&	0.011	&	0.000	&	-0.003	&	0.490	&	0.010	&	0.010	&	0.000	&	0.010	\\

OLS&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
LASSO&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
CART&0.561	&	0.009	&	0.003	&	0.004	&	-0.061	&	0.513	&	0.006	&	0.003	&	0.000	&	-0.013	&	0.489	&	0.003	&	0.003	&	0.000	&	0.011	\\

%%CNT, FD,PO
%90
OLS&0.640	&	0.057	&	0.054	&	0.023	&	-0.140	&	0.498	&	0.042	&	0.040	&	0.002	&	0.002	&	0.498	&	0.035	&	0.033	&	0.001	&	0.002	\\
LASSO&0.641	&	0.056	&	0.056	&	0.023	&	-0.141	&	0.499	&	0.040	&	0.040	&	0.002	&	0.001	&	0.496	&	0.034	&	0.034	&	0.001	&	0.004	\\
CART&0.600	&	0.057	&	0.053	&	0.013	&	-0.100	&	0.484	&	0.041	&	0.039	&	0.002	&	0.016	&	0.489	&	0.034	&	0.034	&	0.001	&	0.011	\\
%900
OLS&0.640	&	0.018	&	0.018	&	0.020	&	-0.140	&	0.501	&	0.013	&	0.013	&	0.000	&	-0.001	&	0.499	&	0.011	&	0.011	&	0.000	&	0.001	\\
LASSO&0.640	&	0.018	&	0.018	&	0.020	&	-0.140	&	0.501	&	0.013	&	0.013	&	0.000	&	-0.001	&	0.499	&	0.011	&	0.011	&	0.000	&	0.001	\\
CART&0.668	&	0.020	&	0.017	&	0.028	&	-0.168	&	0.502	&	0.014	&	0.013	&	0.000	&	-0.002	&	0.499	&	0.010	&	0.011	&	0.000	&	0.001	\\
%9000
OLS&0.639	&	0.005	&	0.006	&	0.019	&	-0.139	&	0.501	&	0.004	&	0.004	&	0.000	&	-0.001	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\
LASSO&0.639	&	0.005	&	0.006	&	0.019	&	-0.139	&	0.501	&	0.004	&	0.004	&	0.000	&	-0.001	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\
CART&0.680	&	0.009	&	0.005	&	0.033	&	-0.180	&	0.514	&	0.006	&	0.004	&	0.000	&	-0.014	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\

%%BIN, Fe,PO
OLS&0.500	&	0.093	&	0.088	&	0.009	&	0.000	&	0.505	&	0.091	&	0.087	&	0.008	&	-0.005	&	0.498	&	0.083	&	0.079	&	0.007	&	0.002	\\
LASSO&0.508	&	0.090	&	0.088	&	0.008	&	-0.008	&	0.512	&	0.088	&	0.088	&	0.008	&	-0.012	&	0.497	&	0.080	&	0.080	&	0.006	&	0.003	\\
CART&0.508	&	0.092	&	0.088	&	0.009	&	-0.008	&	0.507	&	0.092	&	0.088	&	0.008	&	-0.007	&	0.494	&	0.080	&	0.080	&	0.006	&	0.006	\\

OLS&0.500	&	0.028	&	0.028	&	0.001	&	0.000	&	0.507	&	0.028	&	0.028	&	0.001	&	-0.007	&	0.499	&	0.025	&	0.025	&	0.001	&	0.001	\\
LASSO&0.500	&	0.028	&	0.028	&	0.001	&	0.000	&	0.508	&	0.028	&	0.028	&	0.001	&	-0.008	&	0.500	&	0.025	&	0.025	&	0.001	&	0.000	\\
CART&0.616	&	0.032	&	0.029	&	0.014	&	-0.116	&	0.518	&	0.028	&	0.028	&	0.001	&	-0.018	&	0.498	&	0.024	&	0.025	&	0.001	&	0.002	\\

OLS&0.500	&	0.008	&	0.009	&	0.000	&	0.000	&	0.506	&	0.009	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
LASSO&0.500	&	0.008	&	0.009	&	0.000	&	0.000	&	0.506	&	0.009	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
CART&0.627	&	0.015	&	0.009	&	0.016	&	-0.127	&	0.528	&	0.010	&	0.009	&	0.001	&	-0.028	&	0.497	&	0.008	&	0.008	&	0.000	&	0.003	\\

%%BIN, FD,PO
OLS&0.500	&	0.114	&	0.106	&	0.013	&	0.000	&	0.502	&	0.108	&	0.105	&	0.012	&	-0.002	&	0.497	&	0.105	&	0.095	&	0.011	&	0.003	\\
LASSO&0.505	&	0.110	&	0.106	&	0.012	&	-0.005	&	0.506	&	0.103	&	0.105	&	0.011	&	-0.006	&	0.496	&	0.099	&	0.095	&	0.010	&	0.004	\\
CART&0.492	&	0.106	&	0.102	&	0.011	&	0.008	&	0.501	&	0.103	&	0.104	&	0.011	&	-0.001	&	0.487	&	0.096	&	0.095	&	0.009	&	0.013	\\

OLS&0.498	&	0.034	&	0.034	&	0.001	&	0.002	&	0.505	&	0.034	&	0.034	&	0.001	&	-0.005	&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\
LASSO&0.498	&	0.034	&	0.034	&	0.001	&	0.002	&	0.505	&	0.034	&	0.034	&	0.001	&	-0.005	&	0.497	&	0.030	&	0.030	&	0.001	&	0.003	\\
CART&0.618	&	0.037	&	0.034	&	0.015	&	-0.118	&	0.518	&	0.034	&	0.033	&	0.001	&	-0.018	&	0.498	&	0.030	&	0.031	&	0.001	&	0.002	\\

OLS&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.504	&	0.010	&	0.011	&	0.000	&	-0.004	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
LASSO&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.504	&	0.010	&	0.011	&	0.000	&	-0.004	&	0.498	&	0.009	&	0.010	&	0.000	&	0.002	\\
CART&0.632	&	0.016	&	0.011	&	0.018	&	-0.132	&	0.529	&	0.011	&	0.011	&	0.001	&	-0.029	&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\


%%BIN, Fe,iv
OLS&0.499	&	0.091	&	0.092	&	0.008	&	0.001	&	0.508	&	0.093	&	0.091	&	0.009	&	-0.008	&	0.504	&	0.085	&	0.083	&	0.007	&	-0.004	\\
LASSO&0.510	&	0.089	&	0.086	&	0.008	&	-0.010	&	0.517	&	0.091	&	0.086	&	0.009	&	-0.017	&	0.504	&	0.083	&	0.080	&	0.007	&	-0.004	\\
CART&0.551	&	0.100	&	0.097	&	0.013	&	-0.051	&	0.523	&	0.093	&	0.090	&	0.009	&	-0.023	&	0.507	&	0.083	&	0.080	&	0.007	&	-0.007	\\

OLS&0.498	&	0.028	&	0.028	&	0.001	&	0.002	&	0.507	&	0.028	&	0.028	&	0.001	&	-0.007	&	0.498	&	0.025	&	0.025	&	0.001	&	0.002	\\
LASSO&0.499	&	0.028	&	0.028	&	0.001	&	0.001	&	0.508	&	0.028	&	0.028	&	0.001	&	-0.008	&	0.498	&	0.025	&	0.025	&	0.001	&	0.002	\\
CART&0.630	&	0.032	&	0.029	&	0.018	&	-0.130	&	0.525	&	0.029	&	0.028	&	0.001	&	-0.025	&	0.503	&	0.026	&	0.025	&	0.001	&	-0.003	\\

OLS&0.499	&	0.008	&	0.009	&	0.000	&	0.001	&	0.506	&	0.008	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
LASSO&0.499	&	0.008	&	0.009	&	0.000	&	0.001	&	0.506	&	0.008	&	0.009	&	0.000	&	-0.006	&	0.499	&	0.008	&	0.008	&	0.000	&	0.001	\\
CART&0.647	&	0.014	&	0.009	&	0.022	&	-0.147	&	0.530	&	0.010	&	0.009	&	0.001	&	-0.030	&	0.504	&	0.008	&	0.008	&	0.000	&	-0.004	\\

%%BIN, FD,iv
OLS&0.498	&	0.113	&	0.112	&	0.013	&	0.002	&	0.503	&	0.110	&	0.112	&	0.012	&	-0.003	&	0.502	&	0.107	&	0.101	&	0.011	&	-0.002	\\
LASSO&0.507	&	0.109	&	0.105	&	0.012	&	-0.007	&	0.510	&	0.107	&	0.104	&	0.012	&	-0.010	&	0.501	&	0.102	&	0.096	&	0.010	&	-0.001	\\
CART&0.551	&	0.116	&	0.115	&	0.016	&	-0.051	&	0.526	&	0.114	&	0.107	&	0.014	&	-0.026	&	0.498	&	0.098	&	0.097	&	0.010	&	0.002	\\

OLS&0.497	&	0.034	&	0.034	&	0.001	&	0.003	&	0.504	&	0.034	&	0.034	&	0.001	&	-0.004	&	0.495	&	0.030	&	0.031	&	0.001	&	0.005	\\
LASSO&0.498	&	0.034	&	0.033	&	0.001	&	0.002	&	0.505	&	0.034	&	0.033	&	0.001	&	-0.005	&	0.495	&	0.030	&	0.030	&	0.001	&	0.005	\\
CART&0.635	&	0.037	&	0.034	&	0.020	&	-0.135	&	0.528	&	0.036	&	0.034	&	0.002	&	-0.028	&	0.496	&	0.031	&	0.031	&	0.001	&	0.004	\\

OLS&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.503	&	0.010	&	0.011	&	0.000	&	-0.003	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
LASSO&0.498	&	0.010	&	0.011	&	0.000	&	0.002	&	0.503	&	0.010	&	0.011	&	0.000	&	-0.003	&	0.497	&	0.009	&	0.010	&	0.000	&	0.003	\\
CART&0.661	&	0.017	&	0.011	&	0.026	&	-0.161	&	0.533	&	0.011	&	0.011	&	0.001	&	-0.033	&	0.498	&	0.010	&	0.010	&	0.000	&	0.002	\\


%%CNT, Fe,iv
OLS&0.501	&	0.034	&	0.035	&	0.001	&	-0.001	&	0.501	&	0.034	&	0.035	&	0.001	&	-0.001	&	0.501	&	0.032	&	0.032	&	0.001	&	-0.001	\\
LASSO&0.505	&	0.033	&	0.032	&	0.001	&	-0.005	&	0.505	&	0.033	&	0.032	&	0.001	&	-0.005	&	0.501	&	0.031	&	0.031	&	0.001	&	-0.001	\\
CART&0.537	&	0.036	&	0.035	&	0.003	&	-0.037	&	0.512	&	0.034	&	0.034	&	0.001	&	-0.012	&	0.504	&	0.033	&	0.033	&	0.001	&	-0.004	\\

OLS&0.501	&	0.010	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.010	&	0.011	&	0.000	&	-0.001	&	0.501	&	0.010	&	0.010	&	0.000	&	-0.001	\\
LASSO&0.501	&	0.010	&	0.010	&	0.000	&	-0.001	&	0.501	&	0.010	&	0.010	&	0.000	&	-0.001	&	0.501	&	0.009	&	0.010	&	0.000	&	-0.001	\\
CART&0.578	&	0.013	&	0.011	&	0.006	&	-0.078	&	0.512	&	0.011	&	0.010	&	0.000	&	-0.012	&	0.501	&	0.011	&	0.010	&	0.000	&	-0.001	\\

OLS&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
LASSO&0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	&	0.501	&	0.003	&	0.003	&	0.000	&	-0.001	\\
CART&0.593	&	0.008	&	0.003	&	0.009	&	-0.093	&	0.516	&	0.005	&	0.003	&	0.000	&	-0.016	&	0.500	&	0.004	&	0.003	&	0.000	&	0.000	\\

%%CNT, FD,iv
OLS&0.641	&	0.056	&	0.057	&	0.023	&	-0.141	&	0.500	&	0.042	&	0.042	&	0.002	&	0.000	&	0.498	&	0.037	&	0.035	&	0.001	&	0.002	\\
LASSO&0.646	&	0.056	&	0.054	&	0.024	&	-0.146	&	0.503	&	0.041	&	0.039	&	0.002	&	-0.003	&	0.498	&	0.035	&	0.034	&	0.001	&	0.002	\\
CART&0.657	&	0.058	&	0.057	&	0.028	&	-0.157	&	0.510	&	0.042	&	0.040	&	0.002	&	-0.010	&	0.499	&	0.035	&	0.034	&	0.001	&	0.001	\\

OLS&0.639	&	0.017	&	0.018	&	0.020	&	-0.139	&	0.500	&	0.013	&	0.013	&	0.000	&	0.000	&	0.498	&	0.011	&	0.011	&	0.000	&	0.002	\\
LASSO&0.639	&	0.017	&	0.018	&	0.020	&	-0.139	&	0.501	&	0.012	&	0.013	&	0.000	&	-0.001	&	0.498	&	0.011	&	0.011	&	0.000	&	0.002	\\
CART&0.687	&	0.018	&	0.017	&	0.035	&	-0.187	&	0.512	&	0.013	&	0.012	&	0.000	&	-0.012	&	0.499	&	0.011	&	0.011	&	0.000	&	0.001	\\

OLS&0.639	&	0.005	&	0.006	&	0.019	&	-0.139	&	0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.498	&	0.003	&	0.003	&	0.000	&	0.002	\\
LASSO&0.639	&	0.005	&	0.006	&	0.019	&	-0.139	&	0.500	&	0.004	&	0.004	&	0.000	&	0.000	&	0.498	&	0.003	&	0.003	&	0.000	&	0.002	\\
CART&0.703	&	0.006	&	0.005	&	0.041	&	-0.203	&	0.516	&	0.005	&	0.004	&	0.000	&	-0.016	&	0.499	&	0.003	&	0.003	&	0.000	&	0.001	\\



==> tabs/tab_hp_tuned.tex <==
\begin{table}[th]
\centering
 \caption{Hyperparameter tuning}\label{tab:hyperpara_fazio5}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lcccc}  
\hline\hline
\vspace{-2mm}\\
&\multicolumn{2}{c}{Table(3)}&\multicolumn{2}{c}{Table(4)} \\
 \cmidrule(l{.35cm}r{.25cm}){2-3} \cmidrule(l{.35cm}r{.25cm}){4-5}
&Approx & Hybrid& Approx& Hybrid\\
\hline
\vspace{-2mm}\\
\multicolumn{5}{c}{\emph{Base learner for nuisance functions: CART}}  \\
\texttt{cp*}&$\{0.043,0.027\}$&$\{0.41,0.41\}$&$\{0.044,0.027\}$&$\{0.41,0.41\}$\\
\texttt{minbucket*}&$\{2464,1688\}$&$\{5,551\}$&$\{2464,1688\}$&$\{5,551\}$\\
\texttt{maxdepth*}&$\{4,3\}$&$\{10,7\}$&$\{4,3\}$&$\{10,7\}$\\

\vspace{-2mm}\\

\multicolumn{5}{c}{\emph{Base learner for nuisance functions: RF}}  \\
\texttt{num.trees}& 1000 &1000&1000&1000\\
\texttt{min.node.size*}&$\{1558,1170\}$&$\{134,134\}$&$\{134,1429\}$&$\{134,134\}$\\
\texttt{max.depth*}&$\{79,6\}$&$\{22,37\}$&$\{37,85\}$&$\{22,37\}$\\
% \texttt{mtry}& $\{p+1,p\}$&$\{p+1,p\}$&$\{p+1,p\}$&$\{p+1,p\}$\\
% \texttt{importance}& impurity&impurity&impurity&impurity \\

% \vspace{-2mm}\\
% \multicolumn{5}{c}{\emph{Base learner for nuisance functions: Gradient boosting}}  \\
% \texttt{lambda*}&$\{\red{0.043,0.027}\}$&$\{1.79,1.79\}$&$\{\red{0.044,0.027}\}$&$\{2,1.05\}$\\
% \texttt{max\_depth*}&$\{4,3\}$&$\{5,8\}$&$\{4,3\}$&$\{9,7\}$\\
% \texttt{nrounds}& 1000 &1000&1000&1000\\

\vspace{-2mm}\\
\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\footnotesize{Note: * indicates the hyperparameters that are tuned with grid search with options \texttt{(n\_evals = 10, resolution = 20)}. The optimal value for \texttt{cp} is chosen from the real values in the interval $\{0.01,0.05\}$; \texttt{minbucket} and \texttt{min.node.size} from integer values in $\{5,N/2\}$; \texttt{maxdepth} from integer values in $\{1,30\}$, \texttt{max.depth} from $\{1,100\}$, and  \texttt{max\_depth} from $\{5,10\}$; \texttt{lambda} from the real values in  $\{0,2\}$. The hyperparameters in brackets refer to the  (optimal) chosen value for $m$ and $l$, respectively.}
\end{tablenotes}
\end{threeparttable}}
\end{table}




==> tabs/tab_sum_dgp1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CONTINUOUS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[th!]
\centering
 \caption{Simulation results with continuous treatment, DGP1}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=10,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: WG estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.002	&	0.033	&	1.004	&	0.002	&	0.011	&	0.983	&	0.001	&	0.003	&	1.064	\\
OLS	&	0.002	&	0.034	&	1.005	&	0.002	&	0.011	&	0.985	&	0.001	&	0.003	&	1.065	\\
DML-Lasso	&	0.001	&	0.034	&	0.986	&	0.002	&	0.011	&	0.991	&	0.001	&	0.003	&	1.067	\\
DML-CART	&	0.029	&	0.048	&	0.893	&	0.061	&	0.064	&	0.573	&	0.070	&	0.074	&	0.144	\\
DML-RF	&	0.017	&	0.039	&	0.965	&	0.005	&	0.012	&	0.977	&	0.003	&	0.007	&	0.558	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: FD estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.001	&	0.040	&	0.996	&	0.001	&	0.013	&	1.004	&	0.001	&	0.004	&	1.073	\\
OLS	&	0.001	&	0.041	&	0.994	&	0.001	&	0.013	&	1.005	&	0.001	&	0.004	&	1.074	\\
DML-Lasso	&	-0.001	&	0.040	&	1.000	&	0.001	&	0.013	&	1.000	&	0.001	&	0.004	&	1.083	\\
DML-CART	&	0.024	&	0.051	&	0.898	&	0.062	&	0.066	&	0.596	&	0.073	&	0.077	&	0.160	\\
DML-RF	&	0.014	&	0.043	&	0.969	&	0.005	&	0.014	&	0.955	&	0.003	&	0.007	&	0.659	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: CRE   estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.002	&	0.033	&	1.004	&	0.002	&	0.011	&	0.983	&	0.001	&	0.003	&	1.064	\\
OLS	&	0.002	&	0.034	&	1.005	&	0.002	&	0.011	&	0.985	&	0.001	&	0.003	&	1.065	\\
DML-Lasso	&	0.041	&	0.054	&	1.029	&	0.014	&	0.017	&	0.992	&	0.005	&	0.006	&	1.064	\\
DML-CART	&	0.011	&	0.055	&	1.040	&	0.017	&	0.032	&	0.614	&	0.028	&	0.040	&	0.182	\\
DML-RF	&	0.085	&	0.098	&	1.096	&	0.017	&	0.023	&	0.936	&	0.000	&	0.014	&	0.319	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%% BINARY
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[tp!]
% \centering
%  \caption{Simulation results with binary treatment, DGP1}
% \scalebox{.8}{
% \begin{threeparttable}	%use it for notes
% \begin{tabular}{lccccccccc}  
% \vspace{-3mm}\\   
% \hline\hline
% \vspace{-3mm}\\
% &\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=10,000$}\\  	
% \cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
% \hline
% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel A: WG estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	0.001	&	0.090	&	0.986	&	0.000	&	0.028	&	1.018	&	-0.001	&	0.009	&	1.026	\\
% OLS	&	0.001	&	0.091	&	0.989	&	0.000	&	0.028	&	1.017	&	-0.001	&	0.009	&	1.026	\\
% DML-Lasso	&	0.008	&	0.090	&	0.981	&	0.000	&	0.028	&	1.009	&	0.000	&	0.008	&	1.072	\\
% DML-CART	&	0.071	&	0.116	&	0.991	&	0.128	&	0.133	&	0.816	&	0.150	&	0.152	&	0.321	\\
% DML-RF	&	0.042	&	0.097	&	1.019	&	0.008	&	0.029	&	1.003	&	0.004	&	0.010	&	0.941	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel B: FD estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	0.000	&	0.108	&	0.983	&	-0.001	&	0.034	&	0.999	&	-0.002	&	0.011	&	1.019	\\
% OLS	&	-0.002	&	0.110	&	0.979	&	-0.001	&	0.034	&	0.998	&	-0.002	&	0.011	&	1.018	\\
% DML-Lasso	&	0.005	&	0.110	&	0.964	&	-0.002	&	0.034	&	1.005	&	-0.002	&	0.010	&	1.079	\\
% DML-CART	&	0.061	&	0.126	&	0.970	&	0.136	&	0.141	&	0.862	&	0.161	&	0.164	&	0.322	\\
% DML-RF	&	0.034	&	0.114	&	0.973	&	0.010	&	0.035	&	0.991	&	0.003	&	0.012	&	0.940	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel C: CRE   estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	0.001	&	0.090	&	0.986	&	0.000	&	0.028	&	1.018	&	-0.001	&	0.009	&	1.026	\\
% OLS	&	0.000	&	0.091	&	0.989	&	0.000	&	0.028	&	1.017	&	-0.001	&	0.009	&	1.026	\\
% DML-Lasso	&	0.033	&	0.106	&	0.991	&	0.009	&	0.031	&	1.022	&	0.002	&	0.009	&	1.052	\\
% DML-CART	&	0.065	&	0.142	&	0.969	&	0.069	&	0.078	&	0.969	&	0.071	&	0.073	&	0.875	\\
% DML-RF	&	0.106	&	0.156	&	0.998	&	0.010	&	0.033	&	1.040	&	-0.008	&	0.014	&	0.816	\\

% \hline
% \end{tabular} 	
% \begin{tablenotes}[para,flushleft]	
% \emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.}
% \end{tablenotes}
% \end{threeparttable}}
% \end{table}

==> tabs/tab_sum_dgp2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CONTINUOUS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tp!]
\centering
 \caption{Simulation results with continuous treatment, DGP2}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=10,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: WG estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.002	&	0.031	&	0.990	&	0.002	&	0.010	&	0.983	&	0.001	&	0.003	&	1.094	\\
OLS	&	0.001	&	0.031	&	0.996	&	0.002	&	0.010	&	0.981	&	0.001	&	0.003	&	1.094	\\
DML-Lasso	&	-0.001	&	0.031	&	0.993	&	0.002	&	0.010	&	1.013	&	0.001	&	0.003	&	1.082	\\
DML-CART	&	-0.014	&	0.035	&	0.976	&	-0.010	&	0.014	&	0.969	&	-0.011	&	0.012	&	0.948	\\
DML-RF	&	-0.007	&	0.033	&	0.983	&	-0.002	&	0.010	&	1.032	&	0.000	&	0.003	&	1.013	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: FD estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.000	&	0.035	&	0.978	&	-0.001	&	0.011	&	0.996	&	-0.001	&	0.003	&	1.109	\\
OLS	&	-0.001	&	0.036	&	0.962	&	-0.001	&	0.011	&	1.002	&	-0.002	&	0.003	&	1.104	\\
DML-Lasso	&	-0.004	&	0.034	&	0.990	&	-0.001	&	0.011	&	1.006	&	-0.001	&	0.003	&	1.063	\\
DML-CART	&	-0.011	&	0.036	&	0.980	&	-0.001	&	0.010	&	1.029	&	-0.001	&	0.003	&	1.033	\\
DML-RF	&	-0.007	&	0.034	&	1.002	&	-0.002	&	0.010	&	1.035	&	-0.001	&	0.004	&	1.032	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: CRE   estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.002	&	0.028	&	0.990	&	0.002	&	0.009	&	0.999	&	0.002	&	0.003	&	1.075	\\
OLS	&	0.000	&	0.029	&	0.970	&	-0.001	&	0.009	&	1.002	&	0.000	&	0.003	&	1.065	\\
DML-Lasso	&	0.036	&	0.047	&	0.970	&	0.010	&	0.013	&	1.000	&	0.003	&	0.004	&	1.069	\\
DML-CART	&	-0.006	&	0.052	&	1.025	&	-0.025	&	0.028	&	1.070	&	-0.025	&	0.025	&	0.840	\\
DML-RF	&	0.018	&	0.040	&	1.081	&	0.010	&	0.018	&	0.845	&	-0.008	&	0.021	&	0.195	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%% BINARY
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[tp!]
% \centering
%  \caption{Simulation results with binary treatment, DGP2}
% \scalebox{.8}{
% \begin{threeparttable}	%use it for notes
% \begin{tabular}{lccccccccc}  
% \vspace{-3mm}\\   
% \hline\hline
% \vspace{-3mm}\\
% &\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=10,000$}\\  	
% \cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
% \hline
% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel A: WG estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	0.004	&	0.077	&	1.029	&	0.001	&	0.025	&	1.005	&	0.001	&	0.008	&	1.063	\\
% OLS	&	0.001	&	0.080	&	1.013	&	-0.001	&	0.025	&	1.003	&	-0.001	&	0.008	&	1.054	\\
% DML-Lasso	&	-0.003	&	0.080	&	0.999	&	0.000	&	0.025	&	1.023	&	-0.001	&	0.008	&	1.036	\\
% DML-CART	&	-0.006	&	0.080	&	1.003	&	-0.002	&	0.024	&	1.041	&	-0.003	&	0.009	&	0.968	\\
% DML-RF	&	-0.005	&	0.079	&	1.004	&	-0.004	&	0.024	&	1.049	&	-0.001	&	0.008	&	1.034	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel B: FD estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	0.000	&	0.096	&	1.009	&	-0.001	&	0.031	&	0.990	&	-0.002	&	0.009	&	1.074	\\
% OLS	&	-0.002	&	0.098	&	0.995	&	-0.002	&	0.030	&	1.006	&	-0.003	&	0.009	&	1.080	\\
% DML-Lasso	&	-0.004	&	0.099	&	0.960	&	-0.003	&	0.030	&	1.016	&	-0.002	&	0.010	&	1.041	\\
% DML-CART	&	-0.013	&	0.097	&	0.995	&	-0.002	&	0.030	&	1.008	&	-0.002	&	0.010	&	1.009	\\
% DML-RF	&	-0.009	&	0.095	&	1.004	&	-0.003	&	0.030	&	1.013	&	-0.002	&	0.010	&	1.010	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel C: CRE   estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	0.007	&	0.075	&	1.034	&	0.005	&	0.025	&	0.994	&	0.005	&	0.009	&	1.068	\\
% OLS	&	0.002	&	0.080	&	1.013	&	0.000	&	0.025	&	1.004	&	0.000	&	0.008	&	1.058	\\
% DML-Lasso	&	0.024	&	0.087	&	1.003	&	0.005	&	0.026	&	1.027	&	-0.001	&	0.008	&	1.038	\\
% DML-CART	&	-0.005	&	0.128	&	0.985	&	-0.008	&	0.039	&	0.927	&	-0.006	&	0.015	&	0.831	\\
% DML-RF	&	0.010	&	0.093	&	1.021	&	-0.002	&	0.031	&	0.949	&	-0.003	&	0.011	&	0.899	\\

% \hline
% \end{tabular} 	
% \begin{tablenotes}[para,flushleft]	
% \emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.}
% \end{tablenotes}
% \end{threeparttable}}
% \end{table}

==> tabs/tab_sum_dgp3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CONTINUOUS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[tp!]
\centering
 \caption{Simulation results with continuous treatment, DGP3}
\scalebox{.8}{
\begin{threeparttable}	%use it for notes
\begin{tabular}{lccccccccc}  
\vspace{-3mm}\\   
\hline\hline
\vspace{-3mm}\\
&\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=10,000$}\\  	
\cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
&	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
\hline
\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel A: WG estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.000	&	0.022	&	0.985	&	0.001	&	0.007	&	0.993	&	0.001	&	0.002	&	1.087	\\
OLS	&	0.993	&	0.993	&	0.994	&	0.993	&	0.993	&	0.983	&	0.993	&	0.993	&	1.023	\\
DML-Lasso	&	0.992	&	0.992	&	0.921	&	0.993	&	0.993	&	0.992	&	0.993	&	0.993	&	1.051	\\
DML-CART	&	0.700	&	0.711	&	0.383	&	0.700	&	0.706	&	0.138	&	0.712	&	0.717	&	0.045	\\
DML-RF	&	0.942	&	0.946	&	0.221	&	0.925	&	0.927	&	0.102	&	0.895	&	0.901	&	0.028	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel B: FD estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.000	&	0.026	&	0.989	&	0.001	&	0.008	&	1.012	&	0.001	&	0.003	&	1.066	\\
OLS	&	0.992	&	0.992	&	0.952	&	0.993	&	0.993	&	0.966	&	0.993	&	0.993	&	1.037	\\
DML-Lasso	&	0.992	&	0.992	&	0.864	&	0.993	&	0.993	&	0.990	&	0.993	&	0.993	&	1.037	\\
DML-CART	&	0.950	&	0.950	&	0.487	&	0.969	&	0.970	&	0.319	&	0.972	&	0.972	&	0.066	\\
DML-RF	&	0.975	&	0.976	&	0.622	&	0.987	&	0.987	&	0.524	&	0.991	&	0.991	&	0.343	\\

\vspace{-1mm}\\
\multicolumn{10}{c}{\emph{Panel C: CRE   estimator}}\\
\vspace{-3mm}\\
ORACLE	&	0.000	&	0.022	&	0.985	&	0.001	&	0.007	&	0.993	&	0.001	&	0.002	&	1.087	\\
OLS	&	0.993	&	0.993	&	0.994	&	0.993	&	0.993	&	0.983	&	0.993	&	0.993	&	1.023	\\
DML-Lasso	&	1.013	&	1.013	&	1.096	&	1.000	&	1.000	&	1.018	&	0.996	&	0.996	&	0.976	\\
DML-CART	&	0.205	&	0.291	&	0.365	&	0.032	&	0.121	&	0.215	&	0.082	&	0.155	&	0.061	\\
DML-RF	&	0.700	&	0.753	&	0.235	&	0.271	&	0.497	&	0.106	&	0.150	&	0.410	&	0.045	\\

\hline
\end{tabular} 	
\begin{tablenotes}[para,flushleft]	
\emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.}
\end{tablenotes}
\end{threeparttable}}
\end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%% BINARY
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[tp!]
% \centering
%  \caption{Simulation results with binary treatment, DGP3}
% \scalebox{.8}{
% \begin{threeparttable}	%use it for notes
% \begin{tabular}{lccccccccc}  
% \vspace{-3mm}\\   
% \hline\hline
% \vspace{-3mm}\\
% &\multicolumn{3}{c}{$N=100$}&\multicolumn{3}{c}{$N=1,000$}&\multicolumn{3}{c}{$N=10,000$}\\  	
% \cmidrule(l{.35cm}r{.25cm}){2-4}\cmidrule(l{.35cm}r{.25cm}){5-7}\cmidrule(l{.35cm}r{.25cm}){8-10}		
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	%
% &	$Bias(\widehat{\theta})$ &	RMSE	&	$se(\widehat{\theta})/sd(\widehat{\theta})$	\\
% \hline
% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel A: WG estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	-0.097	&	0.120	&	1.010	&	-0.092	&	0.095	&	1.003	&	-0.093	&	0.093	&	1.047	\\
% OLS	&	15.785	&	15.801	&	0.985	&	15.780	&	15.782	&	1.011	&	15.792	&	15.793	&	1.057	\\
% DML-Lasso	&	15.884	&	15.901	&	0.917	&	15.806	&	15.808	&	1.000	&	15.795	&	15.795	&	1.078	\\
% DML-CART	&	7.923	&	7.958	&	0.822	&	7.824	&	7.831	&	0.551	&	7.778	&	7.784	&	0.205	\\
% DML-RF	&	8.831	&	8.873	&	0.645	&	7.895	&	7.897	&	0.985	&	7.900	&	7.900	&	0.828	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel B: FD estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	-0.011	&	0.105	&	0.991	&	-0.002	&	0.034	&	0.984	&	-0.004	&	0.011	&	1.021	\\
% OLS	&	15.775	&	15.798	&	0.979	&	15.786	&	15.788	&	0.991	&	15.792	&	15.793	&	1.049	\\
% DML-Lasso	&	15.829	&	15.854	&	0.916	&	15.808	&	15.811	&	0.999	&	15.795	&	15.795	&	1.084	\\
% DML-CART	&	15.669	&	15.695	&	0.908	&	15.877	&	15.879	&	0.985	&	15.932	&	15.932	&	0.965	\\
% DML-RF	&	15.874	&	15.899	&	0.921	&	15.861	&	15.863	&	1.007	&	15.888	&	15.889	&	0.995	\\

% \vspace{-1mm}\\
% \multicolumn{10}{c}{\emph{Panel C: CRE   estimator}}\\
% \vspace{-3mm}\\
% ORACLE	&	-0.008	&	0.085	&	1.016	&	-0.001	&	0.027	&	1.011	&	-0.002	&	0.009	&	1.046	\\
% OLS	&	15.785	&	15.801	&	0.985	&	15.780	&	15.782	&	1.011	&	15.792	&	15.793	&	1.057	\\
% DML-Lasso	&	16.101	&	16.117	&	0.927	&	15.937	&	15.939	&	1.025	&	15.908	&	15.908	&	1.093	\\
% DML-CART	&	2.203	&	2.609	&	0.410	&	1.293	&	1.339	&	0.429	&	1.292	&	1.310	&	0.210	\\
% DML-RF	&	4.504	&	5.027	&	0.231	&	0.107	&	0.198	&	0.443	&	0.033	&	0.121	&	0.204	\\

% \hline
% \end{tabular} 	
% \begin{tablenotes}[para,flushleft]	
% \emph{The figures in the table are the average values over the total number of replications. The number of replications is 1,000. The true causal parameter $\theta$ is 0.50.}
% \end{tablenotes}
% \end{threeparttable}}
% \end{table}

==> tabs/tab_summary_fazio5.tex <==
\begin{table}[th!]
\centering
 \caption{Summary statistics}\label{tab:fazio5_summary}
\scalebox{.95}{
\begin{threeparttable}	%use it for notes
   \begin{tabular}{lcccc}   
\vspace{-5mm}\\   
\hline\hline
\vspace{-4mm}\\
            &        Mean&          SD&         Min&         Max\\
\hline
\vspace{-3mm}\\
Vote Conservative  &       0.102&       0.303&        0&        1\\
NMW         &       0.020&       0.138&        0&        1\\
HH income    &       8.082&       1.312&       -1.32&       11.46\\
HH size      &       3.145&       1.213&        1&       14\\
Age         &      35.914&      10.930&       18&       65\\
Age squared      &    1,409.3&     838.9&      324&     4,225\\
Degree      &       0.102&       0.303&        0&        1\\
Married     &       0.534&       0.499&        0&        1\\

\vspace{-2mm}\\
\hline
Observations     &       19,961&            &            &            \\
No. groups     &       4,927&            &            &            \\
\hline
\end{tabular} 	
% \begin{tablenotes}[para,flushleft]	
% \emph{Note: .}
% \end{tablenotes}
\end{threeparttable}}
\end{table}



==> thoughts.tex <==
%Following \blue{Semenova et al. (2021)}, we can use %Equations~\eqref{eqn:outcome} and~\eqref{eqn:treat} to write:
%\begin{equation}\label{eqn:rf}
% y_{it} = \underbrace{\theta_0 m_0(\x) +g_0(\x)+ f_i + e_i}_{= l_0(\x)}+ \theta_0  \nu_{it}  + \epsilon_{it} 
%\end{equation}
%The residuals from~\eqref{eqn:outcome} and~\eqref{eqn:treat} %are:
%%%%%%%%
%\begin{align}
%& \nu_{it} \equiv d_{it} - m_0(\x)  \label{eqn:res_treat}\\
%& \ty \equiv  y_{it}-l_0(\x) \label{eqn:res_outcome}
%\end{align}

%From the relationship between the outcome and treatment residuals (i.e., from Equation~\eqref{eqn:rf}), we get
%%%%%%%%%%%%%
%\begin{equation}\label{eqn:rf2}
%\ty = \theta_0  \nu_{it}  + \epsilon_{it} 
%\end{equation}
%\noindent where $ \theta_0 $ is estimated with a learner (e.g., Lasso, causal forest, etc.). We want to orthogonalise the learner to overcome regularisation biases \blue{(Chernozhukov et al., 2019)}.

\

\noindent \textbf{Algorithm.} We can construct a feasible but inefficient (although the estimating equation is {\em locally} efficient in the sense of being semi-parametrically efficient if $\epsilon_{it}$ is truly homoscedastic) estimating equation using a two-step process.  In the spirit of the \texttt{re-em} iterative process, and that used by \blue{Belloni}, we could set about estimation using the following algorithm \red{(for step~2)}:

\begin{enumerate}
    \item Learn $m_0(\xit)$ from the concatenated data on $\{ d_{it}, \xit \}$:\ call this ${\hat m}(\xit})$ 
    \item	Set $p=0$.
    \item	Choose starting value $\theta^{(p)}$ (could just be zero).
    \item	Increment $p = p + 1$
    \begin{enumerate}[label={\roman*}.]
        \item	Calculate $\ty^{(p)} = y_{it} - d_{it}\theta^{(p-1)}$ 
        \item	Ignoring the autocorrelation in concatenated data $\{\ty^{(p)}: t=1,...,T; i=1,...,n\}$, apply the learner to the data (after setting aside, say, 20\% of the individuals and all of their person-wave observations for validation) to learn $g^{(p)}(\x)$ %\red{[In DML algorithm $g(.)$ is learned using only $y$ and $X$ not $d$; $d$ and $X$ are used to learn $m(.)$. So we should learn $m(.)$ and $g(.)$ first. Then orthogonalise the estimating equation.]}
        \item	Calculate $r^{(p)}_{it} = y_{it} - d_{it}\theta^{(p-1)} - g^{(p)}(\x)$ and estimate variance-covariance matrix $\Sigma^{(p)}=n^{-1}\Sigma_{i=1}^n{\bf r}_i^{(p)}{\bf r}_i^{(p)T}$, where ${\bf r}_i^{(p)} = (r_{i1}^{(p)}},...,r_{iT}^{(p)})^T$ 
        \item	Estimate $\theta^{(p)}$ using the relevant estimating equation with $g^{(p)}(.)$ and $\Sigma^{(p)}$ plugged in (the Neyman orthogonal estimating equation will also require ${\hat m}()$) 
    \end{enumerate}
    \item	Return to Step~(4) and repeat until convergence in successive $|\theta^{(p)} -\theta^{(p-1)}|$ to obtain our estimate ${\hat\theta}_0$. 
\end{enumerate}

\noindent If we assume that $g_t(.) \ne g(.)$ then Step~(5) becomes applying $t$ learners in succession to the data from each wave.  \red{(is this implicitly assuming that realisations in $t-1$ are not correlated with those in $t$ for unit $i$?) [No - because $g_t$ and $m_t$ appear only at wave $t$, the learning is done only on the data at each wave; when it comes to plugging in the learnt functions into the estimating equation for $\theta_0$, however, the auto-correlation is taken into account]}  %For the Neyman-orthogonal estimating equation, Step~(5) would need to include estimating $m(\x)$ for the selection probabilities to obtain $m^p(\x)$.

\

\noindent \textbf{Correlated random effects (CRE).}
Let $\zit$ be a $k\times 1$ vector of strictly exogenous variables such that $\E[\nu_{it}|\zi] = 0$ and $\E[\epsilon_{it}|\zi] = 0$. Define $\bzi=T\inv\sum_{t=1}^T \zit$ to be a vector of time averages of $\zit$. Let $\xit=(\zit, \bzi, \wi)$ be a $p\times 1$ vector of pre-determined (time-varying and time-invariant) variables. Following \blue{Mundlak (1978)}'s CRE approach, the unobserved heterogeneity $\alpha_i$ is projected onto the vector of time-invariant exogenous characteristics as $\alpha_i = \bzi'\gre + \xi_i$ and $\E(\alpha_i|\zi)=\bzi'\gre$. [Yes! - but I think $M_i$ needs to include $d_{it}$.] 
\red{AP: We include the individual-specific average of the treatment using Mundlak's device as follows $\alpha_{i} = \bdi'\gre + \xi_i$ in the second stage of DML. Because the unobserved heterogeneity  is a linear projection and the functions are not linear we cannot use $\bxi$. Random forest estimates $m(.)$ using $\dit$ and $\xit$, and $g(.)$ using $\yit$ and $\xit$.}

\blue{ PC 18 Nov 6.30pm - I think Mundlak is fine here under mild assumptions (to be determined). Looking again at the original 1978 paper, everything hinges on there being a linear correlation between the individual effects and the regressors.  However, you are correct that it's only the effect of $d_{it}$ that concerns us, not that of $\xit$. This is because, as stated immediately after defining (\ref{eqn:outcome}), we can identify $\theta_0$ if $\E(\epsilon_{it}| \dit, \xit)=\E(\epsilon_{it} | \xit)$. This usually requires the individual effects $\alpha_i$ from (\ref{eqn:outcome}) and (the yet to be defined) $\psi_i$ from (\ref{eqn:treat}) to be uncorrelated. What's important here is that this moment restriction is the same whether the regressor effects are linear or non-linear in (\ref{eqn:outcome}). In the spirit of Mundlak, we now need to assume something like
\[
\alpha_i = \gamma_0 + \gamma}_1\bar{d}_i+\gamma_2\bar{h}(\bar{\bf{x}}_i)+a_i.
\]
Actually, $\bar{h}(\bar{\bf x}}_i) = \sum_{t=1}^Th(\xit)/T$ is a simplifying assumption (based on generalising equations (2.3) and (2.4) in Mundlak's paper, but really it's $\bar{h}(\xit)$) but we have no idea what $h$ is, only that it is a well-defined many-to-one mapping. If $\bar{h}$ was linear then we could only guarantee that $a_i$ was orthogonal to the column-span of $(\bf{d},X)$ and thus potentially dependent on $d_{it}$ (although hopefully not) and $g(\xit)$ (although we don't care about the latter).  The residual $a_i$ is orthogonal to the space spanned by $\bar{d}_i$ and $h_i=\bar{h}(\bar{\bf{x}}_i)$ even if it's not orthogonal to that spanned by $\bar{d}_i$ and $\xit$. This implies it's also orthogonal to that spanned by $d_{it},h_i$ if treatment is continuous. Hence, decomposing $\epsilon_{it}=\alpha_i + e_{it}$, (\ref{eqn:outcome}) can be rewritten as 
\[
y_{it}=\gamma_0 + d_{it}\theta_0 + \bar{d}_i\gamma_1 + k(\xit,\bar{\bf x}}_i) + a_i + e_{it},
\]
which means we must learn a linear combination of the two functions $k_{it}=k(\xit,\bar{\bf x}}_i) = g(\xit) + \gamma_2h(\bar{\bf{x}}_i)$. Hence, we have to assume something that ensures $a_i$ remains orthogonal to the space spanned by $d_{it}$ and $k_{it}$ (I think this is something like $h$ and $g$ being defined on the same function (Banach?) space such that $k$ is also defined on it).  (Note:\ If we hadn't included h then $a_i$ would not be orthogonal to this space and thus potentially correlated.)

This is a bit hand-wavy but will do for now.  Broadly, though, I think this is what you wrote above and told me this morning, but I didn't get what you meant.  However, if so, I belatedly agree!}



  g_hat = NULL
  if (exists("ml_g", where = private$learner_)) {
    # get an initial estimate for theta using the partialling out score
    psi_a = -(d - m_hat) * (d - m_hat)
    psi_b = (d - m_hat) * (y - l_hat)
    theta_initial = -mean(psi_b, na.rm = TRUE) / mean(psi_a, na.rm = TRUE)

    data_aux = data.table(self$data$data_model,
      "y_minus_theta_d" = y - theta_initial * d)

    g_hat = dml_cv_predict(self$learner$ml_g,
      c(self$data$x_cols, self$data$other_treat_cols),
      "y_minus_theta_d",
      data_aux,
      nuisance_id = "nuis_g",
      smpls = smpls,
      est_params = self$get_params("ml_g"),
      return_train_preds = FALSE,
      task_type = private$task_type$ml_g,
      fold_specific_params = private$fold_specific_params)
  }
